Pareto-frontier Entropy Search with Variational Lower Bound Maximization

This study considers multi-objective Bayesian optimization (MOBO) through the information gain of the Pareto-frontier. To calculate the information gain, a predictive distribution conditioned on the Pareto-frontier plays a key role, which is defined as a distribution truncated by the Pareto-frontier. However, it is usually impossible to obtain the entire Pareto-frontier in a continuous domain, and therefore, the complete truncation cannot be known. We consider an approximation of the truncate distribution by using a mixture distribution consisting of two possible approximate truncation obtainable from a subset of the Pareto-frontier, which we call over- and under-truncation. Since the optimal balance of the mixture is unknown beforehand, we propose optimizing the balancing coefficient through the variational lower bound maximization framework, by which the approximation error of the information gain can be minimized. Our empirical evaluation demonstrates the effectiveness of the proposed method particularly when the number of objective functions is large.

==> main-back.tex <==

% \tableofcontents


\begin{abstract}
This study considers multi-objective Bayesian optimization (MOBO) through the information gain of the Pareto-frontier. 
%
To calculate the information gain, a predictive distribution conditioned on the Pareto-frontier plays a key role, which is defined as a distribution truncated by the Pareto-frontier.
%
However, it is usually impossible to obtain the entire Pareto-frontier in a continuous domain, and therefore, the complete truncation cannot be known.
%
We consider an approximation of the truncated distribution by using a mixture distribution consisting of two possible approximate truncations obtainable from a subset of the Pareto-frontier, which we call over- and under-truncation.
% We first reveal two possible approximate truncation through the partially obtained Pareto-frontier, which we call over- and under-truncation.
%
Since the optimal balance of the mixture is unknown beforehand, we propose optimizing the balancing coefficient through the variational lower bound maximization framework, by which the approximation error of the information gain can be minimized. 
%
% Our empirical evaluation shows effectiveness of the proposed method by using several benchmark functions
Our empirical evaluation demonstrates the effectiveness of the proposed method particularly when the number of objective functions is large.
\end{abstract}



% \section{はじめに}
\section{Introduction}
\label{sec:intro}


% 複数のブラックボックス目的関数を同時に最適化する多目的最適化は様々な状況で重要である．
Multi-objective optimization (MOO) of black-box functions is ubiquitous in a variety of fields such as materials science, engineering, drug design, and AutoML.
%
% 例えば，材料開発における安定性と電気伝導度の最適化や，機械学習モデルの最適化における予測精度と公平性の最適化などトレードオフのある指標の最適化は分野横断的に現れる．
% For example, simultaneous optimization of multiple physical properties can be seen in material discovery, and performance optimization under multiple different criteria (such as accuracy, fairness, and robustness) of a machine learning model 
%
% 伝統的には遺伝アルゴリズムに基づく研究が盛んであったが，観測コストの高い問題では多数の世代数を前提とするものは適用が難しい．
Evolutionary algorithms have been classically studied for MOO, but they require a large number of function evaluations, which is often difficult for practical problems. 
%
% そこで，確率モデル（通常はガウス過程回帰）により未知の目的関数を推定しながら探索するベイズ最適化に基づく手法が様々研究されている（例えば\cite{Knowles2006-parego,Emmerich2005-single,Ponweiser2008-multiobjective,Belakaria2019-max,Suzuki2020-multi,Qing2022-text,Tu2022-joint}）．
On the other hand, Bayesian optimization (BO) based approaches to MOO, which use a probabilistic surrogate model (typically, Gaussian process), have been widely studied recently \citep[e.g.,][]{Knowles2006-parego,Emmerich2005-single,Ponweiser2008-multiobjective,Belakaria2019-max,Suzuki2020-multi,Qing2022-text,Tu2022-joint}. 


% 本稿では最適値の情報量を考えるアプローチに着目する\cite{Wang2017-Max}．
% We focus on an approach of multi-objective BO (MOBO) based on the information gain of Pareto-frontier \citep{Suzuki2020-multi}. 
This study focuses on multi-objective BO (MOBO) based on the information gain of the Pareto-frontier. %  \citep{Suzuki2020-multi}. 
%
% 通常，多目的最適化における最適値はパレートフロンティアと呼ばれる集合$\cF^*$として定義される．
Since the optimal solution of an MOO problem is not unique in general, the optimal values are represented as a set of output vectors, called the Pareto-frontier $\cF^*$.
%
% そのため獲得関数の自然な基準として観測する値とパレートフロンティアの間の情報量が考えられることが\cite{Suzuki2020-multi}により提案された．
% Pareto-frontier entropy search (PFES) \citep{Suzuki2020-multi} considers the information gain of Pareto-frontier as an acquisition function of MOBO.
Pareto-frontier entropy search (PFES) \citep{Suzuki2020-multi} considers the mutual information between the Pareto-frontier and a candidate point as an acquisition function of MOBO.
%
% この考え方はその後も拡張され\cite{Qing2022-text,Tu2022-joint}，パレートフロンティア全体の不確かさを考慮した意思決定を行うことで，実践上高い性能を発揮できることが示されてきた．
The effectiveness of the basic idea of PFES has been repeatedly shown \citep{Qing2022-text,Tu2022-joint}.


%パレートフロンティアの情報量を考える全ての既存手法で，パレートフロンティアが与えられたもとでの予測分布
%$p(\*f(\*x) \mid \cF^*)$
% が重要な役割を果たす（$\*f(\*x)$は入力$\*x$での目的関数値を並べたベクトルであり，$\cF^*$はガウス過程のサンプルパスから定まるパレートフロンティア）．
In the information-theoretic approaches considering the information of the Pareto-frontier \citep{Suzuki2020-multi,Qing2022-text,Tu2022-joint}, the predictive distribution given the Pareto-frontier $p(\*f(\*x) \mid \cF^*)$ plays a key role in the information evaluation, where $\*f(\*x)$ is a vector of objective function values at the input $\*x$.
%
% パレートフロンティアが条件付けられることで，それ以上に良い$\*f(\*x)$は存在し得ないため切断された分布を考えることになる（図\ref{fig:PFTN}(a)．図の詳細は\ref{ssec:VLBMaximization}節で議論する）．
In this distribution, $\*f(\*x)$ cannot be better than $\cF^*$ because $\cF^*$ should be the Pareto-frontier.
%
Therefore, $p(\*f(\*x) \mid \cF^*)$ becomes a truncated distribution (see Fig.~\ref{fig:PFTN}(a) for which details will be discussed in Section~\ref{ssec:VLBMaximization}).
%
% しかしながら連続空間の場合は$\cF^*$全体を得ることは実質的に不可能であり，実践上は有限サイズの部分集合
%$\cF^*_S \subseteq \cF^*$
%のみしか得られない（図\ref{fig:PFTN}(a)中，赤い星点）．
However, it is practically impossible to obtain the entire $\cF^*$ in a continuous space, and we only obtain a finite size subset $\cF^*_S \subseteq \cF^*$ (red stars in Fig.~\ref{fig:PFTN}(a)). 
%
% そのため，$\cF^*$による厳密な切断を実行することはできない．
This means that the exact truncation by $\cF^*$ shown in Fig.~\ref{fig:PFTN}(a) cannot be calculated.
%
% そこで既存の研究は全て有限個の点$\cF^*_S$を起点にして過剰に空間を切断する近似に基づいている（図\ref{fig:PFTN}(c)）．
To avoid this issue, all the existing studies use approximations based on an overly truncated distribution created by $\cF^*_S$ (Fig.~\ref{fig:PFTN}(d)).
%
% しかしながら，この方法は真の$\cF^*$による切断に比べてパレートフロンティアと$\*f(\*x)$の依存関係を強めに評価することになる（真の切断よりも$\*f(\*x)$の分布の変化が大きい）．
% A drawback of this approach is that dependency between $\*f(\*x)$ and $\cF^*$ is estimated always stronger than the true truncation.
A drawback of this approach is that the effect of truncation by $\cF^*$ on $\*f(\*x)$ is always estimated stronger than the true truncation, because of which we call it over-truncation.
% \note{entropyの変化を検証できないか}


% 本研究は情報論的多目的ベイズ最適化の情報量評価に初めて変分下限最大化原理を導入するものである．
In this study, we introduce the variational lower bound maximization approach into the mutual information (MI) estimation of information-theoretic MOBO, which is called Pareto-frontier Entropy search with Variational lower bound maximization (PFEV).
%
% 従来の過剰な切断に加え，新たに保守的な切断から定まる分布（図\ref{fig:PFTN}(b)）を考える．
In addition to the conventional over-truncation, we also consider a conservative approach, called under-truncation (shown as Fig.~\ref{fig:PFTN}(c)).
%
% 保守的な切断は真の$\cF^*$による切断に比べてパレートフロンティアと$\*f(\*x)$の依存関係を弱く見積もることになる．
The under-truncation estimates the effect of truncation by $\cF^*$ weaker than the true truncation.
%
% そこで提案法では，過剰および保守的な切断から定まる分布の混合により変分分布を作る（図\ref{fig:PFTN}(d)）．
Therefore, to balance two opposite approaches, we combine the over and the under-truncation in such a way that a mixture of them (Fig.~\ref{fig:PFTN}(e)) defines a variational distribution of the MI approximation.
%
% さらに，混合比を変分パラメータとみなして変分下限最大化で最適化する．
We show that the mixture weight can be optimized through the variational lower bound maximization.
% By regarding the mixture weight as a variational parameter, the variational lower bound can be optimized so that the MI approximation error is minimized.
% そのため混合比を適切に選ぶ必要があるが，混合比を変分パラメータとみなして変分下限最大化で最適化するのが提案法である．
%
% これにより変分分布と真の分布との近似の意味で，過剰な切断と保守的な切断の最も良いバランスを選択して情報量の評価を改善することができる．
This means that the optimal balance of the over and the under-truncation can be determined so that the MI approximation error is minimized.



% 本論文の貢献を要約すると以下となる．
Our contributions are summarized as follows:
\begin{itemize}
 \setlength{\itemsep}{0pt}
 \item % 提案法は連続空間における情報論的多目的ベイズ最適化において初めて情報量の完全な下限を用いるものである（既存の研究では，特定の条件下で$2$目的関数の場合のみしか示されていなかった）．
       PFEV is the first approach to continuous space MOBO that is based on a general lower bound of MI (existing work only shows a lower bound under a restrictive condition of two objective problems, for which we discuss in Section~\ref{sec:related-work}). 
       
 \item % 保守的な切断分布および，既存の過剰な切断との混合分布により変分分布を定義し，変分下限最大化を定式化する．
       We newly introduce an under-truncation approximation for $p(\*f(\*x) \mid \cF^*)$.
       %
       Further, we define variational distribution as a mixture of distributions with the over and the under-truncation, and show how to optimize the mixture weight.
       % for which the mixture weight can be optimized through variational lower bound maximization.
       %

 \item We also discuss properties and extensions of PFEV.
       % 下限とPI (probability of improvement)との関係性や，モンテカルロ近似による計算方法についても議論する．
       % For our MI lower bound, its relation with PI (probability of improvement) and a Monte-Carlo approximation are derived.
       For example, we show that our MI lower bound can be further lower bounded by PI (probability of improvement).
       %
       We also discuss a Monte-Carlo approximation tailored to our lower bound.
       % and 
       %
       We further discuss several extended settings such as parallel querying.

 \item % 人工関数やベンチマークデータにより提案法の精度評価を行い，提案法の探索効率が高いことを実証した．
       % Through empirical evaluation on Gaussian process generated and benchmark functions, we demonstrate effectiveness of PFEV.
       Through empirical evaluation on Gaussian process generated functions, benchmark functions, and an application to machine learning hyper-parameter optimization, we demonstrate effectiveness of PFEV.
       %
       % 特に，二種類の切断方法の違いは出力の次元が上がるほど顕著になるため混合の効果が期待されるが，実験的にもこの傾向が確認された．
       % Since difference between the over and the under truncation becomes large when the output dimension is high, a stronger benefit of using the mixture can be expected.
       %
       % We actually observed that PFEV is effective particularly in larger output dimension problems. 
       We empirically observed that PFEV shows a particular difference from existing over-truncation based methods when output dimension $\geq 3$, in which the difference of two truncation becomes more apparent. 
\end{itemize}

% --------------------------------------------------
% \section{多目的最適化の最適性とガウス過程回帰}
\section{Multi-Objective Optimization and Gaussian Process Model}
\label{sec:preliminary}

% \note{(Memo: PFES論文そのまますぎるので少し変えたが, もう少し変えた方が良いかも)}


% 入力空間 $\cX \subseteq \RR^d$ に対して，$L \geq 2$ 個の目的関数 
% $f^l: \cX \rightarrow \RR$ $(l = 1, \ldots, L)$
% の最大化を考える多目的最適化問題を扱う．
We consider Bayesian optimization (BO) for a multi-objective optimization (MOO) problem of maximizing $L \geq 2$ objective functions 
$f^l: \cX \rightarrow \RR$ $(l = 1, \ldots, L)$,
where 
$\cX \subseteq \RR^d$
is an input space. 
%
Let
$\*f_{\*x} \coloneqq (f^1_{\*x}, \ldots, f^L_{\*x})^\top$, 
where $f^l_{\*x} \coloneqq f^l(\*x)$. 
%
% 多目的最適化問題における最適解は，通常パレート最適性によって定義される．
The optimal solutions of MOO are characterized by the Pareto optimality. 
%
% 2つの点 $\*f_{\*x}$ と $\*f_{\*x'}$ について，すべての $l \in \{ 1, \ldots, L \}$ に対して $f^l_{\*x} \geq f^l_{\*x'}$ が成り立ち，少なくとも1つの不等式が等号無しで成り立つとき，「$\*f_{\*x}$ は $\*f_{\*x'}$ を支配する」といい，この関係を $\*f_{\*x} \succ \*f_{\*x'}$ と表す．
For given $\*f_{\*x}$ and $\*f_{\*x'}$, 
if 
$f^l_{\*x} \geq f^l_{\*x'}$ for $\forall l \in \{ 1, \ldots, L \}$  
and there exists $l$ that satisfies 
$f^l_{\*x} > f^l_{\*x'}$,
then ``$\*f_{\*x}$ dominates $\*f_{\*x'}$'', written as $\*f_{\*x} \succ \*f_{\*x'}$.
%
% 領域内の他のどの $\*f_{\*x'}$ にも支配されない $\*f_{\*x}$ をパレート最適という．
When $\*f_{\*x}$ is not dominated by any other $\*f_{\*x'}$, then $\*f_{\*x}$ is Pareto-optimal.
%
% パレートフロンティア $\cF^*$ は，パレート最適な $\*f_{\*x}$ の集合であり，
% $\cF^* \coloneqq \{ \*f_{\*x} \in \cF_{\cX} \mid \*f_{\*x'} \not\succ \*f_{\*x}, \forall \*f_{\*x'} \in \cF_{\cX} \}$ 
% と表される．
The Pareto-frontier $\cF^*$ is a set of Pareto-optimal $\*f_{\*x}$ that can be defined as
$\cF^* \coloneqq \{ \*f_{\*x} \in \cF_{\cX} \mid \*f_{\*x'} \not\succ \*f_{\*x}, \forall \*f_{\*x'} \in \cF_{\cX} \}$,
where 
$\cF_{\cX} \coloneqq \{ \*f_{\*x} \in \RR^L \mid \forall \*x \in \cX \}$.
%
% ただし，
% $\cF_{\cX} \coloneqq \{ \*f_{\*x} \in \RR^L \mid \forall \*x \in \cX \}$ 
% である．
%
% パレート最適点は無限に存在し得るが，多くの手法では真のパレートフロンティア $\cF^*$ を十分な精度で近似する小さな部分集合を見つけることを目指す．


% 各目的関数をガウス過程回帰によってモデル化する．
Each objective function is represented by the Gaussian process (GP) regression.
%
% $\*x_i$ の $l$ 番目の目的関数値に対する観測値は 
% $y_{i}^l = f^l_{\*x_i} + \veps$ 
% と仮定し，
%$\veps \sim \cN(0,\sigma^2_{\rm noise})$ 
%とする．
The observation of the $l$-th objective function is 
$y_{i}^l = f^l_{\*x_i} + \veps$,
where 
$\veps \sim \cN(0,\sigma^2_{\rm noise})$.
%
% 訓練データは 
% $\cD \coloneqq \{ (\*x_i, \*y_i )\}_{i = 1}^n$ 
% と表され，
% $\*y_i = (y_{i}^1,\ldots,y_{i}^L)^\top$
% である．
The training dataset with $n$ observations is written as
$\cD \coloneqq \{ (\*x_i, \*y_i )\}_{i = 1}^n$, 
where 
$\*y_i = (y_{i}^1,\ldots,y_{i}^L)^\top$.
%
% カーネル関数 $k(\*x,\*x')$ を用いて，独立な $L$ 個のガウス過程回帰を各次元に適用する．
We use independent $L$ GPs with a kernel function $k(\*x,\*x')$.
%
% ここで
% $\*k(\*x) \coloneqq (k(\*x,\*x_1),\ldots,k(\*x_,\*x_n))^\top$，
% $\*y^l \coloneqq (y_{1}^l, \ldots, y_{n}^l)^\top$ 
% であり，$\*K$ は $(i,j)$ 要素が $k(\*x_i,\*x_j)$ で定義されるカーネル行列とする．
Let
$\*k(\*x) \coloneqq (k(\*x,\*x_1),\ldots,k(\*x_,\*x_n))^\top$, 
$\*y^l \coloneqq (y_{1}^l, \ldots, y_{n}^l)^\top$, 
and
$\*K$ be the matrix whose $(i,j)$-element is $k(\*x_i,\*x_j)$.
%
% このとき，事前平均を0と設定すると$l$ 番目のガウス過程回帰の事後分布
% $p(f^l_{\*x} \mid \cD)$
% は
% $\cN(\mu_l(\*x), \sigma^2_l(\*x))$
% であり，平均と分散は
% $\mu_l(\*x) = \*k(\*x)^\top \left( \*K + \sigma^2_{\rm noise} \*I \right)^{-1} \*y^{l}$
% と
% $\sigma^2_l(\*x) = k(\*x,\*x) - \*k(\*x)^\top \left( \*K + \sigma^2_{\rm noise} \*I \right)^{-1} \*k(\*x)$
% となる．
The posterior 
$p(f^l_{\*x} \mid \cD)$ 
of the $l$-th GP (with $0$ prior mean) is written as 
$\cN(\mu_l(\*x), \sigma^2_l(\*x))$,
where 
$\mu_l(\*x) = \*k(\*x)^\top \left( \*K + \sigma^2_{\rm noise} \*I \right)^{-1} \*y^{l}$
and
$\sigma^2_l(\*x) = k(\*x,\*x) - \*k(\*x)^\top \left( \*K + \sigma^2_{\rm noise} \*I \right)^{-1} \*k(\*x)$.
%
% 独立性より
% $p(\*f_{\*x} \mid \cD) = \prod_{l \in [L]} p(f^l_{\*x} \mid \cD)$
% である．
From independence, we have 
$p(\*f_{\*x} \mid \cD) = \prod_{l \in [L]} p(f^l_{\*x} \mid \cD)$.
% また，
% $\*\mu(\*x) \coloneqq (\mu_1(\*x),\ldots,\mu_L(\*x))^\top$ 
% および 
% $\*\sigma(\*x) \coloneqq (\sigma_1(\*x),\ldots,\sigma_L(\*x))^\top$ 
% と定義する．
%
% 簡潔性のため，訓練データ $\cD$ による条件付けは表記上省略する．
For notational brevity, conditioning on $\cD$ is omitted (e.g., $p(\*f_{\*x} \mid \cD)$ is written as $p(\*f_{\*x})$).
%
% 例えば，事後分布 $p(\*f_{\*x} \mid \cD)$ は $p(\*f_{\*x})$ と表記する．

% --------------------------------------------------
\section{Pareto-frontier Entropy Search with Variational Lower Bound Maximization}
\label{sec:PFEV}

% 本節では，観測 $\*f_{\*x}$ とパレートフロンティア $\cF^*$ との相互情報量 
% ${\rm MI}(\*f_{\*x} ; \cF^*)$
% を基にした多目的ベイズ最適化の獲得関数を考える． 
We consider multi-objective Bayesian optimization (MOBO) based on mutual information 
${\rm MI}(\*f_{\*x} ; \cF^*)$
between an objective function value $\*f_{\*x}$ and the Pareto-frontier $\cF^*$ (Note that, throughout the paper, $\cF^*$ is a random variable determined via the predictive distribution of $\*f_{\*x}$).
%
An intuition behind this criterion is to select $\*x$ that provides the maximum information gain of the Pareto-frontier $\cF^*$.
%
% ${\rm MI}(\*f_{\*x} ; \cF^*)$は\citep{Suzuki2020-multi}が提案した指標であり，$\*f_{\*x}$を観測することで最適な$\cF^*$について得られる情報量だと解釈できる．
The effectiveness of this approach is shown by \citep{Suzuki2020-multi}, but it is known that accurate evaluation of ${\rm MI}(\*f_{\*x} ; \cF^*)$ is difficult.
%
% しかしながら，情報量
% ${\rm MI}(\*f_{\*x} ; \cF^*)$
% は厳密評価が難しいことが知られている．
%
% 提案法は${\rm MI}(\*f_{\*x} ; \cF^*)$の評価に変分下限最大化原理を初めて導入するものであり，2種類の分布の組み合わせにより変分分布を構成する．
Our proposed method is the first method introducing the variational lower bound maximization to evaluate ${\rm MI}(\*f_{\*x} ; \cF^*)$. 
%
% 本稿ではこの方法を Pareto-frontier Entropy search with Variational lower bound maximization（PFEV）と呼ぶ．
We call our proposed method Pareto-frontier Entropy search with Variational lower bound maximization (PFEV). 

% --------------------------------------------------
% \subsection{Variation Lower Bound (VLB)}
\subsection{Lower Bound of Mutual Information}
\label{ssec:VLB}

% ${\rm MI}(\*f_{\*x} ; \cF^*)$ の変分下限 $L(\*x)$ を以下のように定義する：
A lower bound $\mr{LB}(\*x)$ of ${\rm MI}(\*f_{\*x} ; \cF^*)$ can be derived as 
\begin{align}
 & \mr{MI}(\*f_{\*x} ; \cF^* ) 
 \notag \\
 & =
 \int p(\cF^*) \int p(\*f_{\*x} \mid \cF^*) 
 \log \frac{ p({\*{f}_{\*{x}}} \mid \cF^*) }{ p({\*{f}_{\*{x}}}) } \mr{d} \*f_{\*x} \mr{d} \cF^* 
 \notag \\ % ---
 & = \int p(\cF^*) \sbr{ 
 \int p(\*f_{\*x} \mid \cF^*) \log \frac{ q(\*{f}_{\*{x}} \mid \cF^*) }{ p(\*f_{\*x}) } \mr{d} \*{f}_{\*x} \right.
 \notag \\
 & \qquad \left. + D_{\mr{KL}}\rbr{ 
 p(\*f_{\*x} \mid \cF^*) \parallel q(\*f_{\*x} \mid \cF^*) 
 } 
 } \mr{d} \cF^* 
 \notag \\ % ---
 & \geq \EE_{\cF^*}\sbr{
 \int p(\*f_{\*x} \mid \cF^*) \log \frac{q(\*f_{\*x} \mid \cF^{*})}{p(\*f_{\*x})} \mr{d} \*f_{\*x}
 } \notag \\ % ---
 & = \EE_{\cF^*, \*f_{\*x}}\sbr{
 \log \frac{q(\*f_{\*x} \mid \cF^{*})}{p(\*f_{\*x})} 
 }
 \eqqcolon \mr{LB}(\*{x}), 
\label{eq:VLB-q}
\end{align}
where $D_{\mr{KL}}$ is Kullback-Leibler (KL) divergence, and $q(\*f_{\*x} \mid \cF^*)$ is a density function called a variational distribution. 
% ただし，$D_{\mr{KL}}$ はKullback-Leibler（KL）ダイバージェンスであり，$q(\*f_{\*x} \mid \cF^*)$ は変分分布と呼ばれる確率密度関数である．
%
A similar lower bound was first derived in the context of constrained BO \citep{Takeno2022-Sequential}.
% 同様の方法で導出される下限は制約付きベイズ最適化の文脈で\citep{Takeno2022-Sequential}でも用いられている．
%
% この下限は，以下のsupport条件を満たす任意の $q(\*f_{\*x} \mid \cF^*)$ に対して成立する：
This lower bound holds for any distribution $q(\*f_{\*x} \mid \cF^*)$ that satisfies the following support condition: 
\begin{align}
\mr{supp}(q(\*f_{\*x} \mid \cF^*)) \supseteq \mr{supp}(p({\*f_{\*x}} \mid \cF^*)), 
\label{eq:VDC}
\end{align}
% ただし，$\mr{supp}$は任意の確率密度関数 $p$ に対して，
% $\mr{supp}(p(\*f \mid \cF^*)) = \{ \*f \in \RR^L \mid p(\*f \mid \cF^*) \neq 0 \}$ 
%と定義される．
where $\mr{supp}$ is a set of non-zero points of a given density, defined as 
$\mr{supp}(p(\*f \mid \cF^*)) = \{ \*f \in \RR^L \mid p(\*f \mid \cF^*) \neq 0 \}$. 
%
% この条件に加え，$0 \log 0 = 0$ という情報理論における慣習的条件\citep{Cover2006-Elements}を用いることで，$L(\*x)$ が定義できることに注意されたい．
In addition to this condition, the lower bound 
% $L(\*x)$ 
$\mr{LB}(\*x)$ 
is derived by using the convention $0 \log 0 = 0$ \citep{Cover2006-Elements}. 
%
% なお，条件\eq{eq:VDC}を variational distribution condition（VDC）と呼ぶことにする（VDCが成立しない場合，$\log 0$により未定義となる）．
We call the condition \eq{eq:VDC} variational distribution condition (VDC). 
%
Note that if VDC is not satisfied, 
$\mr{LB}(\*x)$ 
is not defined, 
because then, the probability measure induced by 
$p({\*f_{\*x}} \mid \cF^*)$
is not absolutely continuous 
with respect to those of
$q(\*f_{\*x} \mid \cF^*)$.
% $L(\*x)$ 
% $\mr{LB}(\*x)$ 
% is not defined because of $\log 0$.

% --------------------------------------------------
\subsection{Variational Lower Bound Maximization by Combining Over- and Under-Truncation}
% \subsection{保守的および過剰な切断の組み合わせによる\\変分下限最大化}
\label{ssec:VLBMaximization}

% 下限 $L(\*x)$ は 
% $q(\*f_{\*x} \mid \cF^*) = p(\*f_{\*x} \mid \cF^*)$ 
% のとき，真の $\mr{MI}(\*f_{\*x} ; \cF^*)$ と一致する．
If 
$q(\*f_{\*x} \mid \cF^*) = p(\*f_{\*x} \mid \cF^*)$ for $\cF^*$ almost everywhere, the lower bound 
% $L(\*x)$ 
$\mr{LB}(\*x)$ 
is equal to 
$\mr{MI}(\*f_{\*x} ; \cF^*)$. 
%
% しかしながら，$p(\*f_{\*x} \mid \cF^*)$ の解析的な表現は知られていない．
However, the analytical representation of 
$p(\*f_{\*x} \mid \cF^*)$
is not known.
%
% この問題は情報論的なベイズ最適化に共通の問題として知られており，切断正規分布による近似が効果的であることが繰り返し示されている（例えば\citep{Wang2017-Max,Takeno2020-Multifidelity,Perrone2019-Constrained,Suzuki2020-multi}）．
This stems from a common well-known difficulty of information-theoretic BO, and effectiveness of the truncated distribution based approximation has been repeatedly shown \citep[e.g.,][]{Wang2017-Max,Takeno2020-Multifidelity,Perrone2019-Constrained,Suzuki2020-multi} not only for MOBO, but also for a variety contexts of BO problems (such as standard single-objective problems, constraint problems, and multi-fidelity problems). 


% ここで，$\*f \in \RR^L$に対して，$\*f \preceq \cF^*$としたときに$\*f$は$\cF^*$のいずれかの要素によって支配されているか同じ値であるとする．
Define 
$\*f \preceq \cF^*$
as that $\*f$ is dominated by or equal to at least one element in $\cF^*$. 
%
% 切断近似を用いると，
% $p(\*f_{\*x} \mid \cF^*)$
% の条件部を
% $\*f_{\*x} \preceq \cF^*$
% を満たす領域で正規分布を切断する条件に置き換えた
% $q(\*f_{\*x} \mid \cF^*) = p(\*f_{\*x} \mid \*f_{\*x} \preceq \cF^*)$
% を用いることになる： 
The truncation-based approximation replaces the conditioning in 
$p(\*f_{\*x} \mid \cF^*)$
with
$\*f_{\*x} \preceq \cF^*$, 
by which we obtain
$q(\*f_{\*x} \mid \cF^*) = p(\*f_{\*x} \mid \*f_{\*x} \preceq \cF^*)$: 
\begin{align*}
q(\*f_{\*x} \mid \cF^*) = 
 \begin{cases}
  p(\*f_{\*x}) / Z^{\cF^*}(\*x) & \text{ if }  \*f_{\*x} \in \cA^{\cF^*}, \\
  0 & \text{ otherwise, }
 \end{cases}
\end{align*}
% ただし，
% $\cA^{\cF^*} \coloneqq \{ \*f \in \RR^L \mid \*f \preceq \*f^\prime, \exists \*f^\prime \in \cF^* \}$ 
% および 
% $Z^{\cF^*}(\*x) \coloneqq p(\*f_{\*x} \in \cA^{\cF^*})$ 
% である．
where
$\cA^{\cF^*} \coloneqq \{ \*f \in \RR^L \mid \*f \preceq \*f^\prime, \exists \*f^\prime \in \cF^* \}$ 
and
$Z^{\cF^*}(\*x) \coloneqq p(\*f_{\*x} \in \cA^{\cF^*})$
is the normalization constant. 
%
% 図\ref{fig:PFTN}(a)に示す通り，$q(\*f_{\*x} \mid \cF^*)$ は $\cF^*$ によって支配される領域のみを残して切断した正規分布である．
As shown in Fig.~\ref{fig:PFTN}(a), 
$q(\*f_{\*x} \mid \cF^*)$ is a truncated normal distribution in which only the region dominated by $\cF^*$ remains.
%
% \citep{Suzuki2020-multi}はこれをPFTN (Pareto-Frontier Truncated Normal distribution)と呼んだ．
\citet{Suzuki2020-multi} call this distribution PFTN (Pareto-Frontier Truncated Normal distribution). 
%
%これは，$\cF^*$ が与えられたとき，$\cF^*$ を支配するような $\*f_{\*x}$ は存在し得ないという条件を元々の予測分布に課したものとして解釈できる．
PFTN is derived by the fact that if $\cF^*$ is given, any $\*f_{\*x}$ dominating $\cF^*$ cannot exist.
%
% しかしながら実践上は連続空間で完全な $\cF^*$ を求めることは難しく，図\ref{fig:PFTN}(a)の星印で示すような離散的な点だけしか得ることができない（そのような点の取得方法については \ref{ssec:computations}節で述べる）．
However, $\cF^*$ cannot be obtained in practice in the continuous domain, and we only obtain limited discrete points, such as those indicated by the red star points in Fig.~\ref{fig:PFTN}(a).
%
% この離散点からなる $\cF^*$ の部分集合を $\cF^*_S \subseteq \cF^*$ とする．
A subset of $\cF^*$ defined by these discrete points is written as $\cF^*_S \subseteq \cF^*$ (we discuss how to calculate $\cF^*_S$ in Section~\ref{ssec:computations}).
%
% 本研究では，この離散点 $\cF^*_S$ を起点とする2種類の切断を考える．
In this study, we consider combining two truncated distributions derived from
$\cF^*_S$, instead of using $\cF^*$ that is not obtainable. 


% --------------------------------------------------
% Fig: PFTN
% --------------------------------------------------
\begin{figure}[t]
 \centering

 \subfigure[]{
 \ig{.15}{./figs/PFTN-a-crop.pdf}}
 \subfigure[]{
 \ig{.15}{./figs/PFTN-PF.pdf}}

 \subfigure[]{
 \ig{.15}{./figs/PFTN-b-ver5.pdf}}
 \subfigure[]{
 \ig{.15}{./figs/PFTN-c-ver5.pdf}}
 \subfigure[]{
 \ig{.15}{./figs/PFTN-d-ver4.pdf}}
 \caption{
 % (a) $\cF^*$で切断された正規分布$q(\*f_{\*x} \mid \cF^*)$．
 (a) Predictive distribution truncated by $\cF^*$.
 %
 (b) Examples of possible truncation given $\cF^*_S$.
 % (b) $\tilde{\cF}^*_S$を起点に保守的に切断した正規分布$q_U(\*f_{\*x} \mid \tilde{\cF}^*_S)$．
 (c) Under-truncation based on $\tilde{\cF}^*_S$. 
 %
 % (c) $\tilde{\cF}^*_S$を起点に過剰に切断した正規分布$q_O(\*f_{\*x} \mid \tilde{\cF}^*_S)$．
 (d) Over-truncation based on $\tilde{\cF}^*_S$.
 %
 % (d) $q_U(\*f_{\*x} \mid \tilde{\cF}^*_S)$と$q_O(\*f_{\*x} \mid \tilde{\cF}^*_S)$の混合分布$q_\lambda(\*f_{\*x} \mid \tilde{\cF}^*_S)$．
 (e) Mixture of 
 $q_U(\*f_{\*x} \mid \tilde{\cF}^*_S)$
 and
 $q_O(\*f_{\*x} \mid \tilde{\cF}^*_S)$.
 }
 \label{fig:PFTN}
\end{figure}

% % --------------------------------------------------
% % Fig: PFTN
% % --------------------------------------------------
% \begin{figure}[t]
%  \begin{center}
%   \ig{.45}{./figs/truncate-dists.pdf}
%  \end{center}
%  \caption{
%  % (a) $\cF^*$で切断された正規分布$q(\*f_{\*x} \mid \cF^*)$．
%  (a) Predictive distribution truncated by $\cF^*$.
%  %
%  % (b) $\tilde{\cF}^*_S$を起点に保守的に切断した正規分布$q_U(\*f_{\*x} \mid \tilde{\cF}^*_S)$．
%  (b) Under truncation based on $\tilde{\cF}^*_S$. 
%  %
%  % (c) $\tilde{\cF}^*_S$を起点に過剰に切断した正規分布$q_O(\*f_{\*x} \mid \tilde{\cF}^*_S)$．
%  (c) Over truncation based on $\tilde{\cF}^*_S$.
%  %
%  % (d) $q_U(\*f_{\*x} \mid \tilde{\cF}^*_S)$と$q_O(\*f_{\*x} \mid \tilde{\cF}^*_S)$の混合分布$q_\lambda(\*f_{\*x} \mid \tilde{\cF}^*_S)$．
%  (d) Mixture of 
%  $q_U(\*f_{\*x} \mid \tilde{\cF}^*_S)$
%  and
%  $q_O(\*f_{\*x} \mid \tilde{\cF}^*_S)$.
%  }
%  \label{fig:PFTN}
% \end{figure}


In Fig.~\ref{fig:PFTN}(b), the orange dashed lines are examples of possible truncation behind $\cF_S^*$ and the red dot line is the true $\cF^*$, which is unknown.
%
% 一つ目の切断が図\ref{fig:PFTN}(b)に示す保守的な切断である．
The first truncated distribution is based on the most conservative truncation shown in Fig.~\ref{fig:PFTN}(c). 
%
% この切断は $\cF^*_S$ のいずれかの要素を支配する領域を $0$ にすることで定義される（$\cF^*_S$ がパレート最適であると条件付けられているため，$\cF^*_S$を支配する領域に点が存在してはならない）．
This truncation is defined by removing ``the region that dominates $\cF^*_S$'' (any point that dominates $\cF^*_S$ cannot exist).
%
% 切断されて残る領域を $\cA_U^{\cF^*_S} \coloneqq \RR^L \setminus \{ \*f \in \RR^L \mid \*f^\prime \preceq \*f, \exists \*f^\prime \in \cF^*_S \}$ と定義する．
The remaining region is written as
$\cA_U^{\cF^*_S} \coloneqq \RR^L \setminus \{ \*f \in \RR^L \mid \*f^\prime \preceq \*f, \exists \*f^\prime \in \cF^*_S \}$. 
%
% このとき，保守的な切断が定義する切断分布を
The resulting truncated normal distribution is
\begin{align*}
q_U(\*f_{\*x} \mid \cF^*_S) \coloneqq 
\begin{cases}
p(\*f_{\*x}) / Z_U^{\cF^*_S}(\*x) & \text{ if } \*f_{\*x} \in \cA_U^{\cF^*_S}, \\
0 & \text{ otherwise, }
\end{cases}	
\end{align*}
% と表す．
%
% ただし，$Z_U^{\cF^*_S}(\*x) \coloneqq p(\*f_{\*x} \in \cA_U^{\cF^*_S})$ である．
where 
$Z_U^{\cF^*_S}(\*x) \coloneqq p(\*f_{\*x} \in \cA_U^{\cF^*_S})$.
%
We call this distribution PFTN-U (PFTN with under-truncation).
%
% この分布は広いsupportを持ち，$\mr{supp}(q_U(\*f_{\*x} \mid \cF^*_S)) \supseteq \mr{supp}(p({\*f_{\*x}} \mid \cF^*))$ となりVDCを満たす．
PFTN-U has a larger support
$\mr{supp}(q_U(\*f_{\*x} \mid \cF^*_S)) \supseteq \mr{supp}(p({\*f_{\*x}} \mid \cF^*))$,
and thus, VDC is satisfied.
%
% 切断され $0$ になる領域を実際の切断より小さく見積もっており，保守的な切断だと解釈できる（$\*f_{\*x} \preceq \cF^*$ という条件が $\*f_{\*x}$ に与える影響を小さめに見積もっている）．
This truncation is conservative in the sense that the region where the density function becomes zero is smaller than 
$q(\*f_{\*x} \mid \cF^*)$, 
by which it underestimates the effect of the condition $\*f_{\*x} \preceq \cF^*$ on $\*f_{\*x}$.
%


% 二つ目の切断が図\ref{fig:PFTN}(c)に示す過剰な切断である．
The second truncated distribution is based on the over-truncation shown in Fig~\ref{fig:PFTN}(d).
%
% この領域は $\cF^*_S$ が支配する領域の和集合であり，
% $\cA_O^{\cF^*_S} \coloneqq \{ \*f \in \RR^L \mid \*f \preceq \*f^\prime, \exists \*f^\prime \in \cF^*_S \}$ 
% と定義する．
This is ``the region dominated by $\cF^*_S$'', defined as
$\cA_O^{\cF^*_S} \coloneqq \{ \*f \in \RR^L \mid \*f \preceq \*f^\prime, \exists \*f^\prime \in \cF^*_S \}$. 
%
% このとき，過剰な切断が定義する分布を
The resulting truncated normal distribution is 
\begin{align*}
 q_O(\*f_{\*x} \mid \cF^*_S) \coloneqq
 \begin{cases}
  p(\*f_{\*x}) / Z_O^{\cF^*_S}(\*x) & \text{ if } \*f_{\*x} \in \cA_O^{\cF^*_S}, \\
  0 & \text{ otherwise, }	 
 \end{cases}
\end{align*}
% と表す．
%
%ただし，
%$Z_O^{\cF^*_S}(\*x) \coloneqq p(\*f_{\*x} \in \cA_O^{\cF^*_S})$ である．
where 
$Z_O^{\cF^*_S}(\*x) \coloneqq p(\*f_{\*x} \in \cA_O^{\cF^*_S})$.
%
% この分布は $q_U$ とは逆に過剰な切断であり，supportが $p(\*f_{\*x} \mid \cF^*)$ より狭くなっている（$\*f_{\*x} \preceq \cF^*$ という条件が $\*f_{\*x}$ に与える影響を大きめに見積もっている）．
In contrast to $q_U$, $q_O$ overly truncates the distribution in the sense that the region where the density function value becomes zero is larger than $q(\*f_{\*x} \mid \cF^*)$, by which it overestimates the effect of the condition $\*f_{\*x} \preceq \cF^*$ on $\*f_{\*x}$.
%
We call this distribution PFTN-O (PFTN with over-truncation).
% また，このことによりVDCを満たさない．
%
It is important to note that PFTN-O may not satisfy VDC \eq{eq:VDC} because 
$\mr{supp}(q_O(\*f_{\*x} \mid \cF^*_S)) \subseteq \mr{supp}(p({\*f_{\*x}} \mid \cF^*))$.


% --------------------------------------------------
% Fig: Difference over and under in 3dim
% --------------------------------------------------
\begin{figure}[t]
 \begin{center}
  \ig{.3}{./figs/over-under-3dim.pdf}
 \end{center}
 \caption{
 % 出力$3$次元の場合の$2$種類の切断の例．
 An example of truncation in three-dimensional output space.
 %
 The resulting truncate regions have a large difference.
 % 切断後に残るsupport領域が大きく異なるため$q_U$と$q_O$は大きく異なる分布になる可能性がある．
 }
 \label{fig:over-under-3dim}
\end{figure}


As we have already discussed, $q_O$ and $q_U$ over and under estimates the truncation by the true $\cF^*$.
%
Therefore, instead of using one of them, we consider the mixture defined as follows:
% すでに述べた通り，$q_O$ と $q_U$ はそれぞれ $\cF^*$ が与えられた後のsupportの変化を過大および過小評価している（
% $\cA_O^{\cF^*_S} \subseteq \cA^{\cF^*} \subseteq \cA_U^{\cF^*_S}$
% ）．
%
% 特に出力の次元が大きい時，2つの切断方法のどちらを採用したかによるsupportのずれは大きなものになる（図\ref{fig:over-under-3dim}は$L = 3$の場合）．
%
% そこでPFEVでは，保守的な切断分布と過剰な切断分布の混合により変分分布を定義する：
\begin{align}
& q_{\lambda}(\*f_{\*x} \mid \cF^*_S) 
= \lambda q_U(\*f_{\*x} \mid \cF^*_S) + (1 - \lambda) q_O(\*f_{\*x} \mid \cF^*_S), 
\notag \\ 
& =
\begin{cases}
 % \rbr{ \lambda / Z_U^{\cF^*_S}(\*x) + (1 - \lambda) / Z_O^{\cF^*_S}(\*x) } p(\*f_{\*x}) & 
\rbr{ \frac{ \lambda }{ Z_U^{\cF^*_S}(\*x) } + \frac{ 1 - \lambda }{ Z_O^{\cF^*_S}(\*x)} } p(\*f_{\*x}) & 
\text{ if } \*f_{\*x} \in \cA_O^{\cF^*_S}, 
\\
\lambda p(\*f_{\*x}) / Z_U^{\cF^*_S}(\*x) 
& \text{ if } \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S}, 
\\
0 & \text{ otherwise, }
\end{cases}
\label{eq:q}
\end{align}
% ただし，$\cA_{U \setminus O}^{\cF^*_S} \coloneqq \cA_U^{\cF^*_S} \setminus \cA_O^{\cF^*_S}$ かつ $\lambda \in (0, 1]$ は混合比とする．
where 
$\cA_{U \setminus O}^{\cF^*_S} \coloneqq \cA_U^{\cF^*_S} \setminus \cA_O^{\cF^*_S}$,
and 
$\lambda \in (0, 1]$ is a weight of the mixture.
%
% $\lambda \neq 0$ とすることで，
% $\mr{supp}(q_{\lambda}(\*f_{\*x} \mid \cF^*_S)) \supseteq \mr{supp}(p({\*f_{\*x}} \mid \cF^*))$ 
% を満たすため，この混合分布はVDCを満たしている．
Because of 
$\lambda \neq 0$,
we have 
$\mr{supp}(q_{\lambda}(\*f_{\*x} \mid \cF^*_S)) \supseteq \mr{supp}(p({\*f_{\*x}} \mid \cF^*))$, 
meaning that the mixture satisfies VDC.
%
% 混合による近似のイメージを図\ref{fig:PFTN}(d)に示す．
Figure~\ref{fig:PFTN}(e) shows an example of the mixture.
%
% $\lambda$により，過小及び過剰な切断の影響度合いをコントロールできるようになっている．
The effect of PFTN-U and PFTN-O can be controlled by $\lambda$. 
%
% 特に出力の次元が大きい時，2つの切断方法のどちらを採用したかによるsupportのずれは大きなものになる（図\ref{fig:over-under-3dim}は$L = 3$の場合）．
% Particularly when the dimension of the output $L$ is large, difference between two types of truncation should be large (Fig.~\ref{fig:over-under-3dim} shows an illustration of $L = 3$), and therefore, the balance of them can have a larger effect.
% Note that when $|\cF^*_S| \rightarrow \infty$, the difference between PFTN-U and PFTN-O should decrease (because $\cF^*_S$ approaches to $\cF^*$).
%
% However, the practical size of $|\cF^*_S|$ (such as $50$) is usually small particularly for $L \geq 3$ (Fig.~\ref{fig:over-under-3dim} shows an illustration of $|\cF^*_S| = 2$ in $L = 3$), and therefore, we conjecture that the balance of them can have a large effect.
% \red{The difference between two types of truncation should be particularly large when the dimension of the output $L$ is large (even in the case of $L = 3$, a large difference can be seen as illustrated in Fig.~\ref{fig:over-under-3dim}).
%
% Therefore, we conjecture that the balance of them can have a strong effect particularly for problems with $L \geq 3$.}
% \red{
In the 2D illustration in Fig.~\ref{fig:PFTN}, the difference between the two truncations might appear small.
%
However, as shown in Fig.~\ref{fig:over-under-3dim}, in three or more dimensions, the two truncations are significantly different, obviously (further discussion is in Appendix~\ref{app:hyper-volume}).
%
Therefore, we conjecture that the balance of them can have a strong effect, particularly for problems with $L \geq 3$.
% }

By substituting 
$q_{\lambda}(\*f_{\*x} \mid \cF^*_S)$ 
into
% $L(\*x)$,
$\mr{LB}(\*x)$,
we define 
% $L(\*x, \lambda)$ 
$\mr{LB}(\*x, \lambda)$ 
as 
% $q_{\lambda}(\*f_{\*x} \mid \cF^*_S)$ を $L(\*x)$ に代入したものを $L(\*x, \lambda)$ とすると
\begin{align}	
& 
% L(\*x, \lambda) 
\mr{LB}(\*x, \lambda) 
\notag
\\
& =
\EE_{\cF^*, \*f_{\*x}} \sbr{
\log \rbr{ 
\frac{ \lambda q_U(\*f_{\*x} \mid \cF^*_S) + (1 - \lambda) q_O(\*f_{\*x} \mid \cF^*_S) }
{ p(\*f_{\*x}) } 
} } \notag
\\ % ---
% & = \EE_{\cF^*, \*f_{\*x}} \sbr{
% \log
% \left\{
% \rbr{ 
% \frac{ \lambda }{ Z_U^{\cF^*_S}(\*x) } + \frac{ 1 - \lambda }{ Z_O^{\cF^*_S}(\*x) }
% } 
% \II( \*f_{\*x} \in \cA_O^{\cF^*_S} ) \right. 
% \right.
% \notag \\ 
% & \qquad \qquad \qquad \left. +
% \left.
% % \log 
% \rbr{
% \frac{ \lambda }{ Z_U^{\cF^*_S}(\*x) }
% }
% \II( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} )
% \right\}
% },
% \\ % ---
& 
= \EE_{\cF^*, \*f_{\*x}} 
% \sbr{
%\sbr{
\bigl[
\log
\bigl\{
% \rbr{ 
% \frac{ \lambda }{ Z_U^{\cF^*_S}(\*x) } + \frac{ 1 - \lambda }{ Z_O^{\cF^*_S}(\*x) }
% } 
\zeta_\lambda^{\cF^*_S}(\*x)
\II( \*f_{\*x} \in \cA_O^{\cF^*_S} ) 
%\right. 
%\right.
%\notag \\ 
% & \qquad \qquad \qquad \left. +
% \left.
% \log 
% \rbr{
% \frac{ \lambda }{ Z_U^{\cF^*_S}(\*x) }
% }
\notag \\
& \qquad \qquad \qquad
+ \eta_\lambda^{\cF^*_S}(\*x)
\II( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} )
\bigr\}
\bigr]
% }
,
%},
\label{eq:VLB-lambda}
\end{align}
% ただし，$\II$ を指示関数とする．
% where $\II$ is the indicator function.
where 
$\zeta_\lambda^{\cF^*_S}(\*x) = \frac{ \lambda }{ Z_U^{\cF^*_S}(\*x) } + \frac{ 1 - \lambda }{ Z_O^{\cF^*_S}(\*x) }$, 
$\eta_\lambda^{\cF^*_S}(\*x) = \frac{ \lambda }{ Z_U^{\cF^*_S}(\*x) }$, 
and
$\II$ is the indicator function.
%
%
% 混合比 $\lambda$ はこの変分下限を最大化して推定することができる：
Importantly, the weight parameter $\lambda$ can be estimated by maximizing the lower bound: 
\begin{align}
\max_{\lambda \in (0,1]} 
 % L(\*x, \lambda)
 \rm{LB}(\*x, \lambda)
\label{eq:MaxVLB}
\end{align}
% \eq{eq:VLB-q}より
% \scalebox{0.8}{$\mr{MI}(\*f_{\*x} ; \cF^*) = L(\*x, \lambda) + \EE_{\cF^*} \sbr{ D_{\mr{KL}}\rbr{ p(\*f_{\*x} \mid \cF^*) \parallel q_{\lambda}(\*f_{\*x} \mid \cF^*) } }$}
% であるため，
% $\max_{\lambda \in (0,1]} L(\*x, \lambda)$ 
% は 
% \scalebox{0.8}{$\min_{\lambda} \EE_{\cF^*} \sbr{ D_{\mr{KL}}\rbr{ p(\*f_{\*x} \mid \cF^*) \parallel q_{\lambda}(\*f_{\*x} \mid \cF^*) }}$} を考えることと等価である．
% %
% つまり，真の $p(\*f_{\*x} \mid \cF^*)$ とのKLダイバージェンスの最小化を試みていると解釈できる（これはvariational lower boundでよく使われるtrickである \citep{Bishop2023-deep}）．
% %
% \citep{Takeno2022-Sequential}は $\mr{MI}$ の下限について非負性を保証していたが，\eq{eq:MaxVLB}も非負性を保証することができる（導出はAppendixに記述する）．
%
% この下限最大化について，variational lower boundでよく使われるtrick\citep{Bishop2023-deep}により以下の性質が得られる． 
This maximization implies the following property, which is a well-known advantage of the variational lower bound maximization \citep{Bishop2023-deep}:
%
% --------------------------------------------------
% Remark: Variational approx.
% --------------------------------------------------
\begin{rema}
% 式\eq{eq:VLB-q}より
From \eq{eq:VLB-q}, 
\begin{align*}
 \mr{MI}(\*f_{\*x} ; \cF^*) = &
 % L(\*x, \lambda) 
 \mr{LB}(\*x, \lambda) 
 \\
 & + \EE_{\cF^*} \sbr{ D_{\mr{KL}}\rbr{ p(\*f_{\*x} \mid \cF^*) \parallel q_{\lambda}(\*f_{\*x} \mid \cF^*) } }. 
\end{align*}
% \scalebox{0.8}{
% $\mr{MI}(\*f_{\*x} ; \cF^*) = L(\*x, \lambda) + \EE_{\cF^*} \sbr{ D_{\mr{KL}}\rbr{ p(\*f_{\*x} \mid \cF^*) \parallel q_{\lambda}(\*f_{\*x} \mid \cF^*) } }$}
% のため，式\eq{eq:MaxVLB}
% $\max_{\lambda \in (0,1]} L(\*x, \lambda)$ 
% は 
%\scalebox{0.85}{$\min_{\lambda \in (0,1]} \EE_{\cF^*} \sbr{ D_{\mr{KL}}\rbr{ p(\*f_{\*x} \mid \cF^*) \parallel q_{\lambda}(\*f_{\*x} \mid \cF^*) }}$} を考えることと等価である．
Therefore, \eq{eq:MaxVLB} is equivalent to 
\begin{align*}
 % \scalebox{0.85}{
 \min_{\lambda \in (0,1]} \EE_{\cF^*} \sbr{ D_{\mr{KL}}\rbr{ p(\*f_{\*x} \mid \cF^*) \parallel q_{\lambda}(\*f_{\*x} \mid \cF^*) }}.
 % }. 
\end{align*}
%
% つまり，真の $p(\*f_{\*x} \mid \cF^*)$ と$q_\lambda$のKLダイバージェンスの最小化を試みていると解釈できる．
As a result, \eq{eq:MaxVLB} can be seen as the minimization of difference between true $p(\*f_{\*x} \mid \cF^*)$ and $q_\lambda$. 
%（これはvariational lower boundでよく使われるtrickである \citep{Bishop2023-deep}）． 
\end{rema}
%
% \vspace{.5em}
%
% さらに，以下の性質が成立する．
Further, we have the following property: 
% --------------------------------------------------
% Remark: PI and Positivity 
% --------------------------------------------------
\begin{rema}
 \label{rem:lower-bound-of-VLB}
 % 式\eq{eq:MaxVLB}は以下のように下から抑えられる（証明はAppendix~\ref{app:lower-bound-of-VLB}に示す）．
 \eq{eq:MaxVLB} can be bounded from below (the proof is in Appendix~\ref{app:lower-bound-of-VLB}): 
 \begin{align*}  
 \max_{\lambda \in (0,1]} 
  % L(\*x, \lambda) 
  \mr{LB}(\*x, \lambda) 
  \geq
 \EE_{\cF^*}\sbr{ p( \*f_{\*x} \notin \cA_U^{\cF_S^*}) }
 > 0. 
 \end{align*}
 %
 % $p( \*f_{\*x} \notin \cA_U^{\cF_S^*} )$
 % は$\*f_{\*x}$が$\cA_U^{\cF_S^*}$と比べてパレートフロンティアを改善する確率であり，
 % $\EE_{\cF^*}\sbr{ p( \*f_{\*x} \notin \cA_U^{\cF_S^*}) }$
 % はある種のPI (Probability of Improvement) の期待値だと解釈できる．
 $p( \*f_{\*x} \notin \cA_U^{\cF_S^*} )$
 can be seen as the probability of improvement (PI) from the region $\cA_U^{\cF_S^*}$, from which positivity of \eq{eq:MaxVLB} is also directly derived. 
 %
 % また，下限\eq{eq:MaxVLB}が正であることもそこから直ちに導かれる．
\end{rema}
%
% \vspace{.5em}
%
% PIとの関係性はこれまで単一目的関数でのMax-value Entropy Search\citep{Wang2017-Max}やその制約付きベイズ最適化拡張\citep{Takeno2022-Sequential}でも指摘されてきた性質である．
%
% Max-value Entropy Search\citep{Wang2017-Max}の多目的拡張\citep{Suzuki2020-multi,Qing2022-text}においてMIの近似指標のpositivityは示されてこなかった．
%
% 一般にMIは非負のため$0$は自明な下界であるが，このremarkは\eq{eq:MaxVLB}が常に自明な下界よりは大きなものであることを保証している．
While MI has a trivial lower bound $0$ in general, this remark guarantees that \eq{eq:MaxVLB} is a larger lower bound than this trivial bound. 
%
% また，PIで下から抑えられているため，PIの意味で有望な点に対しては0より実質的に大きな値を持つこともわかる．
Further, we can also see that if the candidate $\*x$ is promising in a sense of PI, \eq{eq:MaxVLB} should have substantially larger value than $0$. 


% 結果的に，$\mr{MI}(\*f_{\*x} ; \cF^*)$ の下限\eq{eq:MaxVLB}を最大化する $\*x$ の選択は
As a result, the selection of $\*x$ is formulated as 
\begin{align*}
 \max_{\*x, \lambda \in (0,1]} 
 % L(\*x, \lambda),  
 \mr{LB}(\*x, \lambda),  
\end{align*}
% と書くことができる．
%
% $\*x$ と $\lambda$ の最適化は同時に行なうことができることに注意されたい．
in which $\*x$ and $\lambda$ can be simultaneously optimized ($(d + 1)$-dimensional maximization).
%
% つまり，シンプルに$d + 1$ 次元の最大化問題として扱うことができる．
%
% 一方で，各$\*x$に対して$\lambda$に関する最大化\eq{eq:MaxVLB}を行う実装も考えられる．
%
% この場合は$L(\*x, \lambda)$が$\lambda$については上に凸であることを考慮すると効率的に計算できる．

% --------------------------------------------------
\subsection{Computations}
% \subsection{計算方法}
\label{ssec:computations}

% 式\eq{eq:VLB-lambda}の $L(\*x, \lambda)$ の期待値はモンテカルロサンプリングで以下のように近似する：
We employ the Monte-Carlo (MC) estimation to calculate the expectation in 
% $L(\*x, \lambda)$: 
$\mr{LB}(\*x, \lambda)$: 
\begin{align}
\mr{LB}(\*x, \lambda) 
% L(\*x, \lambda) 
&\approx 
\frac{1}{K} \sum_{(\tilde{\cF}^*_S, \tilde{\*f}) \in F}
\log
\left\{
% \rbr{ 
% \frac{ \lambda }{ Z_U^{\tilde{\cF}^*_S}(\*x) } + \frac{ 1 - \lambda }{ Z_O^{\tilde{\cF}^*_S}(\*x) }
% } 
\zeta_\lambda^{\tilde{\cF}^*_S}(\*x)
\II( \tilde{\*f_{\*x}} \in \cA_O^{\tilde{\cF}^*_S} ) 
\right.
\nonumber \\
& \qquad \qquad \qquad +
% \log 
\left.
% \rbr{
% \frac{ \lambda }{ Z_U^{\tilde{\cF}^*_S}(\*x) }
% }
\eta_\lambda^{\tilde{\cF}^*_S}(\*x)
\II( \tilde{\*f}_{\*x} \in \cA_{U \setminus O}^{\tilde{\cF}^*_S} )
\right\}, 
% \frac{1}{K} \sum_{(\tilde{\cF}^*_S, \tilde{\*f}) \in F}
% \log\rbr{ 
% \frac{ \lambda }{ Z_U^{\tilde{\cF}^*_S}(\*x) } + \frac{ 1 - \lambda }{ Z_O^{\tilde{\cF}^*_S}(\*x) }
% } 
% \II( \tilde{\*f_{\*x}} \in \cA_O^{\tilde{\cF}^*_S} ) \nonumber \\
% & \qquad +
% \log \rbr{
% \frac{ \lambda }{ Z_U^{\tilde{\cF}^*_S}(\*x) }
% }
% \II( \tilde{\*f}_{\*x} \in \cA_{U \setminus O}^{\tilde{\cF}^*_S} ), 
\label{eq:LB-MC}
\end{align}
% ただし，$F$ をサンプリングした $(\cF^*_S, \*f)$ の組の実現値 $(\tilde{\cF}^*_S, \tilde{\*f})$ の集合，サンプリング回数 $K = |F|$ とする．
where $F$ is a set of sampled pairs of $(\cF^*_S, \*f)$, for which a sample pair is denoted as
$(\tilde{\cF}^*_S, \tilde{\*f})$, and $K = |F|$ is the number of samples.
%
% 以降，` $\tilde{}$ 'が付いている変数は確率変数に対してサンプリングされた実現値とする．
Henceforth, variables with ` $\tilde{}$ ' indicate sampled values.
%
% $\cF^*_S$ のサンプルを得る方法は過去の情報論的ベイズ最適化で採用されてきた方法と同じ方法が利用できる\citep{Suzuki2020-multi,Hernandez-lobatoa2016-Predictive}．
For $\cF^*_S$, the same sampling strategy can be used as existing information-theoretic MOBO methods \citep{Suzuki2020-multi,Hernandez-lobatoa2016-Predictive}, in which a sample path
$\tilde{f}^l$
is approximately generated by using random feature map (RFM) \citep{Rahimi2008-Random}. 
% 
% これらの手法では，random feature map（RFM）\citep{Rahimi2008-Random}を用いて，現在のガウス過程回帰をベイズ線形モデル $\*w_l^\top \phi(\*x)$ で近似する．
%
% ただし，$\*w_l \in \RR^D$ は $l$ 番目の目的関数に対するパラメータベクトルであり，$\phi: \cX \rightarrow \RR^D$ は予め定義された基底ベクトルである．
%
% $\*w_l$ の事後分布から $\tilde{\*w}_l$ を生成することで，関数のサンプル $\tilde{f}^l(\*x) \approx \tilde{\*w}_l^\top \phi(\*x)$ を得ることができる．
%
% パレートフロンティアのサンプル $\cF^*_S$ は，$l = 1, \ldots, L$ に対して $\tilde{\*w}_{l}^\top \phi(\*x)$ を最大化する多目的最適化を解くことで得られる．
We obtain $\cF^*_S$ by solving the MOO maximizing sampled
$\tilde{f}^l(\*x)$ 
for 
$l = 1, \ldots, L$.
%
% この最大化には，NSGA-II \citep{Deb2002-Fast}のような一般的な多目的最適化アルゴリズムを用いることができる．
This maximization can be performed by general MOO solvers such as the well-known NSGA-II \citep{Deb2002-Fast}.
%
% NSGA-IIの場合，近似パレートフロンティアのサイズ $|\cF^*_S|$ を指定することができる（典型的には100未満）．
In the case of NSGA-II, $|\cF^*_S|$ can be specified, typically less than $100$.
%
% $(\tilde{\cF}^*_S, \tilde{\*f})$ は同時分布からのサンプルだが，$\tilde{\cF}^*_S$ を得る際に使った $\tilde{\*w}_l^\top \phi(\*x)$ を $\tilde{\*f}$ とすればよい．
% The pair $(\tilde{\cF}^*_S, \tilde{\*f})$ is a sample from the joint distribution
%
% $Z_O^{\tilde{\cF}^*_S}, Z_U^{\tilde{\cF}^*_S}$ は領域 $\cA_O^{\tilde{\cF}^*_S}$ や $\cA_U^{\tilde{\cF}^*_S}$ を矩形に分割することで非常に簡単な計算に帰着できる
% Computations of $Z_O^{\tilde{\cF}^*_S}$ and $Z_U^{\tilde{\cF}^*_S}$ can be easily performed by decomposing $\cA_O^{\tilde{\cF}^*_S}$ and $\cA_U^{\tilde{\cF}^*_S}$ into box regions, respectively (as shown by \citep{Suzuki2020-multi} for which details are in Appendix~\ref{app:CalcZ}).
Computations of $Z_O^{\tilde{\cF}^*_S}$ and $Z_U^{\tilde{\cF}^*_S}$ can be easily performed by the cell (hyper-rectangle) decomposition-based approach as shown by \citep{Suzuki2020-multi} for which details are in Appendix~\ref{app:CalcZ}.
% decomposing $\cA_O^{\tilde{\cF}^*_S}$ and $\cA_U^{\tilde{\cF}^*_S}$ into box regions, respectively (as shown by \citep{Suzuki2020-multi} for which details are in Appendix~\ref{app:CalcZ}).
%
% （
% これはPFES\citep{Suzuki2020-multi}で示された方法をそのまま使うことができる\remove{．
% %
% 詳細はAppendix~\ref{app:CalcZ}に記述する}
%）．
%
% 分割は各 $\tilde{\cF}_S^*$ につき1回行えばすべての $\*x$ で使い回すことができる．
This decomposition is only required once for each iteration of BO because it is common for all candidate $\*x$.



We also consider another way to numerically approximate 
% $L(\*x,\lambda)$ 
$\mr{LB}(\*x,\lambda)$ 
based on the following transformation: 
% $L(\*x,\lambda)$ は期待値 $\EE_{\cF^*, \*f_{\*x}}$ を $\EE_{\cF^*} \EE_{\*f_{\*x} \mid \cF^*}$ と書き換えると以下のように表現することもできる：
% By replacing 
% $\EE_{\cF^*, \*f_{\*x}}$ in $L(\*x,\lambda)$ 
% with 
% $\EE_{\cF^*} \EE_{\*f_{\*x} \mid \cF^*}$,
% we can rewrite 
{\small
\begin{align}
% & L(\*x,\lambda) 
& \mr{LB}(\*x,\lambda) 
\notag \\
& \! = \!
\EE_{\cF^*, \*f_{\*x}} \!
\sbr{
\II( \*f_{\*x} \in \cA_O^{\cF^*_S} ) 
\log
% \rbr{ 
% \frac{ \lambda }{ Z_U^{\cF^*_S}(\*x) } + \frac{ 1 - \lambda }{ Z_O^{\cF^*_S}(\*x) }
% } 
\zeta_\lambda^{\tilde{\cF}^*_S}(\*x)
% \right. 
% \notag \\ 
% & \qquad \qquad \qquad \left. 
\! + \!
\II( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} )
\log 
% \rbr{
% \frac{ \lambda }{ Z_U^{\cF^*_S}(\*x) }
% }
\eta_\lambda^{\tilde{\cF}^*_S}(\*x)
}
% \label{eq:} 
\notag
\\ %--
& = \EE_{\cF^*} \left[
p(\*f_{\*x} \in \cA_O^{\cF^*_S} \mid \cF^*) 
\log
% \rbr{ 
% \frac{ \lambda }{ Z_U^{\cF^*_S}(\*x) } + \frac{ 1 - \lambda }{ Z_O^{\cF^*_S}(\*x) }
% } 
\zeta_\lambda^{\tilde{\cF}^*_S}(\*x)
\right.
\notag \\
& \qquad \qquad \qquad \left. 
+ p(\*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} \mid \cF^*) 
\log 
% \rbr{
% \frac{ \lambda }{ Z_U^{\cF^*_S}(\*x) }
% }
\eta_\lambda^{\tilde{\cF}^*_S}(\*x)
% } 	
\right]
\notag \\ % --
& \approx
% \frac{1}{K} \sum_{\tilde{\cF}^*_S \in F_{\rm PF}}
\frac{1}{K} \sum_{(\tilde{\cF}^*_S, \tilde{\*f}) \in F}
p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{\cF}^*) 
\log
% \rbr{ 
% \frac{ \lambda }{ Z_U^{\tilde{\cF}^*_S}(\*x) } + \frac{ 1 - \lambda }{ Z_O^{\tilde{\cF}^*_S}(\*x) }
% } 
\zeta_\lambda^{\tilde{\cF}^*_S}(\*x)
\notag \\
& \qquad \qquad 
+ p(\*f_{\*x} \in \cA_{U \setminus O}^{\tilde{\cF}^*_S} \mid \tilde{\cF}^*) \log 
% \rbr{
% \frac{ \lambda }{ Z_U^{\tilde{\cF}^*_S}(\*x) }
% }
\eta_\lambda^{\tilde{\cF}^*_S}(\*x).
\label{eq:LB-MC-2}
\end{align}}%
% where $F_{\rm PF}$ is a set of sampled $\tilde{\cF}^*_S$ (extract only $\tilde{\cF}^*_S$ from $F$). 
%
Note that the second line is from 
$\II( \*f_{\*x} \in \cA_O^{\cF^*_S} ) = 1 - \II( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} )$, and the third line is obtained by replacing 
$\EE_{\cF^*, \*f_{\*x}}$ %in $L(\*x,\lambda)$ 
with 
$\EE_{\cF^*} \EE_{\*f_{\*x} \mid \cF^*}$.
% ただし，$F_{\rm PF}$ はサンプリングした $\tilde{\cF}^*_S$ の集合とする（$F$ のうち $\tilde{\cF}^*_S$ だけから作った集合）．
%
% この式を\eq{eq:LB-MC}と比べると，\eq{eq:LB-MC}は 
% $p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{\cF}^*) \approx \II( \tilde{\*f}_{\*x} \in \cA_O^{\tilde{\cF}^*_S} )$ 
% および 
% $p(\*f_{\*x} \in \cA_{U \setminus O}^{\tilde{\cF}^*_S} \mid \tilde{\cF}^*) \approx \II( \tilde{\*f}_{\*x} \in \cA_{U \setminus O}^{\tilde{\cF}^*_S} )$ 
% という1サンプルのみでの近似を行なっていると解釈できる
Since \eq{eq:LB-MC}
% Comparing \eq{eq:LB-MC-2} with \eq{eq:LB-MC}, which 
can be rewritten as 
$\frac{1}{K} \sum_{(\tilde{\cF}^*_S, \tilde{\*f}) \in F}
\II( \tilde{\*f_{\*x}} \in \cA_O^{\tilde{\cF}^*_S} ) 
\log
\zeta_\lambda^{\tilde{\cF}^*_S}(\*x)
+ 
\II( \tilde{\*f}_{\*x} \in \cA_{U \setminus O}^{\tilde{\cF}^*_S} )
\log
\eta_\lambda^{\tilde{\cF}^*_S}(\*x) 
$,
by comparing this re-written expression with \eq{eq:LB-MC-2},
%
%Comparing this with \eq{eq:LB-MC}, 
we can interpret that \eq{eq:LB-MC} performs one-sample approximations
$p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{\cF}^*) \approx \II( \tilde{\*f}_{\*x} \in \cA_O^{\tilde{\cF}^*_S} )$ 
and 
$p(\*f_{\*x} \in \cA_{U \setminus O}^{\tilde{\cF}^*_S} \mid \tilde{\cF}^*) \approx \II( \tilde{\*f}_{\*x} \in \cA_{U \setminus O}^{\tilde{\cF}^*_S} )$.
% \footnote{
% % 注釈として 
% \parbox{.4\tw}{
% $p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{\cF}^*)$ の条件部の $\tilde{\cF}^*$ 
% はパレートフロンティア全体のサンプルに相当するが，指示関数でのサンプル近似
% $\II( \tilde{\*f}_{\*x} \in \cA_O^{\tilde{\cF}^*_S} )$
% には $\tilde{\cF}^*$ が明示的には必要ないことに注意されたい（暗黙のうちに定まっている $\tilde{\cF}^*$ に対して 
% $\tilde{\*f}_{\*x} \in \cA_O^{\tilde{\cF}^*_S}$ 
% を評価している）．}}. 
%
% 式\eq{eq:LB-MC}は $K \rightarrow \infty$ で真の下限\eq{eq:VLB-lambda}には収束するものの，$[0,1]$ の確率である 
%$p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{\cF}^*), p(\*f_{\*x} \in \cA_{U \setminus O}^{\tilde{\cF}^*_S} \mid \tilde{\cF}^*)$ 
%に対して $0$ か $1$ の極端な値を与えるため小さな $K$ ではばらつきが大きい可能性がある．
%
% そこで，
% $p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{\cF}^*)$, 
% $p(\*f_{\*x} \in \cA_{U \setminus O}^{\tilde{\cF}^*_S} \mid \tilde{\cF}^*)$ 
% の推定に事前知識を導入し，ベイズMAP (maximum a posteriori) を用いることでばらつきを低減することを考える．
We consider improving this approximations by introducing prior knowledge about 
$p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{\cF}^*)$
and
$p(\*f_{\*x} \in \cA_{U \setminus O}^{\tilde{\cF}^*_S} \mid \tilde{\cF}^*)$.
% を推定する


% $\cA_O^{\tilde{\cF}^*_S}$ と $\cA_{U \setminus O}^{\tilde{\cF}^*_S}$ 
% は互いに素であり，
% $p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{\cF}^*) + p(\*f_{\*x} \in \cA_{U \setminus O}^{\tilde{\cF}^*_S} \mid \tilde{\cF}^*) = 1$ 
% である．
%
% ここで，$\theta \coloneqq p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{\cF}^*)$ 
% とする．
Let $\theta \coloneqq p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{\cF}^*)$.
%
% $\theta$
% は
% $\theta 
% \approx p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \*f_{\*x} \preceq \tilde{\cF}^*) 
% \approx p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \*f_{\*x} \in \cA_U^{\tilde{\cF}^*_S}) 
% = Z_O^{\tilde{\cF}^*_S}(\*x) / Z_U^{\tilde{\cF}^*_S}(\*x) 
% \eqqcolon \hat{p}$ 
% のように近似できる
We use an approximation
$\theta 
% \approx p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \*f_{\*x} \preceq \tilde{\cF}^*) 
\approx p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \*f_{\*x} \in \cA_U^{\tilde{\cF}^*_S}) 
= Z_O^{\tilde{\cF}^*_S}(\*x) / Z_U^{\tilde{\cF}^*_S}(\*x) 
\eqqcolon \hat{p}$ 
as our prior knowledge. 
%
% 1つ目の近似はPFTNによる切断近似であり，2つ目の近似は手に入らない $\tilde{\cF}^*$ の代わりに，
% $\*f_{\*x} \in \cA_U^{\tilde{\cF}^*_S}$ 
% という条件を使ったものである．
The approximation is replacement of the conditioning by 
$\tilde{\cF}^*$ 
with the under-truncation
$\*f_{\*x} \in \cA_U^{\tilde{\cF}^*_S}$.
%
Note that $Z_O^{\tilde{\cF}^*_S}(\*x)$ and $Z_U^{\tilde{\cF}^*_S}(\*x)$ are required even in the na\"ive MC \eq{eq:LB-MC}, $\hat{p}$ can be obtained without additional computations.
% $Z_O^{\tilde{\cF}^*_S}(\*x)$，$Z_U^{\tilde{\cF}^*_S}(\*x)$ 
% は獲得関数には必ず必要なので $\hat{p}$ は追加的なコストなく計算できる．
%
% 近似値 $\hat{p}$ をピークに持つような事前分布を $\theta$ の推定に導入する．
A prior distribution having the mode at $\hat{p}$ is introduced to estimate $\theta$.
%
% $\hat{p}$ に中央値を持つようなベータ分布を $\theta$ の事前分布に設定し，$\theta$ のMAPを求めると
We use the beta distribution by which MAP (maximum a posteriori) becomes
\begin{align*}
\theta_{\mr{MAP}}(\*f_{\*x}) = \frac{\hat{p} + \II(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S})}{2}.
\end{align*}
% となる．
%
% 導出の詳細はAppendix~\ref{app:BayesMAP}に記述する．
The detailed derivation is in Appendix~\ref{app:BayesMAP}.
%
% $\theta_{\mr{MAP}}$ は $\hat{p}$ と 
% $\II(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S})$ 
% の平均になっている．
$\theta_{\mr{MAP}}$ 
can be seen as an average of 
$\hat{p}$ 
and 
$\II(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S})$.


% $\VV_{\*f_{\*x} \mid \tilde{\cF}^*_S}[\theta_{\mr{MAP}}(\*f_{\*x})] = \VV_{\*f_{\*x} \mid \tilde{\cF}^*_S}[\II(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S})]/4$ 
% であるためこの項の分散が低減することがわかる．\red{(Memo:ここの議論もう少しちゃんとしたい)}
% %
% 代わりに近似値 $\hat{p}$ へバイアスするが，このモンテカルロ近似は通常は小サンプル（実験では$K = 10$をデフォルトとした．\citep{Wang2017-Max}など過去の情報論的なベイズ最適化手法でも同程度）であるため分散低減の恩恵が大きいことを経験的に観察している．
% 代わりに近似値 $\hat{p}$ へバイアスするが小サンプルのため分散低減の恩恵が大きい \red{($\hat{p}$ をそのまま使ったらどうなるのかと言われそう．何か問題があった気がする(常に $\lambda$ が極端な方に行くとか？)けど思い出せない)}．
%
% 結果的に $L(\*x,\lambda)$ の近似は
As a result, we obtain 
\begin{align}
% L(\*x,\lambda) 
\mr{LB}&(\*x,\lambda) 
\approx 
\frac{1}{K} \sum_{(\tilde{\cF}^*_S, \tilde{\*f}) \in F}
\theta_{\mr{MAP}}(\tilde{\*f}_{\*x}) 
\log \zeta_\lambda^{\tilde{\cF}^*_S}(\*x)
\nonumber
\\
& % \qquad  \qquad 
+
(1 - \theta_{\mr{MAP}}(\tilde{\*f}_{\*x}))
\log \eta_\lambda^{\tilde{\cF}^*_S}(\*x) 
\eqqcolon \wh{\mr{LB}}(\*x,\lambda).
% \frac{1}{K} \sum_{(\tilde{\cF}^*_S, \tilde{\*f}) \in F}
% \log
% \rbr{ 
% \frac{ \lambda }{ Z_U^{\tilde{\cF}^*_S}(\*x) } + \frac{ 1 - \lambda }{ Z_O^{\tilde{\cF}^*_S}(\*x) }
% } 
% \theta_{\mr{MAP}}(\tilde{\*f}_{\*x}) \nonumber \\
% & \qquad +
% \log \rbr{
% \frac{ \lambda }{ Z_U^{\tilde{\cF}^*_S}(\*x) }
% }
% (1 - \theta_{\mr{MAP}}(\tilde{\*f}_{\*x})).
\label{eq:LB-MAP}
\end{align}
% となる．
% \red{(Memo: 忘れたが $\lambda$ に関して上に凸ではなかったか？もしそうならどこかで言及)}
% $\VV_{\*f_{\*x} \mid \tilde{\cF}^*_S}[\theta_{\mr{MAP}}(\*f_{\*x})] = \VV_{\*f_{\*x} \mid \tilde{\cF}^*_S}[\II(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S})]/4$ 
% であるためこの項の分散が低減することがわかる．\red{(Memo:ここの議論もう少しちゃんとしたい)}
% %
% 事前知識を用いたことで，推定量のばらつきが軽減することを経験的に確認している．
We empirically observe that the estimation variance can be improved by the prior.
%
% 代わりに近似値 $\hat{p}$ へバイアスするが，このモンテカルロ近似は通常は小サンプル（実験では$K = 10$をデフォルトとした．\citep{Wang2017-Max}など過去の情報論的なベイズ最適化手法でも同程度）であるため分散低減の恩恵が大きい．
Instead, the bias to $\hat{p}$ can occur, but because the number of samples is usually small (our default setting is $K = 10$ in the experiments, which is same as existing information-theoretic BO studies such as \citep{Wang2017-Max}), variance reduction has a stronger benefit in practice. 
%
% \remove{
% 推定量のばらつき，精度に関する解析的，実験的考察を\red{Appendix~\ref{app:}}に記述する．}
Further discussion on the accuracy of this estimator is in Appendices~\ref{app:variance-BayesMAP} and \ref{app:empirical-study-BayesMAP}.


% PFEVの手続きをAlgorithm~\ref{alg:PFEV}に示す．
The procedure of PFEV is shown in Algorithm~\ref{alg:PFEV}.
%
% $Z_U^{\tilde{\cF}_S}$
% 及び
% $Z_O^{\tilde{\cF}_S}$
% の計算はPFESで示された矩形分割に基づく方法で計算できるため，理論上の計算複雑性はPFESとほぼ同じである．
% Since
% $Z_U^{\tilde{\cF}_S}$
% and
% $Z_O^{\tilde{\cF}_S}$
% can be computed by the cell-based decomposition approach employed in PFES (see Appendix~\ref{app:CalcZ}), computational complexity of PFEV is similar to PFES.
% %
% 簡単のため
% $A_O^{\tilde{\cF}_S^*}$ および $A_U^{\tilde{\cF}_S^*}$ の
% 矩形分割の数を $C$ とする．
%
% ガウス過程の事後分布の $\*\mu(\*x)$，$\*\sigma(\*x)$ が計算済みであり，$F$ がサンプル済みであるとすると，この時，獲得関数\eq{eq:LB-MAP}の計算量は $O(K C L)$ となる．
Assume that we already have the posterior mean and variance of the GPs.
%
Then, computations of \eq{eq:LB-MAP} is $O(K C L)$, where $C$ is the number of hyper-rectangle cells in the decomposition.
%  of
For the cell decomposition, we employ the quick hypervolume (QHV) algorithm \citep{Russo2014-quick} as indicated by \citep{Suzuki2020-multi}.
% $A_O^{\tilde{\cF}_S^*}$ 
% and 
% $A_U^{\tilde{\cF}_S^*}$.
%
% $F$ のサンプリングにはRFMの次元 $D$ に対して $O(D^3)$ とNSGA-IIのコストがかかる（ただし，すでに述べたようにこれは各繰り返しに1度だけでよい）．
Sampling of $F$ requires $O(D^3)$ for RFM with $D$ basis functions and the cost of NSGA-II is also required.
%
% \citep{Suzuki2020-multi}が報告した通り，実践的にはNSGA-IIにかかるコストが大きくなりやすく，相対的には下限計算が占める割合は小さい．
% As reported by \citep{Suzuki2020-multi}, the computational cost of NSGA-II is dominant in practice and the cost of the lower bound calculation is relatively small.
We empirically see that, for small $L$, the computational cost of NSGA-II is dominant, and for large $L$, QHV becomes dominant, both of which are commonly required for several information-theoretic MOBO \citep{Suzuki2020-multi,Qing2022-text,Tu2022-joint}.
%
Compared with them, the practical cost of the lower bound calculation in \text{CalcPFEV} of Algorithm~\ref{alg:PFEV} is often relatively small (see Appendix~\ref{app:time} for details).
% \ref{ssec:VLBMaximization}節の最後に述べた通り，獲得関数最大化は$d+1$次元の問題として扱う．
As discussed in the end of Section~\ref{ssec:VLBMaximization}, the acquisition function maximization is formulated as $(d + 1)$-dimensional optimization (line 10 of Algorithm~\ref{alg:PFEV}). 
%
% 一方で，各$\*x$に対して$\lambda$に関する内側の一次元最大化を行う実装も考えられる．
On the other hand, it is also possible to optimize $\lambda$ for each given $\*x$ as an inner one-dimensional optimization.
%
% この場合は式\eq{eq:LB-MAP}(または\eq{eq:LB-MC})が$\lambda$について上に凸であることを考慮すると効率的に計算できる（\replace{Appendix~\ref{app:lambda-convexity}参照}{凸性は$2$階微分から簡単に確かめられる}）．
In the latter case, efficient computations can be performed by considering \eq{eq:LB-MAP} (or \eq{eq:LB-MC}) is concave with respect to $\lambda$.
% (Details are in Appendix~\ref{app:lambda-convexity}).
%
Further, we can show that the maximizer of $\lambda$ exists though the candidate $\lambda$ is defined as a left open interval $(0,1]$. 
%
Details of these discussions about the maximization problem of $\lambda$ are shown in Appendix~\ref{app:lambda-convexity}.



% --------------------------------------------------
% Algorithm: PFEV
% --------------------------------------------------
\setlength{\textfloatsep}{10pt}
\begin{algorithm}[t]
\caption{Pseudo-code of PFEV}
\label{alg:PFEV}
\begin{algorithmic}[1]
      % \SetAlgoVlined
      % \Procedure{PFEV}{Initial dataset $\cD_0$}
%      \FUNCTION{PFEV}{Initial dataset $\cD_0$}
      \STATE \textbf{Function} \textsc{PFEV}( Initial dataset $\cD_0$ ):
      \FOR{$t = 0, \ldots, T$}
      \STATE $F \leftarrow \{\}$
      \FOR{$k = 1, \ldots, K$}
      \STATE Generate a sample path $\tilde{\*f}$ from the current posterior of $\*f$
      \STATE Obtain $\tilde{\cF}_S^*$ by applying NSGA-II to $\tilde{\*f}_{\*x}$ 
      \STATE Create cell-decomposition by QHV
      \STATE $F \leftarrow F \cup (\tilde{\cF}_S^*, \tilde{\*f})$
      \ENDFOR
      \STATE $(\*x_{t+1}, \lambda_{t+1}) \leftarrow \argmax_{\*x, \lambda} \textsc{CalcPFEV}(\*x, \lambda ; F)$
      \STATE Evaluate $\*f_{\*x_{t+1}}$ and observe $\*y_{t+1}$
      \STATE $\cD_{t+1} \leftarrow \cD_{t} \cup (\*x_{t+1}, \*y_{t+1})$
      \ENDFOR
%      \ENDFUNCTION
      % --------------------------------------------------
%      \FUNCTION{CalcPFEV}{$\*x, \lambda ; F$}
      \STATE \textbf{Function} \textsc{CalcPFEV}( $\*x, \lambda ; F$ ):
      \STATE Calculate $Z_O^{\tilde{F}^*_S}(\*x), Z_U^{\tilde{F}^*_S}(\*x)$, and $\II(\tilde{\*f}_{\*x} \in \cA_O^{\tilde{F}^*_S})$ for $(\tilde{\cF}_S^*, \tilde{\*f}) \in F$
      \STATE {\bf return} Approximate lower bound \eq{eq:LB-MAP}
%      \ENDFUNCTION
\end{algorithmic}
\end{algorithm}



% --------------------------------------------------
% \section{関連研究}
\section{Related Work}
\label{sec:related-work}
% --------------------------------------------------
% \red{前半部分（MESMOまで）がPFES論文そのまますぎるので修正すべき．可能であれば，多目的ベイズ最適化の最近の(2020$\sim$2024頃の)論文も入れたい}

% MOBOにはさまざまな方法が提案されてきた．
For MOBO, a variety of approaches have been proposed, typically by extending single-objective acquisition function such as expected improvement and upper confidence bound \citep[e.g.,][]{Emmerich2005-single,Shah2016-pareto,Zuluaga2016-pal,daulton20differentiable,ament2023unexpected}.
% 
Information-theoretic approaches \citep[e.g.,][]{Hernandez-lobatoa2016-Predictive,Belakaria2019-max} also have been extended from its counterpart of the single-objective BO \citep{Henning2012-Entropy,Hernandez2014-Predictive,Wang2017-Max}. 
% information theoreticな方法は初めsingle-objectiveからmulti-objectiveへ拡張
% 中でも提案法と最も関連が深い手法はPFES\citep{Suzuki2020-multi}である．
Among these, the most closely related method to the proposed method is PFES \citep{Suzuki2020-multi}.
%
% PFESは情報論的ベイズ最適化\citep{Henning2012-Entropy,Hernandez2014-Predictive}の中でも，最適値$\max_{\*x} f(\*x)$に関する情報利得を考えるアプローチ\citep{Wang2017-Max}の多目的拡張だと考えることができる．
PFES can be seen as a multi-objective extension of the max value based information-theoretic BO, called max-value entropy search (MES) \citep{Wang2017-Max}.
%
% PFESとそれ以前の情報論的多目的手法\citep{Hernandez-lobatoa2016-Predictive,Belakaria2019-max}やその他のアプローチ（例えば標準的な期待改善量のパレート超体積拡張\citep{Emmerich2005-single}などがある）との関連は\citep{Suzuki2020-multi}が詳しくReviewしているためそちらを参照されたい．
Information-theoretic MOBO before PFES and other approaches are reviewed in \citep{Suzuki2020-multi}. 
%
% ここでは，PFES以降の情報論的な多目的ベイズ最適化の中で提案法と関連の深いものについて述べる．
Here, we mainly focus on information-theoretic MOBO methods after PFES.
%
% \remove{その他の関連研究はAppendix~\ref{}にも述べる．}
% Other related work including other information theoretic methods to single-objective problems (e.g., \citep{Henning2012-Entropy,Hernandez2014-Predictive}) and other criteria are discussed in Appendix~\ref{app:related-work}.
A more comprehensive related work including other information-theoretic methods and other criteria are discussed in Appendix~\ref{app:related-work}.



% PFTNによるMI近似はPFESが初めて導入したものである．
The MI approximation with PFTN was first introduced by PFES.
%
% ただし，MIの計算はエントロピーの差分に基づく古典的な方法\citep{Wang2017-Max}であり下限ではない．
On the other hand, the MI approximation is based on a decomposition into difference of the entropy, which is a classical approach in information-theoretic BO \citep{Hernandez2014-Predictive}.
%
% 制約付きベイズ最適化の文脈において，\citep{Takeno2022-Sequential}はエントロピーの差分と切断正規分布の組み合わせによるMI近似が負になる可能性を示し，これが致命的な不具合を起こし得ることを実証した．
In the context of constrained BO, \citet{Takeno2022-Sequential} revealed that the entropy difference based decomposition can cause a critical issue originated from a negative value of the MI approximation.
%
% PFESが非負性を持つかは現状明らかにされていない．
The positivity of PFES has not been clarified.
%
% またPFESは過剰な切断のみ考えてPFTNを定義している．
Further, PFES only uses over-truncation (PFTN-O). 
%
% 過剰な切断では真の$\cF^*$での切断と比べて$\*f_{\*x}$の分布が大きく変化するため，$\cF^*$と$\*f_{\*x}$の依存関係を過大評価する可能性がある．
Therefore, effect of the truncation by $\cF^*$ on $\*f_{\*x}$ is overly estimated.



% PFES以降の情報論的アプローチに，$\cF^*$および対応する$\*x$の結合エントロピーを考えるJoint Entropy Search (JES) \citep{Tu2022-joint} が提案されたが，これも過剰な切断のみ考えることによるlimitationを引き継いでいる．
After PFES, Joint Entropy Search (JES) \citep{Tu2022-joint} was proposed in which the joint entropy of the optimal $\*x$ and $\cF^*$ is considered.
%
This approach is also only uses over-truncation. 
%
% MIの下限に基づくもう一つの方法としてParallel Feasible Pareto Frontier Entropy Search（$\{\text{PF}\}^{2}\text{ES}$）がある\citep{Qing2022-text}．
Another approach considering the lower bound of MI is Parallel Feasible Pareto Frontier Entropy Search ($\{\text{PF}\}^{2}\text{ES}$) \citep{Qing2022-text}, which also pointed out the problem of over-truncation.
%
% この手法もやはり過剰な切断のみに基づいている．
However, $\{\text{PF}\}^{2}\text{ES}$ is still based only on over-truncation.
%
A shifting parameter $\*\veps \in \RR^L$ of the Pareto-frontier is heuristically introduced to mitigate over-truncation, for which theoretical justification is not clarified.
% また下限であることが一般には証明されてない（実際には計算できない$|\mr{PF}| \to \infty$の極限で出力2次元の場合のみ証明が示されている）．
Further, their criterion is not guaranteed as a lower bound in general (only when $L = 2$ with the assumption $|\cF_S^*| \to \infty$).
%
% さらに，パレートフロンティアの位置をシフトするパラメータ$\*\veps \in \RR^L$が実践上ヒューリスティックに設定され理論的妥当性は不明である．



% --------------------------------------------------
\section{Discussion on Extensions}
\label{sec:extensions}


% --------------------------------------------------
% Fig: GP由来の人工関数実験 (d = 2 and 3)
% --------------------------------------------------
\begin{figure*}[t!]
\centering
\subfigure[$(d, L) = (2, 2)$]{
 \ig{.19}{./figs/GP-main/RHV_input_dim_2output_dim_2_length_scale_0.1.pdf}
} \hspace{-.5em}
\subfigure[$(d, L) = (2, 3)$]{
 \ig{.19}{./figs/GP-main/RHV_input_dim_2output_dim_3_length_scale_0.1.pdf}
} \hspace{-.5em}
\subfigure[$(d, L) = (2, 4)$]{
 \ig{.19}{./figs/GP-main/RHV_input_dim_2output_dim_4_length_scale_0.1.pdf}
} \hspace{-.5em}
\subfigure[$(d, L) = (2, 5)$]{
 \ig{.19}{./figs/GP-main/RHV_input_dim_2output_dim_5_length_scale_0.1.pdf}
} \hspace{-.5em}
\subfigure[$(d, L) = (2, 6)$]{
 \ig{.19}{./figs/GP-main/RHV_input_dim_2output_dim_6_length_scale_0.1.pdf}
}

\subfigure[$(d, L) = (3, 2)$]{
 \ig{.19}{./figs/GP-main/RHV_input_dim_3output_dim_2_length_scale_0.1.pdf}
} \hspace{-.5em}
\subfigure[$(d, L) = (3, 3)$]{
 \ig{.19}{./figs/GP-main/RHV_input_dim_3output_dim_3_length_scale_0.1.pdf}
} \hspace{-.5em}
\subfigure[$(d, L) = (3, 4)$]{
 \ig{.19}{./figs/GP-main/RHV_input_dim_3output_dim_4_length_scale_0.1.pdf}
} \hspace{-.5em}
\subfigure[$(d, L) = (3, 5)$]{
 \ig{.19}{./figs/GP-main/RHV_input_dim_3output_dim_5_length_scale_0.1.pdf}
} \hspace{-.5em}
\subfigure[$(d, L) = (3, 6)$]{
 \ig{.19}{./figs/GP-main/RHV_input_dim_3output_dim_6_length_scale_0.1.pdf}
}

 \caption{
 Performance comparison in GP-derived synthetic functions (average and standard deviation of $10$ runs).
 }
 \label{fig:results-GP} 
\end{figure*}

PFEV is a general framework so that we can drive extensions for the following four scenarios:
%
\paragraph{Parallel querying:}%
 	    In parallel querying, we consider querying multiple points at one iteration, which is an important practical setting.
	    %
	    % いま同時に$Q$点の選択を考えているとする．
	    Suppose that we consider $Q > 1$ points selection. 
	    %
	    Let 
	    $\cX_q \coloneqq \{\*x^{(1)}, \ldots, \*x^{(q)} \}$
	    and
	    $\cH_q = \{ \*f_{\*x^{(1)}}, \ldots, \*f_{\*x^{(q)}} \}$
	    for $q \leq Q$.
	    %
	    % 相互情報量
	    % % $\mr{MI}(\cH_q \cup \*f_{\*x} ; \cF^*)$
	    % $\mr{MI}(\cH_Q ; \cF^*)$
	    % に対する$d \times Q$の同時最適化は高次元最適化になるため，$Q$点をgreedyに選ぶ戦略を考える．
	    The MI for all $Q$ points 
	    $\mr{MI}(\cH_Q ; \cF^*)$
	    represents the benefit of selecting $\cX_q$, but this results in a $(Q \times d)$-dimensional optimization problem, which can be unstable.
	    %	    
	    % Takeno2022のアプローチに従って，条件付き相互情報量を使った定式化が可能である．
	    Instead, we follow the approach in \citep{Takeno2022-Sequential}, which is a greedy selection based on conditional mutual information (CMI).
	    %
	    % ある$q$番目の$\*x^{(q)}$までを決定した後に$q+1$番目の$\*x$を探す場合は相互情報量を以下のように分解する: 
	    When we select the $(q+1)$-th $\*x$ after determining $\*x^{(1)}, \ldots, \*x^{(q)}$, the MI can be decomposed into
	    \begin{align*}
	     &
	     \mr{MI}(\cH_q \cup \*f_{\*x} ; \cF^*)
	     % \\
	     % & 
	     \! = \!
	     \mr{MI}(\cH_q ; \cF^*)
	     \! + \!
	     \mr{CMI}(\*f_{\*x} ; \cF^* \mid \cH_q),
	    \end{align*}
	    where
	    $\mr{CMI}(\*f_{\*x} ; \cF^* \mid \cH_q)
	    =
	    \EE_{\cH_q}[ \mr{MI}(\*f_{\*x} ; \cF^* \mid \cH_q) ]$
	    is the MI conditioned on $\cH_q$.
	    %
	    % $\mr{CMI}$を最適化する$\*x$を一つずつ追加していけばよい．
	    Since the first term does not depend on $\*x$, we only need to optimize $\mr{CMI}$ to select $\*x$. 
	    %
	    % この計算は訓練データにサンプリングで作成した
	    % $\cH_q$
	    % を追加したGPを使って通常のPFEVと同様の計算をすればよい．
	    The calculation of $\mr{CMI}$ can be performed by adding sampled $\cH_q$ into the training dataset of the GPs, after which evaluation of the lower bound is almost same as the single querying.
	    %
	    % 詳細はAppendix~\ref{app:parallel-querying}に示す．
	    See Appendix~\ref{app:parallel-querying} for details. 
%
\paragraph{Decoupled setting:}%
In the decoupled setting, we can observe only one selected objective function instead of querying all $L$ objective functions simultaneously \citep{Hernandez-lobatoa2016-Predictive}.
	    %
	    % PFEVではある$l$番目のみ計測した時の相互情報量
	    % $\mr{MI}(f^l_{\*x} ; \cF^*)$
	    % を考えればDecoupled settingの自然は指標とできる．
	    In PFEV, the criterion for the decoupled setting can be defined as 
	    $\mr{MI}(f^l_{\*x} ; \cF^*)$,
	    which is the information gain from only one objective function $f^l_{\*x}$.
	    %
	    % この相互情報量に対する変分下限はSection~\ref{sec:PFEV}で示した方法と同様のアプローチで導出できる．
	    The lower bound of $\mr{MI}(f^l_{\*x} ; \cF^*)$ can be derived by the same approach shown in Section~\ref{sec:PFEV}.
	    %
	    In this case, we need to approximate $p(f^l_{\*x} \mid \cF^*)$ instead of $p(\*f_{\*x} \mid \cF^*)$, for which we can use the marginal distribution of 
	    $q_\lambda(\*f_{\*x} \mid \cF^*)$. 
	    %
	    % Decoupled settingが扱える手法は少なく，我々の知る限りではPESMOとPFESおよびKG baseの手法のみである．
	    %
	    % 詳細はAppendix~\ref{app:decoupled-setting}に示す．
	    See Appendix~\ref{app:decoupled-setting} for detail.
%
\paragraph{Joint entropy search:}% 
	    % PFEVにおいて，出力空間の値のみでなく，入力$\*x$も含めた情報量$\mr{MI}(\*f_{\*x} ; \cX^*, \cF^*)$を考えるJES拡張を考えることもできる, 
	    % where
	    % $\cX^* = \{ \*x \mid \*f_{\*x} \in \cF^* \}$.
	    For PFEV, not only the information gain of the Pareto-frontier $\cF^*$ but also the corresponding input $\*x$ can be considered as
	    $\mr{MI}(\*f_{\*x} ; \cX^*, \cF^*)$,
	    where
	    $\cX^* = \{ \*x \mid \*f_{\*x} \in \cF^* \}$.
	    %
	    This can be seen as a JES extension of PFEV.
	    %
	    % JESでは$p(\*f(\*x) \mid \cF^*)$の代わりに
	    % $p(\*f \mid \cX^*, \cF^*)$
	    % を近似する必要がある．
	    When we derive the lower bound for
	    $\mr{MI}(\*f_{\*x} ; \cX^*, \cF^*)$ 
	    by the same approach as Section~\ref{sec:PFEV}, a variational approximation for $p(\*f \mid \cX^*, \cF^*)$ is required.
	    %
	    % JESの基本的なアイデアはこの分布を近似する際に訓練データに$\cX^*, \cF^*$を追加することである．
	    A basic idea of JES \citep{Tu2022-joint} is to simply add 
	    $(\cX^*, \cF^*)$
	    into the training data of the GPs.
	    %
	    % PFEVの場合は，変分分布
	    % $q(\*f \mid \cX^*, \cF^*)$
	    % でこの分布を近似することになるが，この時，$\cX^*, \cF^*$をGPに追加した分布に置き換えて混合分布を作ればよい．
	    In the case of PFEV, 
	    we can define the variational distribution 
	    $q(\*f \mid \cX^*, \cF^*)$
	    by using the same mixture as \eq{eq:q}.
	    %
	    The only difference is that $(\cX^*, \cF^*)$ is added to the training data of the GPs.
	    %
	    Since we have not observed particular performance improvement by this additional conditioning, we employ $\mr{MI}(\*f_{\*x} ; \cF^*)$ as the default setting of PFEV. 
	    %
	    % 詳細はAppendix~\ref{app:JES}に示す．
	    See Appendix~\ref{app:JES} for detail.
	    %
	    % \red{採用してない理由あった方が良い?}
%
\paragraph{Noisy observations:}%
	    % ノイズを含んだ観測値との情報量は
	    % $\mr{MI}(\*y_{\*x} ; \cF^*)$
	    % となる．
	    It is also possible to derive the information gain obtained from noisy observation
	    $\mr{MI}(\*y_{\*x} ; \cF^*)$,  
	    where
	    $\*y_{\*x} = \*f_{\*x} + \*\veps$ 
	    with
	    $\*\veps \sim \cN(\*0, \sigma_{\rm noise}^2 \*I)$, 
	    though we mainly consider $\mr{MI}(\*f_{\*x} ; \cF^*)$ for brevity.
	    %
	    In this case, instead of 
	    $p(\*f_{\*x} \mid \cF^*)$,
	    we need to consider
	    $p(\*y_{\*x} \mid \cF^*)$. 
	    % この場合，
	    % $p(\*f_{\*x} \mid \cF^*)$ 
	    % の代わりに
	    % $p(\*y_{\*x} \mid \cF^*)$
	    % を考える必要があるが，
	    % $p(\*y_{\*x} \mid \cF^*) = p(\*y_{\*x} \mid \*f_{\*x}) p(\*f_{\*x} \mid \cF^*)$
	    % と書けるため，Section~\ref{sec:PFEV}と同様に$p(\*f_{\*x} \mid \cF^*)$を変分分布$q_{\lambda}$に置き換えて下限を導出できる．
	    Through the relation
	    $p(\*y_{\*x} \mid \cF^*) = \int p(\*y_{\*x} \mid \*f_{\*x}) p(\*f_{\*x} \mid \cF^*) \mr{d} \*f_{\*x}$,
	    we can derive the lower bound based on the same approximation of 
	    $p(\*f_{\*x} \mid \cF^*)$ 
	    by using
	    $q_{\lambda}$.
	    %
	    % 詳細はAppendix~\ref{app:noisy-obs}に示す．
	    See Appendix~\ref{app:noisy-obs} for detail.

% \begin{description}
%  \item[Parallel querying:] 
% 	    % 一度のクエリーで複数の点を指定できる設定は実践上重要である．
% 	    In the parallel querying, we consider querying multiple points at one iteration, which is an important practical setting.
% 	    %
% 	    % いま同時に$Q$点の選択を考えているとする．
% 	    Suppose that we consider $Q > 1$ points selection. 
% 	    %
% 	    Let 
% 	    $\cX_q \coloneqq \{\*x^{(1)}, \ldots, \*x^{(q)} \}$
% 	    and
% 	    $\cH_q = \{ \*f_{\*x^{(1)}}, \ldots, \*f_{\*x^{(q)}} \}$
% 	    for $q \leq Q$.
% 	    %
% 	    % 相互情報量
% 	    % % $\mr{MI}(\cH_q \cup \*f_{\*x} ; \cF^*)$
% 	    % $\mr{MI}(\cH_Q ; \cF^*)$
% 	    % に対する$d \times Q$の同時最適化は高次元最適化になるため，$Q$点をgreedyに選ぶ戦略を考える．
% 	    MI for all $Q$ points 
% 	    $\mr{MI}(\cH_Q ; \cF^*)$
% 	    represents the benefit of selecting $\cX_q$, but this results in a $(Q \times d)$-dimensional optimization problem, which can be unstable.
% 	    %	    
% 	    % Takeno2022のアプローチに従って，条件付き相互情報量を使った定式化が可能である．
% 	    Instead, we follow an approach in \citep{Takeno2022-Sequential}, which is a greedy selection based on conditional mutual information (CMI).
% 	    %
% 	    % ある$q$番目の$\*x^{(q)}$までを決定した後に$q+1$番目の$\*x$を探す場合は相互情報量を以下のように分解する: 
% 	    When we select the $(q+1)$-th $\*x$ after determining $\*x^{(1)}, \ldots, \*x^{(q)}$, MI can be decomposed into
% 	    \begin{align*}
% 	     &
% 	     \mr{MI}(\cH_q \cup \*f_{\*x} ; \cF^*)
% 	     % \\
% 	     % & 
% 	     \! = \!
% 	     \mr{MI}(\cH_q ; \cF^*)
% 	     \! + \!
% 	     \mr{CMI}(\*f_{\*x} ; \cF^* \mid \cH_q),
% 	    \end{align*}
% 	    where
% 	    $\mr{CMI}(\*f_{\*x} ; \cF^* \mid \cH_q)
% 	    =
% 	    \EE_{\cH_q}[ \mr{MI}(\*f_{\*x} ; \cF^* \mid \cH_q) ]$
% 	    is the MI conditioned on $\cH_q$.
% 	    %
% 	    % $\mr{CMI}$を最適化する$\*x$を一つずつ追加していけばよい．
% 	    Since the first term does not depends on $\*x$, we only need to optimize $\mr{CMI}$ to select $\*x$. 
% 	    %
% 	    % この計算は訓練データにサンプリングで作成した
% 	    % $\cH_q$
% 	    % を追加したGPを使って通常のPFEVと同様の計算をすればよい．
% 	    The calculation of $\mr{CMI}$ can be performed by adding sampled $\cH_q$ into the training dataset of the GPs, after which evaluation of the lower bound is almost same as the single querying.
% 	    %
% 	    % 詳細はAppendix~\ref{app:parallel-querying}に示す．
% 	    See Appendix~\ref{app:parallel-querying} for detail. 

%  \item[Decoupled setting:] 
% 	    % 多目的最適化において，全ての目的関数を同時に計測するのではなく選択した一つだけを計測できる設定をDecoupled settingと呼ぶ\citep{}．
% 	    In the decoupled setting, we can observe only one selected objective function instead of querying all $L$ objective functions simultaneously \citep{Hernandez-lobatoa2016-Predictive}.
% 	    %
% 	    % PFEVではある$l$番目のみ計測した時の相互情報量
% 	    % $\mr{MI}(f^l_{\*x} ; \cF^*)$
% 	    % を考えればDecoupled settingの自然は指標とできる．
% 	    In PFEV, the criterion for the decoupled setting can be defined as 
% 	    $\mr{MI}(f^l_{\*x} ; \cF^*)$,
% 	    which is the information gain from only one objective function $f^l_{\*x}$.
% 	    %
% 	    % この相互情報量に対する変分下限はSection~\ref{sec:PFEV}で示した方法と同様のアプローチで導出できる．
% 	    The lower bound of $\mr{MI}(f^l_{\*x} ; \cF^*)$ can be derived by the same approach shown in Section~\ref{sec:PFEV}.
% 	    %
% 	    In this case, we need to approximate $p(f^l_{\*x} \mid \cF^*)$ instead of $p(\*f_{\*x} \mid \cF^*)$, for which we can use the marginal distribution of 
% 	    $q_\lambda(\*f_{\*x} \mid \cF^*)$. 
% 	    %
% 	    % Decoupled settingが扱える手法は少なく，我々の知る限りではPESMOとPFESおよびKG baseの手法のみである．
% 	    %
% 	    % 詳細はAppendix~\ref{app:decoupled-setting}に示す．
% 	    See Appendix~\ref{app:decoupled-setting} for detail.


%  \item[Joint entropy search:] 
% 	    % PFEVにおいて，出力空間の値のみでなく，入力$\*x$も含めた情報量$\mr{MI}(\*f_{\*x} ; \cX^*, \cF^*)$を考えるJES拡張を考えることもできる, 
% 	    % where
% 	    % $\cX^* = \{ \*x \mid \*f_{\*x} \in \cF^* \}$.
% 	    For PFEV, not only the information gain of the Pareto-frontier $\cF^*$ but also the corresponding input $\*x$ can be considered as
% 	    $\mr{MI}(\*f_{\*x} ; \cX^*, \cF^*)$,
% 	    where
% 	    $\cX^* = \{ \*x \mid \*f_{\*x} \in \cF^* \}$.
% 	    %
% 	    This can be seen as a JES extension of PFEV.
% 	    %
% 	    % JESでは$p(\*f(\*x) \mid \cF^*)$の代わりに
% 	    % $p(\*f \mid \cX^*, \cF^*)$
% 	    % を近似する必要がある．
% 	    When we derive the lower bound for
% 	    $\mr{MI}(\*f_{\*x} ; \cX^*, \cF^*)$ 
% 	    by the same approach as Section~\ref{sec:PFEV}, a variational approximation for $p(\*f \mid \cX^*, \cF^*)$ is required.
% 	    %
% 	    % JESの基本的なアイデアはこの分布を近似する際に訓練データに$\cX^*, \cF^*$を追加することである．
% 	    A basic idea of JES \citep{Tu2022-joint} is to simply add 
% 	    $(\cX^*, \cF^*)$
% 	    into the training data of the GPs.
% 	    %
% 	    % PFEVの場合は，変分分布
% 	    % $q(\*f \mid \cX^*, \cF^*)$
% 	    % でこの分布を近似することになるが，この時，$\cX^*, \cF^*$をGPに追加した分布に置き換えて混合分布を作ればよい．
% 	    In the case of PFEV, 
% 	    we can define the variational distribution 
% 	    $q(\*f \mid \cX^*, \cF^*)$
% 	    by using the same mixture as \eq{eq:q}.
% 	    %
% 	    The only difference is that $(\cX^*, \cF^*)$ is added to the training data of the GPs.
% 	    %
% 	    Since we have not observed particular performance improvement by this additional conditioning, we employ $\mr{MI}(\*f_{\*x} ; \cF^*)$ as the default setting of PFEV. 
% 	    %
% 	    % 詳細はAppendix~\ref{app:JES}に示す．
% 	    See Appendix~\ref{app:JES} for detail.
% 	    %
% 	    % \red{採用してない理由あった方が良い?}

%  \item[Noisy observations:]
% 	    % ノイズを含んだ観測値との情報量は
% 	    % $\mr{MI}(\*y_{\*x} ; \cF^*)$
% 	    % となる．
% 	    It is also possible to derive the information gain obtained from noisy observation
% 	    $\mr{MI}(\*y_{\*x} ; \cF^*)$,  
% 	    where
% 	    $\*y_{\*x} = \*f_{\*x} + \*\veps$ 
% 	    with
% 	    $\*\veps \sim \cN(\*0, \sigma_{\rm noise}^2 \*I)$, 
% 	    though we mainly consider $\mr{MI}(\*f_{\*x} ; \cF^*)$ for brevity.
% 	    %
% 	    In this case, instead of 
% 	    $p(\*f_{\*x} \mid \cF^*)$,
% 	    we need to consider
% 	    $p(\*y_{\*x} \mid \cF^*)$. 
% 	    % この場合，
% 	    % $p(\*f_{\*x} \mid \cF^*)$ 
% 	    % の代わりに
% 	    % $p(\*y_{\*x} \mid \cF^*)$
% 	    % を考える必要があるが，
% 	    % $p(\*y_{\*x} \mid \cF^*) = p(\*y_{\*x} \mid \*f_{\*x}) p(\*f_{\*x} \mid \cF^*)$
% 	    % と書けるため，Section~\ref{sec:PFEV}と同様に$p(\*f_{\*x} \mid \cF^*)$を変分分布$q_{\lambda}$に置き換えて下限を導出できる．
% 	    Through the relation
% 	    $p(\*y_{\*x} \mid \cF^*) = \int p(\*y_{\*x} \mid \*f_{\*x}) p(\*f_{\*x} \mid \cF^*) \mr{d} \*f_{\*x}$,
% 	    we can derive the lower bound based on the same approximation of 
% 	    $p(\*f_{\*x} \mid \cF^*)$ 
% 	    by using
% 	    $q_{\lambda}$.
% 	    %
% 	    % 詳細はAppendix~\ref{app:noisy-obs}に示す．
% 	    See Appendix~\ref{app:noisy-obs} for detail.


% \end{description}




% --------------------------------------------------
% \section{実験}
\section{Experiments}
\label{sec:experiments}


% \red{本論とAppendixの違い（MESMO, ParEGO, MOBO-RS，Random）}
% --------------------------------------------------
% 本節では，提案手法PFEVの性能評価について述べる．
We empirically verify the performance of PFEV by comparing {mainly with 
%
% 既存手法であるParEGO \citep{Knowles2006-parego}，EHVI \citep{Emmerich2005-single}，SMSego \citep{Ponweiser2008-multiobjective}，MESMO \citep{Belakaria2019-max}，PFES \citep{Suzuki2020-multi}，および$\{\text{PF}\}^{2}\text{ES}$ \citep{Qing2022-text}との比較を行い，
% ParEGO \citep{Knowles2006-parego}, EHVI \citep{Emmerich2005-single}, MOBO-RS \citep{Paria2020-flexible}, MESMO \citep{Belakaria2019-max}, PFES \citep{Suzuki2020-multi}, $\{\text{PF}\}^{2}\text{ES}$ \citep{Qing2022-text}, and JES \citep{Tu2022-joint}. 
% ParEGO \citep{Knowles2006-parego}, EHVI \citep{Emmerich2005-single}, MOBO-RS \citep{Paria2020-flexible}, MESMO \citep{Belakaria2019-max}, PFES \citep{Suzuki2020-multi}, $\{\text{PF}\}^{2}\text{ES}$ \citep{Qing2022-text}, JES \citep{Tu2022-joint}, \red{and random search}. 
EHVI \citep{Emmerich2005-single}, PFES \citep{Suzuki2020-multi}, $\{\text{PF}\}^{2}\text{ES}$ \citep{Qing2022-text}, JES \citep{Tu2022-joint}, and random search. 
%
In Appendix~\ref{app:additional_experiments}, we added other methods such as ParEGO \citep{Knowles2006-parego}, MOBO-RS \citep{Paria2020-flexible}, and MESMO \citep{Belakaria2019-max}, which are mostly omitted in the main text for brevity of plots. 
}
%
% GP由来の人工関数実験とベンチマーク関数実験の両方で評価を行う．
% We used GP-based synthetic functions and benchmark functions.
We show results on GP-based synthetic functions, benchmark functions, and hyper-parameter optimization problems.

% --------------------------------------------------
% \subsection{実験設定}
% \subsection{Settings}

% 各実験は10回の試行を行う．性能評価には相対ハイパーボリューム（relative hyper-volume: RHV）\citep{Suzuki2020-multi}を用いる．
Each evaluation run $10$ times.
%
As a performance metric, RHV (relative hyper-volume) was used. 
%
% これは，観測済みデータから得られるパレートフロンティアの超体積を，真のパレートフロンティアの超体積で割った値であり，$[0,1]$の範囲を取る．
RHV is defined as the hyper-volume of the observed Pareto-frontier divided by the volume of the reference Pareto-frontier.
%
% Since the true Pareto-frontier is unknown, we used the solution obtained by $10,000$ iterations of NSGA-II as an approximate normalization constant. 
The reference Pareto-frontier was obtained by $10,000$ iterations of NSGA-II.
% RHV is in $[0,1]$ and the best value is $1$.
% 1に近いほど良い性能を示す．
%
% 既存手法のパラメータについて，ParEGOのチェビシェフ線形和の重み定数は\citep{Knowles2006-parego}に従い0.05とし，SMSegoの上側信頼区間の係数$\beta$は\citep{Ponweiser2008-multiobjective}に従い
% $\beta = \Phi^{-1}(0.5+1/2^{L})$
% とする（$\Phi$は標準正規分布の累積分布関数）．
% Appendixに
%
% 目的関数$f^l_{\*x}$のGPのカーネル関数には以下のRBFカーネルを使用する：
All methods used GPs for $f^l_{\*x}$ with a kernel function
$k(\*x, \*x^{\prime})= \exp (- \|\*x-\*x^{\prime} \|_2^2 / (2 \ell^2_{\rm RBF}) )$,
% \begin{align*}
%  % k(\*x, \*x^{\prime})=\theta_1 \exp \left(-\frac{|\*x-\*x^{\prime}|{2}^2}{\theta_2}\right)
%  % k(\*x, \*x^{\prime})= \exp \left(-\frac{ \|\*x-\*x^{\prime} \|_2^2}{\theta}\right),
%  k(\*x, \*x^{\prime})= \exp \left(- \frac{1}{2} \frac{ \|\*x-\*x^{\prime} \|_2^2}{ \ell^2_{\rm RBF} }\right),
% \end{align*}
% ただし，$\theta \in \RR$はハイパーパラメータである．
where $\ell_{\rm RBF} \in \RR$ is a hyper-parameter.
%
% すべての実験において，$\theta$は反復ごとに周辺尤度最大化により最適化する．
The marginal likelihood maximization was performed at every iteration to optimize $\ell_{\rm RBF}$.
% ただし，$\theta_1, \theta_{2} \in \mathbb{R}$はハイパーパラメータである．すべての実験において，$\theta_1$は1.0に固定し，$\theta_2$のみを反復ごとに周辺尤度最大化により最適化する．
%
% MESMO, PFES, $\{$PF$\}^2$ES, PFEVにおける最適値及びパレートフロンティアのサンプルサイズは10とする．
The number of samples of the optimal value or the Pareto-frontier in MESMO, PFES, $\{$PF$\}^2$ES, and PFEV was $10$, each of which was performed by NSGA-II ($1,000$ generations and population size $50$). 
%
% 獲得関数の最大化にはDIRECTアルゴリズム\citep{Jones1993-lipschitzian}を用いる．
We used the DIRECT algorithm \citep{Jones1993-lipschitzian} for the acquisition function maximization. 
%
% 初期観測点は5点をランダムに選択する．
% We selected $5$ random $\*x$ as the initial points.
We selected $5$ random $\*x$ as the initial observations in $\cD$.
%
% \red{
% % Due to high computational cost, SMSego, EHVI and JES were performed up to $L = 4$.
% Due to high computational cost, 
% \remove{EHVI and JES were performed up to $L = 4$.}
Depending on problems, EHVI and JES were performed up to $L = 4$ due to computational issues. % ちょっと誤魔化した表現だけどやってたりやってなかったりバラバラなので(本当はきちんとしたい)
% }
%
% EHVIとJESは$L = 4$まで実行し，PerEGO，MOBO-RS, MESMOの結果は本論では省略する
% \red{EHVI and JES were performed up to $L = 4$, and the results for PerEGO, MOBO-RS, and MESMO are omitted in the main text.}
Other settings are described in Appendix~\ref{app:bo-settings}. 
% （\red{Appendixに一部移動させる？}その他の実験設定の詳細はAppendixに記述する．）実装および計算の複雑性の問題から，PESMO，JESとの比較は行えなかったが，選択した比較手法は現在広く利用されており，PFEVの性能を検証するベースラインとして十分であると考える．



% --------------------------------------------------
% \subsection{GP由来の人工関数実験}
\subsection{Synthetic Functions Generated by GPs}
\label{ssec:GPDerivedArtificialFunctions}



% 本節では，GPから生成した人工関数
% $f_\ell \sim \mathcal{GP}(0, k)$
% を真の目的関数として用いる．
Here, we consider synthetic functions from GPs as true objective functions, i.e., 
$f^l \sim \mathcal{GP}(0, k)$, in which $\ell_{\rm RBF} = 0.1$ was used in the kernel $k$.
%
% また生成する際のカーネル$k$は$\theta = 0.25^2$とした．
%
% ただし連続空間上の関数を得るために，実際にはRFMによる近似を用いて関数サンプルを作成した（基底関数の数は$D = 1000$）．
Since we require objective functions in a continuous domain, we used the RFM-based approximation (the number of RFM basis is $D = 1000$). 
%
% 入力の次元数$d$は$d =2$，入力空間$\cX$は$[0, 1]^{2}$とする．
The input dimensions are $d \in \{ 2, 3 \}$, and the domain $\cX$ is $[0, 1]^{d}$.
%
% 出力の次元数$L$は$L = 3, 4, 5, 6$とする．
The output dimensions are $L \in \{ 2, 3, 4, 5, 6 \}$. 

% --------------------------------------------------
% Fig: Boxplots
% --------------------------------------------------
\begin{figure}[t!]
 \centering

 \ig{.4}{./figs/GP-boxplot/GP-boxplot-legend.pdf}

 \vspace{-.5em}

\subfigure[$L = 2$]{
 \ig{.09}{./figs/GP-boxplot/boxplot_L2.pdf}
} \hspace{-.7em}
\subfigure[$L = 3$]{
 \ig{.09}{./figs/GP-boxplot/boxplot_L3.pdf}
} \hspace{-.7em}
\subfigure[$L = 4$]{
 \ig{.09}{./figs/GP-boxplot/boxplot_L4.pdf}
} \hspace{-.7em}
\subfigure[$L = 5$]{
 \ig{.09}{./figs/GP-boxplot/boxplot_L5.pdf}
} \hspace{-.7em}
\subfigure[$L = 6$]{
 \ig{.09}{./figs/GP-boxplot/boxplot_L6.pdf}
}

 \caption{
 Boxplots of RHV at $100$-th iteration.
 %
 Note that, here, methods omitted in Fig.~\ref{fig:results-GP} (ParEGO, MOBO-RS, and MESMO) are also included, which are shown Appendix~\ref{app:additional_experiments_GP}.
 }
 \label{fig:GP-boxplot}
\end{figure}

% 本節では，GP由来の人工関数を用いて，PFEVと既存の多目的ベイズ最適化手法の性能比較を行う．
%
% 入力空間$\mathcal{X}$を$[0, 1]^{2}$とし，入力空間内の連続領域の任意の値を候補点とする．
%
% 最適化を行う目的関数
% $\boldsymbol{f}(\boldsymbol{x}):=\left(f_{1}(\boldsymbol{x}), \ldots, f_{L}(\boldsymbol{x})\right)^{\top} \in \mathbb{R}^{L}$
% は，以下のように定義されるGPからサンプリングされる：
% \begin{align*}
% f_\ell &\sim \mathcal{GP}(0, k) \text{ for } \ell \in [L] , \\
% k\left(\*x, \*x^{\prime}\right)&=\exp \left(-\frac{\left\|\*x-\*x^{\prime}\right\|^2}{s^2}\right).
% \end{align*}
% ただし，$s \in \mathbb{R}$はlength scaleと呼ばれるハイパーパラメータである．

% 図\ref{fig:benchmark_results}に結果を示す．
Figure~\ref{fig:results-GP} shows the results.
%
% 図\ref{fig:benchmark_results}の結果から，すべての人工関数において，
% 図\ref{fig:benchmark_results}(a)-(d)の全てについてPFEVは既存手法と同等以上の性能を示している．
In all (a)-(j), PFEV shows superior or comparable performance to existing methods. 
% ParEGO，SMSego，EHVI，MESMO，PFES，$\{\text{PF}\}^{2}\text{ES}$と比較して，同等以上の性能を示している．
%
% 特に出力次元が高次元（$L \geq 4$）の場合，PFEVが既存手法よりも明らかに優れていることがわかる．
% \red{Further, we see that, for output dimensions $L \geq 4$, performance of PFEV was particularly better than the other methods.}
% 我々は$L = 2$においてはPFEVがPFESとPF2ESに近い性能になりやすく，$L \geq 3$においてこれらと違いが生まれやすいことを確認した．
In these experiments, we empirically see that the performance of PFEV is often similar to PFES and $\{\text{PF}\}^{2}\text{ES}$ for $L =2$, and differences become clearer for $L \geq 3$. 
%
% これは以下の図はiteration=100における図におけるRHVの各試行すべての結果の値をboxplotにしたものからも確認できる
This can also be confirmed by Fig.~\ref{fig:GP-boxplot}, which shows boxplots of RHV at the $100$-th iteration in all trials of Fig.~\ref{fig:results-GP}.
% 
This result is consistent with our conjecture about the difference of two types of PFTN described in Section~\ref{ssec:VLBMaximization}.
% $|\cF_S| = 50$ can be 
% We empirically see that PFEV shows superior performance particularly when the output dimension is high. 
%
% 出力次元が大きい場合，\ref{ssec:VLBMaximization}節で述べたとおり，2つの切断方法のどちらを採用したかによるsupportのズレは大きくなる．
% In the case of a higher output dimension, the difference of two types of PFTN becomes large as described in Section~\ref{ssec:VLBMaximization}.
%
% そのため$\lambda$の導入により，過小および過剰な切断の影響度合いをコントロールしたことによる効果が出力次元の高い設定の方に顕著に現れたと推察される．
% Therefore, the result suggests that the effect of controlling the balance of under and over-truncation is more influential for higher dimension problems.
%
In Appendix~\ref{app:additional_experiments_GP}, additional results on different $\ell_{\rm RBF}$ and $d = 4$ are shown, in which similar tendency was confirmed.

% 出力次元が大きい場合，\ref{ssec:VLBMaximization}節で述べたとおり，2つの切断方法のどちらを採用したかによるsupportのズレは大きくなる．提案法では，既存の情報論的多目的ベイズ最適化であるPFES，$\{\text{PF}\}^{2}\text{ES}$とは異なり，$\lambda$の導入により，過小および過剰な切断の影響度合いをコントロールできるようになっている．そのため，PFEVは，出力次元が大きい場合に性能が向上する（出力の次元数に関してロバストである）と考えられる．
% （卒論時の離散設定では，目的関数の形状が滑らかな場合において，PFEVのクエリ設定では，あまりそのような傾向が見られなかった結果の理由は若干気になる？）



% --------------------------------------------------
% \subsection{ベンチマーク関数実験}
\subsection{Benchmark Functions}
% --------------------------------------------------

% GP由来の関数については，多目的問題を10個生成し，それぞれの実験を10回実施しました．
% その結果，
% ベンチマーク関数については，ランダムに初期化した10回の平均と標準偏差を報告します．
% 初期点数などの実験の詳細はAppendixに示されています．
% --------------------------------------------------
% Fig: Benchmark 
% --------------------------------------------------
% \begin{figure}[t!]
% \centering
% \subfigure[Fonseca Fleming]{ % $(d, L) = (2, 2)$
%   \ig{.2}{./figs/Bench1/RHV_Fonseca_Fleming_max_input_dim_2_output_dim_2.pdf}
% }
% \subfigure[Kursawe]{ % $(d, L) = (3, 2)$
%   \ig{.2}{./figs/Bench1/RHV_Kursawe_max_input_dim_3_output_dim_2.pdf}
% }
% \subfigure[Viennet]{ % $(d, L) = (2, 3)$
%   \ig{.2}{./figs/Bench1/RHV_Viennet_max_input_dim_2_output_dim_3.pdf}
% }
% \subfigure[FES3]{ % $(d, L) = (3, 4)$
%   \ig{.2}{./figs/Bench1/RHV_FES3_max_input_dim_3_output_dim_4.pdf}
% }
% \subfigure[Fonseca$+$Viennet]{ % $(d, L) = (2, 5)$
%   \ig{.2}{./figs/Bench1/RHV_Fonseca_Viennet_scaled_max_input_dim_2_output_dim_5.pdf}
% }
% \subfigure[FES3$+$Kursawe]{ % $(d, L) = (3, 6)$
%   \ig{.2}{./figs/Bench1/RHV_FES3_Kursawe_scaled_max_input_dim_3_output_dim_6.pdf}
% } 

%  \caption{
%  % ベンチマーク関数における性能比較（10回の実行における平均値と標準誤差）
%  Performance comparison in benchmark functions (average and standard deviation of $10$ runs).
%  }
%  \label{fig:results_benchmark}
% \end{figure}
\begin{figure}[t!]
	\centering
	\subfigure[Fonseca-Fleming]{ % $(d, L) = (2, 2)$
	  \ig{.2}{./figs/benchmark-main/RHV_Fonseca_Fleming_max_input_dim_2_output_dim_2.pdf}
	}
	\subfigure[Kursawe]{ % $(d, L) = (3, 2)$
	  \ig{.2}{./figs/benchmark-main/RHV_Kursawe_max_input_dim_3_output_dim_2.pdf}
	}
	\subfigure[Viennet]{ % $(d, L) = (2, 3)$
	  \ig{.2}{./figs/benchmark-main/RHV_Viennet_max_input_dim_2_output_dim_3.pdf}
	}
	\subfigure[FES3]{ % $(d, L) = (3, 4)$
	  \ig{.2}{./figs/benchmark-main/RHV_FES3_max_input_dim_3_output_dim_4.pdf}
	}
	\subfigure[Fonseca$+$Viennet]{ % $(d, L) = (2, 5)$
	  \ig{.2}{./figs/benchmark-main/RHV_Fonseca_Viennet_scaled_max_input_dim_2_output_dim_5.pdf}
	}
	\subfigure[FES3$+$Kursawe]{ % $(d, L) = (3, 6)$
	  \ig{.2}{./figs/benchmark-main/RHV_FES3_Kursawe_scaled_max_input_dim_3_output_dim_6.pdf}
	} 
	
 \caption{
 % ベンチマーク関数における性能比較（10回の実行における平均値と標準誤差）
 Performance comparison in benchmark functions (average and standard deviation of $10$ runs).
 }
 \label{fig:results_benchmark}
	\end{figure}
% --------------------------------------------------
% Fig: Benchmark Functions
% --------------------------------------------------
% \begin{figure}[t]
%   \centering
%   % \begin{subfigure}[b]{0.22\textwidth}
%   %     \centering
%   %     \includegraphics[width=\linewidth, height=0.7\textheight, keepaspectratio]{./figs/20241028/RHV_FES3_max_sphere_max_input_dim_3_output_dim_5.pdf}
%   %     \caption{FES3+Sphere}
%   % \end{subfigure}
%  \subfigure[FES3+Sphere]{
%  \ig{.22}{./figs/20241028/RHV_FES3_max_sphere_max_input_dim_3_output_dim_5.pdf}
%  }
%   % \begin{subfigure}[b]{0.22\textwidth}
%   %     \centering
%   %     \includegraphics[width=\linewidth, height=0.7\textheight, keepaspectratio]{./figs/20241028/RHV_FES3_max_rosenbrock_max_input_dim_3_output_dim_5.pdf}
%   %     \caption{FES3+Rosenbrock}
%   % \end{subfigure}
%  \subfigure[FES3+Rosenbrock]{
%  \centering
%  \ig{.22}{./figs/20241028/RHV_FES3_max_rosenbrock_max_input_dim_3_output_dim_5.pdf}
%  }

%   \vspace{5pt} % Optional spacing between rows
%   % \begin{subfigure}[b]{0.22\textwidth}
%   %     \centering
%   %     \includegraphics[width=\linewidth, height=0.7\textheight, keepaspectratio]{./figs/20241029/RHV_FES3_max_DTLZ2_max_input_dim_3_output_dim_6.pdf}
%   %     \caption{FES3+DTLZ2}
%   % \end{subfigure}
%  \subfigure[FES3+DTLZ2]{
%  \ig{.22}{./figs/20241029/RHV_FES3_max_DTLZ2_max_input_dim_3_output_dim_6.pdf}
%  }
%   % \begin{subfigure}[b]{0.22\textwidth}
%   %     \centering
%   %     \includegraphics[width=\linewidth, height=0.7\textheight, keepaspectratio]{./figs/20241029/RHV_FES3_max_DTLZ4_max_input_dim_3_output_dim_6.pdf}
%   %     \caption{FES3+DTLZ4}
%   % \end{subfigure}
%  \subfigure[FES3+DTLZ4]{
%  \ig{.22}{./figs/20241029/RHV_FES3_max_DTLZ4_max_input_dim_3_output_dim_6.pdf}
%  }

%   \caption{
%  % ベンチマーク関数における性能比較（10回の実行における平均値と標準誤差）
%  Performance comparison in benchmark functions (average and standard deviation of $10$ runs).
%  }
%   \label{fig:benchmark_results}
% \end{figure}
% 本節では，ベンチマーク関数を用いて，PFEVと既存の多目的ベイズ最適化手法の性能比較を行う．
% 連続領域を持つベンチマーク関数を用いた．
% 入力空間$\mathcal{X}$を$[0, 1]^{2}$とし，入力空間内の連続領域の任意の値を候補点とする．
% ベンチマーク関数はFES3\citep{Huband2006-review}，Sphere\citep{simulationlib}，Rosenbrock\citep{simulationlib}，DTLZ2\citep{Deb2002-scalable}，DTLZ4\citep{Deb2002-scalable}を用いる．
% FES3は入力と出力の次元数は$d = 3$と$L = 4$であり，SphereとRosenbrockの入出力の次元数は$(d, L) = (3, 1)$である．
% また，その他の関数の入出力の次元数は$(d, L) = (3, 2)$である．
% これらの関数の詳細はAppendixに記述する．

% 図\ref{fig:benchmark_results}に四つのベンチマーク関数に対して各獲得関数を適用した結果を示した．
% 入出力の次元数は（a），（b）が$(d, L) = (3, 5)$である．
% 図\ref{fig:benchmark_results}の（a）はFES3関数とSphere関数という二つの多目的関数を組み合わせて多目的最適化問題とする．
% 図\ref{fig:benchmark_results}の（b）はFES3関数とRosenbrock関数という二つの多目的関数を組み合わせて多目的最適化問題とする．
% 図\ref{fig:benchmark_results}の（c）はFES3関数とDTLZ2関数という二つの多目的関数を組み合わせて多目的最適化問題とする．
% 図\ref{fig:benchmark_results}の（d）はFES3関数とDTLZ4関数という二つの多目的関数を組み合わせて多目的最適化問題とする．
% 図\ref{fig:benchmark_results}の結果から，
% すべての人工データにおいて，提案法の性能は，ParEGO, MESMO, PFES, $\{\text{PF}\}^{2}\text{ES}$の性能を上回っている．
% これらの結果から，ベンチマーク関数においても，GP由来の人工関数実験と同様に，出力次元が高次元（$L \geq 4$）の場合において，
% 既存手法と比較した際にPFEVの優位性があるということが確認することができる．



% 本節では，連続領域を持つベンチマーク関数を用いて，PFEVと既存の多目的ベイズ最適化手法の性能比較を行う．
% 次に，ベンチマーク関数を用いた評価を行う．
%
% 入力空間$\mathcal{X}$を$[0, 1]^{2}$とし，入力空間内の連続領域の任意の値を候補点とする．
% 入力空間$\cX$を$[0, 1]^d$とする．
% \red{
% In benchmark function experiments, we created multi-objective problems by combining multiple existing benchmark functions.
% %
% % 評価には，FES3\citep{Huband2006-review}，Sphere\citep{simulationlib}，Rosenbrock\citep{simulationlib}，DTLZ2\citep{Deb2002-scalable}，DTLZ4\citep{Deb2002-scalable}を用いる．
% % 目的関数にはFES3\citep{Huband2006-review}，Sphere\citep{simulationlib}，Rosenbrock\citep{simulationlib}，DTLZ2\citep{Deb2002-scalable}，DTLZ4\citep{Deb2002-scalable}を組み合わせて用いる．
% We used well-known benchmark functions such as FES3 \citep{Huband2006-review}, Sphere \citep{simulationlib}, Rosenbrock \citep{simulationlib}, DTLZ2 \citep{Deb2002-scalable}, and DTLZ4 \citep{Deb2002-scalable}. 
% %
% % FES3は入力と出力の次元数がそれぞれ$d = 3$と$L = 4$であり，SphereとRosenbrockの入出力の次元数は$(d, L) = (3, 1)$である．
% FES3 has the input and output dimensions $(d, L) = (3, 4)$ and  Rosenbrock has $(d, L) = (3, 1)$.
% %
% % その他の関数の入出力の次元数は$(d, L) = (3, 2)$である．
% The other benchmark functions are $(d, L) = (3, 2)$.
% %
% % 入力空間$\cX$は組み合わせるベンチマーク関数の$\cX$の共通部分とする．
% The input domain $\cX$ is defined by the intersection of the combined benchmark functions.
% %
% % これらの関数の詳細はAppendix~\ref{app:benchmarks}に記述する．
% Details of the benchmark functions are shown in Appendix~\ref{app:benchmarks}.
% }


We used benchmark problems called Fonseca-Fleming $(d, L) = (2, 2)$, Kursawe $(d, L) = (3, 2)$, Viennet $(d, L) = (2, 3)$ and FES3 $(d, L) = (3, 4)$ problems (for details, see Appendix~\ref{app:bo-settings}).
%
Further, we combine multiple problems having the same input dimensions, i.e., we created Fonseca$+$Viennet $(d, L) = (2, 5)$ and FES3$+$Kursawe $(d, L) = (3, 6)$.
%
Since the input domain is shared (which is scaled to $[0, 1]^d$ beforehand), only the output dimension increases compared with the original problems.
%
The results are shown in Fig.~\ref{fig:results_benchmark}. 
%
Overall, the performance of proposed PFEV is high among the compared methods.
%
% Here again, we see that in problems with higher output dimensions (FES3 $L =4$, Fonseca$+$Viennet $L = 5$, and FES3$+$Kursawe $L = 6$), PFEV shows its advantage.
Here again, we see that in problems with the output dimension $\geq 3$, PFEV tends to show its advantage.
%
Additional results on benchmark functions are also shown in Appendix~\ref{app:additional_experiments_bench}.
% 評価には，FES3\citep{Huband2006-review}，Sphere\citep{simulationlib}，Rosenbrock\citep{simulationlib}，DTLZ2\citep{Deb2002-scalable}，DTLZ4\citep{Deb2002-scalable}を用いる．
% 目的関数にはFES3\citep{Huband2006-review}，Sphere\citep{simulationlib}，Rosenbrock\citep{simulationlib}，DTLZ2\citep{Deb2002-scalable}，DTLZ4\citep{Deb2002-scalable}を組み合わせて用いる．
% We used well-known benchmark functions such as FES3 \citep{Huband2006-review}, Sphere \citep{simulationlib}, Rosenbrock \citep{simulationlib}, DTLZ2 \citep{Deb2002-scalable}, and DTLZ4 \citep{Deb2002-scalable}. 
%
% FES3は入力と出力の次元数がそれぞれ$d = 3$と$L = 4$であり，SphereとRosenbrockの入出力の次元数は$(d, L) = (3, 1)$である．
% FES3 has the input and output dimensions $(d, L) = (3, 4)$ and  Rosenbrock has $(d, L) = (3, 1)$.
%
% その他の関数の入出力の次元数は$(d, L) = (3, 2)$である．
% The other benchmark functions are $(d, L) = (3, 2)$.
%
% 入力空間$\cX$は組み合わせるベンチマーク関数の$\cX$の共通部分とする．
% The input domain $\cX$ is defined by the intersection of the combined benchmark functions.
%
% これらの関数の詳細はAppendix~\ref{app:benchmarks}に記述する．
% Details of the benchmark functions are shown in Appendix~\ref{app:benchmarks}.



% \red{
% % 図\ref{fig:benchmark_results}に四つの実験設定に対する結果を示す．
% Figure~\ref{fig:benchmark_results} shows the results on four combined functions.
% %
% % 図\ref{fig:benchmark_results}の(a)，(b)はともに入出力の次元数が$(d, L) = (3, 5)$である．
% %
% Figure~\ref{fig:benchmark_results}~ (a) and (b) are both $(d, L) = (3, 5)$.
% %
% (a) combines FES3 and Sphere, and (b) combines FES3 and Rosenbrock.
% % (a)はFES3関数とSphere関数を，(b)はFES3関数とRosenbrock関数を組み合わせた多目的最適化問題である．
% %
% % また，(c)，(d)は$(d, L) = (3, 6)$であり，(c)はFES3関数とDTLZ2関数を，(d)はFES3関数とDTLZ4関数を組み合わせた問題である．
% (c) and (d) are $(d, L) = (3, 6)$. 
% %
% (c) combines FES3 and DTLZ2, and (d) combines FES3 and DTLZ4.
% %
% % 実験結果から，すべての設定において提案法PFEVの性能は，ParEGO，MESMO，PFES，$\{\text{PF}\}^{2}\text{ES}$の性能を上回ることが確認された．
% In the results, PFES outperforms all the other methods.
% %
% % 特に出力次元が高次元（$L \geq 4$）の場合において，GP由来の人工関数実験と同様に，既存手法と比較したPFEVの優位性が顕著に表れている．
% }

% --------------------------------------------------
% \subsection{ベンチマーク関数実験}
% --------------------------------------------------

% --------------------------------------------------
% \subsection{実験}
\subsection{Hyper-parameter Optimization of LightGBM}

% We applied PFEV to optimize class weights in multi-class classification problems using LightGBM \green{\cite{ke2017lightgbm}} as the base model. 
As an application example of hyper-parameter optimization problems, we consider optimizing class weights in multi-class classification problems using LightGBM \citep{ke2017lightgbm} as the base model (this setting is from \citep{ozaki2024multi}).
%
% In this realistic machine learning scenario, 
We focused solely on optimizing the class weight parameters, making the input dimension of BO equal to the number of classes. 
%
The objective functions are the test classification accuracies for each class, which means the output dimension also equals to the number of classes. 
%
% Experiments were conducted on four datasets with varying characteristics: Abalone and Waveform (both with 3 classes), and Pageblocks and Gesturephase (both with 5 classes). 
Experiments were conducted on four datasets: Abalone and Waveform (both with 3 classes), and Pageblocks and Gesturephase (both with 5 classes). 
% 
For each dataset, we split the original data into training and test sets with an 8:2 ratio. 
%
Figure~\ref{fig:lightgbm-results} shows the results, where the vertical axis represents the hyper-volume of test accuracies across all classes, calculated using the reference point at $\*0$. 
%
Note that each objective function is in $[0,1]$ (classification accuracy of each class), and therefore, the volume is also in $[0,1]$ (if all classes achieve accuracy $1$, the volume becomes $1$).
%
As observed in the figure, overall, PFEV shows sufficiently high performance among the compared methods.
% As observed in the figure, PFEV consistently performs well across all datasets compared to other methods.
% %
% This confirms that our approach is effective not only for synthetic functions and benchmark problems but also for practical machine learning hyperparameter optimization tasks. 
% %
% The advantage of PFEV is particularly evident in the Pageblocks and Gesturephase datasets with higher dimensionality (5 classes), which aligns with our previous findings regarding the performance benefits in higher-dimensional objective spaces.


% --------------------------------------------------
% Fig: HPO 
% --------------------------------------------------
\begin{figure}[t!]
 \centering
 
 \subfigure[Abalone (4177 samples, 8 features, 3 classes)]{
 \ig{.2}{./figs/real-data-appendix/HV_train_and_evaluate_abalone_classweight_default_input_dim_3_output_dim_3.pdf}
 }
 ~~~~
 \subfigure[Waveform (5000 samples, 40 features, 3 classes)]{
 \ig{.2}{./figs/real-data-appendix/HV_train_and_evaluate_waveform5000_classweight_default_input_dim_3_output_dim_3.pdf}
 }
 
 \subfigure[Pageblocks (5473 samples, 10 features, 5 classes)]{
 \ig{.2}{./figs/real-data-appendix/HV_train_and_evaluate_pageblocks_classweight_default_input_dim_5_output_dim_5.pdf}
 }
 ~~~~
 \subfigure[Gesturephase (9873 samples, 33 features, 5 classes)]{
 \ig{.2}{./figs/real-data-appendix/HV_train_and_evaluate_gesturephase_classweight_default_input_dim_5_output_dim_5.pdf}
 }
 \caption{Results on hyper-parameter (class-weights) optimization.}
 \label{fig:lightgbm-results}
 % \caption{\red{main-textにParEGO,MOBO-RS,MESMOを追加したもの．このFigを論文に入れる場合，どこかで言及する必要あり．Results on hyper-parameter (class-weights) optimization.}}
 % \label{fig:lightgbm-result-extended}
% \end{figure}
% % --------------------------------------------------
% % Fig: 
% % --------------------------------------------------
% \begin{figure}[t!]
%  \centering   
%  \subfigure[Abalone (4177 samples, 8 features, 3 classes)]{
%  \ig{.2}{./figs/real-data-main/HV_train_and_evaluate_abalone_classweight_default_input_dim_3_output_dim_3.pdf}
%  } 
%  ~~~~~
%  \subfigure[Waveform (5000 samples, 40 features, 3 classes)]{
%  \ig{.2}{./figs/real-data-main/HV_train_and_evaluate_waveform5000_classweight_default_input_dim_3_output_dim_3.pdf}
%  }
%  \subfigure[Pageblocks (5473 samples, 10 features, 5 classes)]{
%  \ig{.2}{./figs/real-data-main/HV_train_and_evaluate_pageblocks_classweight_default_input_dim_5_output_dim_5.pdf}
%  }
%  ~~~~~
%  \subfigure[Gesturephase (9873 samples, 33 features, 5 classes)]{
%  \ig{.2}{./figs/real-data-main/HV_train_and_evaluate_gesturephase_classweight_default_input_dim_5_output_dim_5.pdf}
%  }
%  \caption{Results on hyper-parameter (class-weights) optimization.}
%  \label{fig:lightgbm-results}
% \end{figure}
% --------------------------------------------------
% Fig: MC vs ベイズ推定 Regret比較
% --------------------------------------------------
% \begin{figure}[t!]
 \centering
 \subfigure[$(d, L) = (2, 6)$]{
 % \ig{.22}{./figs/MCvsBayes/RHV_input_dim_2_output_dim_6_length_scale_0.1.pdf}
 \ig{.22}{./figs/MCvsBayes/RHV_input_dim_2_output_dim_6_length_scale_0.1-embed.pdf}
 }
 \subfigure[$(d, L) = (3, 6)$]{
 % \ig{.22}{./figs/MCvsBayes/RHV_input_dim_3_output_dim_6_length_scale_0.1.pdf}
 \ig{.22}{./figs/MCvsBayes/RHV_input_dim_3_output_dim_6_length_scale_0.1-embed.pdf}
 }
 \caption{
 Comparison between two MC estimators \eq{eq:LB-MC} and \eq{eq:LB-MAP} of PFEV using GP-derived synthetic functions.
 % $(d, L)=(2, 6)$ に対して，PFEVのモンテカルロ近似手法（式\eq{eq:LB-MC},式\eq{eq:LB-MAP}） を変更した結果
 }
  \label{fig:mc_vs_bayes_regret}
\end{figure}
% 本節ではGP由来のベンチマーク関数を用いて，式\ref{eq:LB-MC}および式\ref{eq:LB-MAP}で述べたPFEVの
% GPの設定は，\ref{ssec:GPDerivedArtificialFunctions}と同様であり，入出力の次元数は$(d, L) = (2, 6)$である．
% 節で述べたとおり，事前知識を導入したベイズMAPを導入した式\ref{eq:LB-MAP}によるPFEVの結果が良い性能を示した．
% 誌面の都合上結果の計算は割愛するが，他の入出力の次元に関するGP由来の人工関数実験においても，同様に式\ref{eq:LB-MAP}によるPFEVの定式化による結果が良い結果を示した．

% \subsection{ベイズMAP推定の効果検証}
% 本節では，GP由来のベンチマーク関数を用いて，式\ref{eq:LB-MC}および式\ref{eq:LB-MAP}で述べたPFEVの性能を比較する．
% GPの設定は\ref{ssec:GPDerivedArtificialFunctions}と同様とし，入出力の次元数は$(d, L) = (2, 6)$とする．
% 実験結果より，事前知識を導入したベイズMAPを用いる式\ref{eq:LB-MAP}による定式化が良好な性能を示すことが確認された．
% また，他の入出力の次元に関するGP由来の人工関数実験においても，同様に式\ref{eq:LB-MAP}による定式化が優れた結果を示すことを確認している．

% --------------------------------------------------
% \subsection{ベイズMAP推定の効果検証}
\subsection{Comparison of PFEV with Different MC Estimators}

% GP由来の人工関数を用いて式\eq{eq:LB-MC}および式\eq{eq:LB-MAP}でのPFEVの性能を比較する．
By using GP-derived synthetic functions, two estimators of PFEV \eq{eq:LB-MC} and \eq{eq:LB-MAP} are compared.
%
% GPの設定は\ref{ssec:GPDerivedArtificialFunctions}節と同様とし，入出力は$(d, L) = (2, 6)$とする．
The same settings as in Section~\ref{ssec:GPDerivedArtificialFunctions} were used.
% and the input and the output dimensions are $(d, L) = (2, 6)$ and $(d, L) = (3, 6)$. 
%
% 図\ref{fig:mc_vs_bayes_regret}に示す通り，事前知識を導入したベイズMAP\eq{eq:LB-MAP}による定式化が良好な性能を示すことが確認された．
The results of $(d, L) = (2, 6)$ and $(d, L) = (3, 6)$ are shown in Fig.~\ref{fig:mc_vs_bayes_regret}.
%
We see that the MAP-based approximation \eq{eq:LB-MAP} improves the performance compared with \eq{eq:LB-MC}.
%
% また，他の入出力の次元に関するGP由来の人工関数実験においても，同様に式\eq{eq:LB-MAP}による定式化が優れた結果を示すことを確認している．
We confirmed similar results on other GP-derived functions, which is summarized in Fig.~\ref{fig:BayesMAP-boxplot-app} in Appendix~\ref{app:additional_experiments_GP}.
% また，他の入出力の次元に関するGP由来の人工関数実験においても，同様の結果を示すことを確認している．
%
% Further, analysis of MC estimator can be found in Appendix~\ref{app:empirical-study-BayesMAP}.

% {Appendix?}

% --------------------------------------------------
\section{Discussion on Gradient-based Optimization of Acquisition Function}


We employed DIRECT as an optimizer of the acquisition function because it does not require `initial points' unlike the gradient descent that requires the appropriate setting of the initial points (the number of initial points and locations).
%
Our purpose is to focus more on differences of the acquisition functions and to reduce the other factors affecting the performance. 
%
On the other hand, evaluation using gradient-based approaches is also important future work because it is widely used in BO and should have high performance in general. 
%
We partially show comparison with a baseline using the gradient optimization (qLogNEHVI in BoTorch) in Appendix~\ref{app:gradient}.



% Applying a gradient method to the proposed method is an important future work. 
%
Note that the proposed acquisition function (\ref{eq:LB-MAP}) is mostly differentiable, except for the
indicator
$\II(\tilde{\*f}_{\*x} \in \cA_O^{\tilde{\cF}^*_S})$
% I( ~ fx ∈ A~∗FS)O
in 
$\theta_{\mr{MAP}}(\tilde{\*f}_{\*x})$. 
% θMAP( ~ fx)of (8). 
%
We consider that possible approaches are simply ignoring this term in the gradient (regarding the gradient of the indicator as 0) or using a continuous approximation of the gradient. 
%
In the continuous approximation, we replace
$\II(\tilde{\*f}_{\*x} \in \cA_O^{\tilde{\cF}^*_S}) \approx p(\*f \in \cA_O^{\tilde{\cF}^*_S})$, 
where 
$\*f \sim \cN(\tilde{\*f}_{\*x}, \rho \*I)$ 
in which 
$\rho > 0$
% I( ~ fx ∈ A~∗~∗FS) ≈ p(f ∈ AFS) f ∼N( ~ fx
% , where in which , ρI) ρ > 0
is a fixed smoothing parameter. 
%
The right hand side of the approximation is differentiable with respect to 
$\*x$
% x ~ fx
through the similar decomposition to (\ref{eq:decompose_Z_O}) in Appendix~\ref{app:CalcZ} (note that $\tilde{\*f}_{\*x}$ is differential because it is generated from RFM). 
%
This can be interpreted as a counter-part of the standard CDF-based smoothing approximation of an indicator function, extended to the indicator of the Pareto dominated region. 
%
For the calculation, although the cell-based decomposition is required for 
$\cA_O^{\tilde{\cF}_S^*}$,
% AFS
we can reuse the cells created in line 7 of Algorithm~\ref{alg:PFEV}.



% --------------------------------------------------
% \section{まとめ}
\section{Conclusions}

% 本研究では，変分下限最大化に基づく多目的ベイズ最適化を提案した．
We proposed a multi-objective Bayesian optimization acquisition function that is based on variational lower bound maximization.
%
% 二種類の切断から定まる分布の混合を変分下限で最適化することでより適切な変分分布を構成できる．
By combining two normal distributions, defined by under- and over-truncation of Pareto-frontier, we introduced a variational distribution as mixture of these two distributions based on which a lower bound of mutual information can be constructed. 
%
% 実験的には特に目的関数の数が多い場合に，提案法の優位性が確認された．
% Performance superiority was particularly seen in the case of higher dimensional output problems. 
Performance superiority was shown by GP-generated functions and benchmark functions.
%
% 今後の課題としては，パレートフロンティアのサンプルにかかる計算コストの効率化などが挙げられる．
% A current limitation is an extension for the `decoupled' setting (in which each objective function can be observed separately), which is our future work.
A current limitation includes theoretical guarantee of the MI approximation and convergence, which is important open problems for information-theoretic BO.
%
Another possible future direction is to use a more complicated variational distribution. 
%
We employ the simple one parameter ($\lambda$) distribution because $q$ should be estimated based on the $K$ samples, which is usually quite small ($10$ in the experiments). 
%
However, to make the lower bound tight, a more flexible distribution may be required.


\ifdefined\ackn
% --------------------------------------------------
\section*{Acknowledgement} %% 謝辞

% 本研究の一部は科学研究費（23K21696）の補助を受けて行われた．
{This work is partially supported by JSPS KAKENHI (Grant Number 23K21696, 25K03182, 22H00300, and 23K17817), and Data Creation and Utilization Type Material Research and Development Project (Grant No. JPMXP1122712807) of MEXT. 
}
\fi

\ifdefined\impactstate
\section*{Impact Statement}
This paper presents work whose goal is to advance the field of Bayesian optimization. 
%
There are many potential societal consequences of our work, none which we feel must be specifically highlighted here.
\fi

% --------------------------------------------------
% References
% --------------------------------------------------


\bibliography{ref}

\biblstyle
 

% --------------------------------------------------
\clearpage

% --------------------------------------------------
% \section{Appendix}
\appendix

% \remove{ % ibismlでは消す
% % --------------------------------------------------
% \section{獲得関数最適化について}
% }

% \remove{
% \section{Derivation of $L(\*x, \lambda)$ for $q_\lambda$}

% From the fist line of \eq{eq:VLB-lambda}, $L(\*x, \lambda)$ can be written as
% {\tiny
% \begin{align}	
% % &
% % L(\*x, \lambda)
% % \notag
% % \\ % ---
% % & =
% % \EE_{\cF^*, \*f_{\*x}} \sbr{
% % \log \rbr{ 
% % \frac{ \lambda q_U(\*f_{\*x} \mid \cF^*_S) + (1 - \lambda) q_O(\*f_{\*x} \mid \cF^*_S) }
% % { p(\*f_{\*x}) } 
% % } } \notag
% % \\ % ---
% % & =
% \EE_{\cF^*, \*f_{\*x}} \sbr{
% \log \rbr{ 
% \frac{ 
% % \lambda q_U(\*f_{\*x} \mid \cF^*_S) + (1 - \lambda) q_O(\*f_{\*x} \mid \cF^*_S) 
% \rbr{ \lambda / Z_U^{\cF^*_S}(\*x) + (1 - \lambda) / Z_O^{\cF^*_S}(\*x) } p(\*f_{\*x}) 
% \II( \*f_{\*x} \in \cA_O^{\cF^*_S} ) 
% + 
% \lambda p(\*f_{\*x}) / Z_U^{\cF^*_S}(\*x) 
% \II( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} )
% }
% { p(\*f_{\*x}) } 
% } } \notag
% %\\ % ---
% \end{align}}%
% Since 
% $\II( \*f_{\*x} \in \cA_O^{\cF^*_S} )$
% and
% $\II( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} )$
% are mutually exclusive, 
% $L(\*x, \lambda)$
% can be written as the last line of
% \eq{eq:VLB-lambda}.
% }

% --------------------------------------------------
% \subsection{下限の非負性}
\section{Proof of Remark~\ref{rem:lower-bound-of-VLB}}
\label{app:lower-bound-of-VLB}

% 式\eq{eq:MaxVLB}の下限は$\lambda = 1$の場合を使って抑えている．
The lower bound of \eq{eq:MaxVLB} is derived by using the case of $\lambda = 1$:
%
\begin{align*}
 & \max_{\lambda \in (0,1]} 
 % L(\*x, \lambda)
 \mr{LB}(\*x, \lambda)
 \\
 & \geq 
 \mr{LB}(\*x, 1)
 \\
 & 
 = 
 \EE_{\cF^*, \*f_{\*x}}
 \sbr{
 \log \rbr{ \frac{ q_U(\*f_{\*x} \mid \cF_S^*) }{p(\*f_{\*x})} }
 }
 \\
 & = 
 - \EE_{\cF^*}\sbr{
 \int_{\cA_U^{\cF_S^*}} p(\*f_{\*x} \mid \cF^*)
 \log Z_U^{\cF^*_S}(\*x)
 \mr{d} \*f_{\*x}}
 \\
 & = 
 - \EE_{\cF^*}\sbr{ \log Z_U^{\cF^*_S}(\*x) }
 \\
 & = 
 - \EE_{\cF^*}\sbr{ \log (1 - p( \*f_{\*x} \notin \cA_U^{\cF_S^*}) )}
 \\
 & 
 \geq
 \EE_{\cF^*}\sbr{ p( \*f_{\*x} \notin \cA_U^{\cF_S^*}) }
 > 0
\end{align*}

% --------------------------------------------------
% \section{正規化定数$Z_O^{\tilde{\cF}^*_S}, Z_U^{\tilde{\cF}^*_S}$の計算}
\section{Computations of $Z_O^{\tilde{\cF}^*_S}$ and $Z_U^{\tilde{\cF}^*_S}$}
\label{app:CalcZ}

% 本節では，正規化定数$Z_O^{\tilde{\cF}^*_S}, Z_U^{\tilde{\cF}^*_S}$の計算方法について説明する．
%
% まず，過剰な切断による正規化定数
First, we consider the normalization constant of PFTN-O
$Z_O^{\tilde{\cF}^*_S} = p(\*f_{\*x} \in \cA_O^{\cF^*_S})$.
% $Z_O^{\tilde{\cF}^*_S} = p(\*f_{\*x} \in \cA_O^{\cF^*_S})$
% を考える．
% は以下のように定義される：
% \begin{align*}
%  Z_O^{\tilde{\cF}^*_S} \coloneq \operatorname{Pr}\left(\boldsymbol{f}_{\boldsymbol{x}} \in \cA_O^{\tilde{\cF}^*_S} \mid \mathcal{D}\right)
% \end{align*}
%
% この計算のため，$\tilde{\cF}^*_S$に支配されている領域
% $\cA_O^{\tilde{\cF}^*_S}$
% を
% $C \in \NN$
% 個の互いに素な超直方体に分割する．
We decompose 
$\cA_O^{\tilde{\cF}^*_S}$
into disjoint hyper-rectangles, denoted as
$\cA_O^{\tilde{\cF}^*_S} = \cC_1 \cup \cC_2 \cup \ldots \cup \cC_C$,
where 
$\cC_i$ is a hyper-rectangle and $C$ is the number of hyper-rectangles.
%
% この領域は
% $Z_O^{\tilde{\cF}^*_S}$は，2 (c) に示すように、
% 互いに重ならないセルとして 
% $Z_O^{\tilde{\cF}^*_S}=\mathcal{C}_{1} \cup \mathcal{C}_{2} \cup \ldots \cup \mathcal{C}_{M}$ 
% $\cA_O^{\tilde{\cF}^*_S} = \cC_1 \cup \cC_2 \cup \ldots \cup \cC_C$ 
% となる．
%
% このような分割を得るアルゴリズムはパレート超体積計算などでよく研究されており，例えばquick hypervolume（QHV）\citep{Russo2014-quick}を使うことで計算できる．
Algorithms decomposing a dominated region have been studied in the context of the Pareto hyper-volume computation. 
%
We use quick hypervolume (QHV) \citep{Russo2014-quick}, used also in PFES.
%
% 各超直方体$\cC_i$ ($i=1, \ldots, C$)は，$L$次元の直積区間として以下のように表される：
Each hyper-rectangle $\cC_i$ is written as
\begin{align*}
\cC_i = \left(\ell_i^1, u_i^1 \right] \times \left(\ell_i^2, u_i^2 \right] \times \ldots \times \left(\ell_i^L, u_i^L \right], 
\end{align*}
where $\ell_i^l$ and $u_i^l$ are the smallest and largest values in the $l$-th dimension of the $i$-th hyper-rectangle.
%
% この分割は観測データ$\{\*y_i\}_{i=1}^{n}$ではなく，現在のGPRモデルによって生成された$\tilde{\cF}^*_S$に基づいて行われることに注意されたい．
%
% 目的関数間の独立性を用いると，$Z_O^{\tilde{\cF}^*_S}$は以下のように解析的に計算できる：
From the independence of the objective functions, $Z_O^{\tilde{\cF}^*_S}$ can be easily computed by 
\begin{align}
 Z_O^{\tilde{\cF}^*_S}
 & =\sum_{i=1}^{C} 
 \int_{\cC_i} 
 p(\*f_{\*x} ) \mathrm{d} \*f_{\*x}  
 \notag \\
 & = \sum_{i=1}^{C} \prod_{l=1}^{L} \int_{\ell_i^l}^{u_i^l} 
 p(f_{\*x}^l) \mathrm{d} f_{\*x}^l  
 \notag \\
 & = \sum_{i=1}^{C} \prod_{l=1}^L 
 \rbr{ \Phi(\bar{\alpha}_{i,l}) - \Phi(\underline{\alpha}_{i,l}) },
 \label{eq:decompose_Z_O}
 % & = \sum_{i=1}^{C} \prod_{l=1}^L Z_{il},
\end{align}
where 
% $Z_{il} = \Phi(\bar{\alpha}_{i,l}) - \Phi(\underline{\alpha}_{i,l})$ in which
$\underline{\alpha}_{i,l} = (\ell_i^l - \mu_l(\*x))/\sigma_l(\*x)$
and
$\bar{\alpha}_{i,l} = (u_i^l - \mu_l(\*x))/\sigma_l(\*x)$,
and $\Phi$ is the cumulative distribution function of the standard normal distribution.
% ただし，各次元$l$における超直方体$\cC_i$の確率積分値
% $Z_{il} = \Phi(\bar{\alpha}_{i,l}) - \Phi(\underline{\alpha}_{i,l})$
% であり，
% $\underline{\alpha}_{i,l} = (\ell_i^l - \mu_l(\*x))/\sigma_l(\*x)$
% および
% $\bar{\alpha}_{i,l} = (u_i^l - \mu_l(\*x))/\sigma_l(\*x)$
% とする．
%
% ただし，$\Phi(\cdot)$は標準正規分布の累積分布関数とする．
% この定義により，各次元での確率計算を標準化された形式で効率的に行うことができる．


% 次に，保守的な切断による正規化定数$Z_U^{\tilde{\cF}^*_S}$の計算方法について説明する．
Next, we consider $Z_U^{\tilde{\cF}^*_S}$ that can be re-written as
%
% この正規化定数は以下のように書き換えることができる：
% \begin{align*}
% Z_U^{\tilde{\cF}^S} \coloneqq \operatorname{Pr}\left(\boldsymbol{f}{\boldsymbol{x}} \in \cA_U^{\tilde{\cF}^S} \mid \mathcal{D}\right) = 1 - \operatorname{Pr}\left(\boldsymbol{f}{\boldsymbol{x}} \in \cA_O^{\tilde{\cF}^*_S} \mid \mathcal{D}\right)
% \end{align*}
\begin{align*}
Z_U^{\tilde{\cF}^*_S} 
& = p \rbr{ \*f_{\*x} \in \cA_U^{\tilde{\cF}^*_S} }
\\
& = 1 - p \rbr{ \*f_{\*x} \notin \cA_U^{\tilde{\cF}^*_S} }
\\
& = 1 - p\rbr{- \*f_{\*x} \preceq \{ - \*f \mid \*f \in \tilde{\cF}^*_S \}}. 
\end{align*}
% 最後の式は，$\tilde{\cF}^*_S$の符号を反転して表現し直すことで「支配されている領域」として領域$\*f_{\*x} \notin \cA_U^{\tilde{\cF}^*_S}$を等価な別表現に直している．
In the last equation, the region 
$\*f_{\*x} \notin \cA_U^{\tilde{\cF}^*_S}$
is re-written by flipping the sign of $\tilde{\cF}^*_S$ in such a way that the region is written as a ``dominated region''.
%
% これにより，$Z_O^{\tilde{\cF}_S^*}$と同様にQHVのような，パレートフロンティアに「支配されている領域」を分割するアルゴリズムを使って計算することができる．
This enables us to use QHV, which decomposes a ``dominated region'' into hyper-rectangles, for the computation of 
$p(- \*f_{\*x} \preceq \{ - \*f \mid \*f \in \tilde{\cF}^*_S \})$ 
based on almost the same way as \eq{eq:decompose_Z_O}. 
% この計算では，領域$\cA_U^{\tilde{\cF}^*_S}$に対して直接的に計算を行うのではなく，全空間から
% $p \rbr{ \*f_{\*x} \notin \cA_U^{\tilde{\cF}^*_S} }$
% を引く．
%
% この方法により，既に計算した$Z_O^{\tilde{\cF}^*_S}$の結果を利用することができ，効率的な計算が可能となる．
% 具体的な計算手法については，\citep{Suzuki2020-multi}と同様の方法で行うことができる．

% $p\rbr{- \*f_{\*x} \preceq \{ - \*f \mid \*f \in \tilde{\cF}^*_S \}}$

% $- \*f_{\*x} \preceq \{ - \*f \mid \*f \in \tilde{\cF}^*_S \}$

% 空間
% $\*f_{\*x} \notin \cA_U^{\tilde{\cF}^*_S}$
% は符号を反転すると
% $
% - \*f_{\*x}
% \preceq 
% $



% --------------------------------------------------
% \section{獲得関数の$\lambda$に関する凸性}
% \section{Concavity of Acquisition Function about $\lambda$}
\section{Properties about Maximization of $\lambda$}
\label{app:lambda-convexity}

We first show the concavity.
% 表記の簡易化のため
% \eq{eq:LB-MAP}
% と
% \eq{eq:LB-MC}
% を一般化して
To simplify the notation, we unify \eq{eq:LB-MAP} and \eq{eq:LB-MC} as
\begin{align*}
 \wh{\mr{LB}}(\*x,\*\lambda) &= 
 \frac{1}{K} \sum_{(\tilde{\cF}^*_S, \tilde{\*f}) \in F}
 \log\rbr{ 
 \frac{ \lambda }{ Z_U } + \frac{ 1 - \lambda }{ Z_O }
 } 
 \xi(\tilde{\*f_{\*x}})
 \nonumber \\
 & \qquad 
 +
\log \rbr{
 % \frac{ \lambda }{ Z_U^{\tilde{\cF}^*_S} }
 \frac{ \lambda }{ Z_U }
}
 (1 - \xi(\tilde{\*f_{\*x}})),
\end{align*}
% とする．
%
% ただし，
% $Z_U = Z_U^{\cF^*_S}(\*x)$
% と
% $Z_O = Z_O^{\cF^*_S}(\*x)$
% とし，$\xi(\tilde{\*f_{\*x}}) \in [0,1]$は
% \eq{eq:LB-MAP}なら
% $\theta_{\mr{MAP}}(\tilde{\*f_{\*x}})$，
% \eq{eq:LB-MC}なら
% $\II( \tilde{\*f_{\*x}} \in \cA_O^{\tilde{\cF}^*_S} )$
% とする．
where 
$Z_U = Z_U^{\tilde{\cF}^*_S}(\*x)$, 
$Z_O = Z_O^{\tilde{\cF}^*_S}(\*x)$, 
and 
$\xi(\tilde{\*f_{\*x}}) = \theta_{\mr{MAP}}(\tilde{\*f_{\*x}})$ 
when \eq{eq:LB-MAP}, and 
$\xi(\tilde{\*f_{\*x}}) = \II( \tilde{\*f_{\*x}} \in \cA_O^{\tilde{\cF}^*_S} )$
when \eq{eq:LB-MC}. 
%
% \red{
% % この関数を$\lambda$で微分すると以下を得る．
% Taking derivative with respect to $\lambda$, we obtain
% \begin{align*}
%  \pd{\wh{L}(\*x,\lambda)}{\lambda} &= 
%  \frac{1}{K} \sum_{(\tilde{\cF}^*_S, \tilde{\*f}) \in F}
%  \frac{ % 1
%  Z_O - Z_U
%  }{
%  \lambda (Z_O - Z_U) + Z_U
%  % \frac{ \lambda }{ Z_U } + \frac{ 1 - \lambda }{ Z_O }
%  } 
%  \xi(\tilde{\*f_{\*x}})
%  \\
%  & + \frac{ 1 }{ \lambda }
%  (1 - \xi(\tilde{\*f_{\*x}})) 
% \end{align*}
% % この関数を再度$\lambda$で微分すると以下を得る．
% }
The second derivative is  
%
% この関数を$\lambda$で$2$回微分すると以下を得る．
\begin{align*}
 \pd{^2 \wh{\mr{LB}}(\*x,\lambda)}{\lambda^2} &= 
 \frac{1}{K} \sum_{(\tilde{\cF}^*_S, \tilde{\*f}) \in F}
 -
 \rbr{
 \frac{
 % \frac{ 1 }{ Z_U } - \frac{ 1 }{ Z_O }
 Z_O - Z_U
 }{ 
 % \frac{ \lambda }{ Z_U } + \frac{ 1 - \lambda }{ Z_O }
 \lambda (Z_O - Z_U) + Z_U
 }
 }^2
 \xi(\tilde{\*f_{\*x}})
 \\ 
 & 
 \qquad -
 % \frac{
 % \rbr{
 % \frac{ 1 }{ Z_U }
 % }^2
 % }{
 % \rbr{
 % \frac{ \lambda }{ Z_U }
 % }^2
 %  }
% \lambda^2
% (1 - \xi(\tilde{\*f_{\*x}}))  
 \frac{ 1 }{ \lambda^2 }
 (1 - \xi(\tilde{\*f_{\*x}})) 
 \leq 0. 
\end{align*}
Thus, we see concavity.  
% さらに通常は$Z_U > Z_O$であるため（$A_O^{\cF_S^*} \subset A_U^{\cF_S^*}$なので），このとき最後の不等式は等号を含まない形で成立する(つまり狭義凸関数)．
% Further, since usually we have $Z_U > Z_O$ (from $A_O^{\cF_S^*} \subset A_U^{\cF_S^*}$), the last inequality becomes $<$ in this case (i.e., strictly concave). 
%
% 特に，$\lambda$に関する$1$次元最適化のみを考える場合はこの凸性を考慮することで効率化が可能である（複数局所回の可能性を考慮する必要がないので，例えば適当な初期点から始めた勾配ベース最適化により$\lambda$に関する最適解に収束させることができる）．


% \red{
% % また，１階微分で$\lambda = 1$とすると
% If we set $\lambda = 1$ in the first derivative, we see
% \begin{align*}
%  \pd{\wh{L}(\*x,1)}{\lambda} &= 
%  \frac{1}{K} \sum_{(\tilde{\cF}^*_S, \tilde{\*f}) \in F}
%  \rbr{1 - \frac{Z_U}{Z_O}} \xi(\tilde{\*f_{\*x}})
%  + 1 - \xi(\tilde{\*f_{\*x}})
%  \\
%  &=
%  \frac{1}{K} \sum_{(\tilde{\cF}^*_S, \tilde{\*f}) \in F}
%  \rbr{ 1 -  \frac{Z_U}{Z_O} \xi(\tilde{\*f_{\*x}}) }.
% \end{align*}
% % であり，仮に
% %$\xi(\tilde{\*f_{\*x}}) = \hat{p} = Z_O/Z_U$
% %のように近似値をそのまま代入すると
% %$\wh{L}(\*x,1) = 0$
% %となることがわかる
% When we directly use $\hat{p}$ (i.e., $\xi(\tilde{\*f_{\*x}}) = \hat{p} = Z_O/Z_U$), we obtain 
% $\pd{\wh{L}(\*x,1)}{\lambda} = 0$．
% %
% % つまりこのとき，常に$\lambda = 1$が変分下限の最大化点となる．
% This means that $\lambda = 1$ is always the maximizer of the lower bound in this special case.
% }

{
Further, in the case of \eq{eq:LB-MAP}, we can show that the optimal $\lambda$ should exist for $\max_{\lambda \in (0, 1]} \wh{\mr{LB}}(\*x,\lambda)$ though $\lambda$ has a left open interval as a domain.  
%
First, we can derive 
$\hat{p} \in (0,1)$ 
from its definition 
$\hat{p} = Z_O^{\tilde{\cF}^*_S}(\*x) / Z_U^{\tilde{\cF}^*_S}$. 
%
Since $\*f_{\*x}$ is the Gaussian distribution, 
$Z_O^{\tilde{\cF}^*_S}(\*x) = p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S}) \in (0,1)$
and 
$Z_O^{\tilde{\cF}^*_S}(\*x) < Z_U^{\tilde{\cF}^*_S}(\*x) = p(\*f_{\*x} \in \cA_U^{\tilde{\cF}^*_S}) \in (0,1)$.
%
Here, we used 
$\emptyset \neq \cA_O^{\tilde{\cF}^*_S} \subset \cA_U^{\tilde{\cF}^*_S} \subset \RR^L$
(neither 
$\cA_O^{\tilde{\cF}^*_S}$ 
nor 
$\cA_U^{\tilde{\cF}^*_S}$
is the empty set or the entire output space, and 
$\cA_O^{\tilde{\cF}^*_S} \subset \cA_U^{\tilde{\cF}^*_S}$
holds as far as the sampled Pareto frontier set 
$\tilde{\cF}_S^{*}$
is finite while the true Pareto frontier is continuous which is our problem setting). 
% Z_O^{\tilde{\cF}^*_S}(\*x) / Z_U^{\tilde{\cF}^*_S}(\*x) 
%
Therefore, we see $\theta_{\mr{MAP}} \in (0,1)$. 
%
When $\lambda \rightarrow 0$, the second term of \eq{eq:LB-MAP} goes to $\log 0$ (from the definition of $\eta_{\lambda}^{\tilde{\cF}_S^*}$).
%
On the other hand, the first term is finite even when $\lambda \rightarrow 0$.
%
As a result, if $\lambda \rightarrow 0$, we see \eq{eq:LB-MAP} goes to $- \infty$. 
}

Figure~\ref{fig:lambda-transition} shows the transition of $\lambda$ during BO iterations (the average and standard deviation of $10$ runs) for a GP-derived synthetic function ($d = 3, L = 4$). 
%
We see that $\lambda$ takes intermediate values in $(0,1]$, indicating that under- and over-truncated distributions are indeed mixed during BO iterations. 
%
As far as we have examined, no consistent increasing or decreasing tendency has been observed during iterations.

% --------------------------------------------------
% Fig: 
% --------------------------------------------------
\begin{figure}
 \centering

 \ig{.4}{./figs/lambda/lambda-mean.pdf}

 \caption{Transition of selected $\lambda$ for GP-derived synthetic function ($d = 3, L = 4$).}
 \label{fig:lambda-transition}
\end{figure}

% \remove{ % IBISMLでは消す
% --------------------------------------------------
% \section{$p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \cF^*)$の近似値を事前分布に反映したベイズ推定によるMCの改善}
% \section{事前分布を使った変分下限のモンテカルロ推定}
\section{Combining Prior Knowledge in MC Estimator}

% --------------------------------------------------
% \subsection{ベイズ推定の導出}
\subsection{Derivation of MAP}
\label{app:BayesMAP}

% $\theta$ の事前分布としてベータ分布を考える：$\theta \sim \mr{beta}(a, b)$．
We use the beta distribution for the prior $\theta \sim \mr{Beta}(a, b)$. 
%
% 密度関数は
The density function is 
\begin{align*}
p(\theta) = \frac{\theta^{a - 1} (1 - \theta)^{b - 1}}{ B(a,b) }. 
\end{align*}
% と表される．
% 近似 
% $\theta \approx p(\*f_{\*x} \in \cA_O^{\cF^*_S} \mid \*f_{\*x} \in \cA_U^{\tilde{\cF}^*_S}) = Z_O^{\cF^*_S}(\*x) / Z_U^{\cF^*_S}(\*x) \coloneqq \hat{p}$ 
% に対して，$a - 1 = r \hat{p}$ および $b - 1 = r (1 - \hat{p})$ とすることを考える．ただし，$r \geq 0$ とする．
Using the approximation $\theta \approx \hat{p}$, we set $a - 1 = r \hat{p}$ and $b - 1 = r (1 - \hat{p})$, where $r \geq 0$ is a parameter.
%
% このように $a$ と $b$ を設定すると $p(\theta)$ は $\hat{p}$ に最頻値を持つようになる．
This sets the mode of $p(\theta)$ as $\hat{p}$.
%
% 図\ref{fig:beta-pdf}に示す通り $r$ は大きいほど $\hat{p}$ に強いピークを持つ．
As shown in Fig.~\ref{fig:beta-pdf}, a larger $r$ has a stronger peak at $\hat{p}$. 
%
% また，$r = 0$ で $[0,1]$ 内で一様となる．
When $r = 0$, $p(\theta)$ becomes uniform in $[0,1]$.
% なお，ベータ分布は平均値(mean)と最頻値(map)が異なることに注意が必要である．最頻値を考えると $a = 1, b = 1$ で事後分布がモンテカルロと一致するが，平均値の場合は $a = 0, b = 0$ でモンテカルロに一致する（{はずである}）．

% --------------------------------------------------
% Fig: ベータ分布
% --------------------------------------------------
\begin{figure}[t]	
 \begin{center}
  \ig{.25}{./figs/beta-pdf.pdf}
 \end{center}
 \caption{
 Density functions of the beta distribution when $\hat{p} = 0.8$.
 % $\hat{p} = 0.8$
 % とし，
 % $a - 1 = r \hat{p}, b - 1 = r (1 - \hat{p})$
 % としたときのベータ分布の密度関数．
 %
 % どの$r$でも最頻値は$0.8$になる．
 For all $r$, the mode is $0.8$. 
 }
 \label{fig:beta-pdf}
\end{figure}

% 一般に，事前分布にベータ分布を持つベルヌーイ分布の事後分布は $\mr{Beta}(a+m,b+\ell)$ となることが知られている．
% ただし，$m$ がベルヌーイ試行における成功回数，$\ell$ が失敗回数である．
The posterior of the beta distribution with the Bernoulli distribution likelihood is
$\mr{Beta}(a+m,b+\ell)$, 
where $m$ is the number of `success' and $\ell$ is the number of `fail' in Bernoulli trials.
%
% 今，真の確率 
% $p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \cF^*)$ 
% のベルヌーイ分布からサンプルを1点計測していると解釈できる（ある $\cF^*$ のときに $\*f_{\*x} \in \cA_O^{\cF^*_S}$ であったかどうか）．
We can interpret that
$\II(\*f_{\*x} \in \cA_O^{\cF^*_S})$
is a sample from the Bernoulli distribution with the probability
$p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \cF^*)$. 
%
% そのため 
% $m = \II(\*f_{\*x} \in \cA_O^{\cF^*_S})$，
% $\ell = 1 - \II(\*f_{\*x} \in \cA_O^{\cF^*_S})$ 
% と考えることができる．
% 事後分布 $\mr{Beta}(a+m,b+\ell)$ の最頻値を考えると
%
Therefore, we set
$m = \II(\*f_{\*x} \in \cA_O^{\cF^*_S})$
and 
$\ell = 1 - \II(\*f_{\*x} \in \cA_O^{\cF^*_S})$,
from which the mode of the posterior $\mr{Beta}(a+m,b+\ell)$ can be derived as 
{\small
\begin{align*}
\theta_{\mr{MAP}} & = 
\frac{a - 1 + m}{a - 1 + m + b -1 + \ell}
\\
& = 
\frac{r \hat{p} + \II(\*f_{\*x} \in \cA_O^{\cF^*_S})}
{r \hat{p} + \II(\*f_{\*x} \in \cA_O^{\cF^*_S}) + r (1 - \hat{p}) + (1 - \II(\*f_{\*x} \in \cA_O^{\cF^*_S}))}
\\
& = 
\frac{r \hat{p} + \II(\*f_{\*x} \in \cA_O^{\cF^*_S})}
{r + 1}.
\end{align*}}%
% となる．
%
% これは $r = 0$ とすると $\theta_{\mr{MAP}} = \II(\*f_{\*x} \in \cA_O^{\cF^*_S})$ となり，ベイズ的な推定をしないモンテカルロ推定と一致する．
%
% 本文では $r = 1$ とした．
In the main text, we employ $r = 1$.
%

% MC with Bayes MAPでは近似値 $\hat{p}$ へのバイアスが存在する．
The lower bound estimation by MAP \eq{eq:LB-MAP} can have an estimation bias caused by the approximation $\hat{p}$, though it is almost negligible when $K$ is a typical setting (such as $K = 10$).
%
% これは，各 $\cF^*_S$ に対して，対応する $\*f_{\*x}$ は1サンプルしかないことに起因している．
This bias occurs because we only have one $\tilde{\*f}_{\*x}$ for each corresponding
$\tilde{\cF}^*_S$.
%
% そのため，それぞれの $\theta_{\mr{MAP}}$ はサンプリング数を増やしても事前分布の影響力が弱まらず，$\hat{p}$ へのバイアスが残る．
Therefore, in each $\theta_{\mr{MAP}}$, the effect of the prior remains even when $K$ is large. 
%
% そこで $r$ をサンプル数 $K$ が増えると $r \rightarrow 0$ に減衰するように設定することで，通常のモンテカルロと同様の結果に収束させることができる．
We can easily avoid this bias by setting $r$ so that it decreases $r \rightarrow 0$ when $K$ increases, by which the estimator \eq{eq:LB-MAP} converges to the usual MC estimator \eq{eq:LB-MC}. 
%
In Appendix~\ref{app:empirical-study-BayesMAP}, we show that, in practice, the MAP-based approach has an advantage for small $K$ setting.

% --------------------------------------------------
% \subsection{ベイズ推定の分散解析}
\subsection{Analyzing Variance}
\label{app:variance-BayesMAP}

% 式\eq{eq:LB-MAP}を以下のように書き換える
We re-write the estimator of the lower bound \eq{eq:LB-MAP} as
\begin{align*}
 \frac{1}{K} \sum_{(\tilde{\cF}^*_S, \tilde{\*f}) \in F}
 a(\tilde{\cF}^*_S)
 \xi(\tilde{\*f_{\*x}})
 % \theta_{\mr{MAP}}(\tilde{\*f}_{\*x}) 
 +
 b(\tilde{\cF}^*_S).
\end{align*}
where 
$a(\tilde{\cF}^*_S) = 
\log\rbr{ 
\frac{ \lambda }{ Z_U^{\tilde{\cF}^*_S}(\*x) } + \frac{ 1 - \lambda }{ Z_O^{\tilde{\cF}^*_S}(\*x) }
} - 
\log \rbr{
\frac{ \lambda }{ Z_U^{\tilde{\cF}^*_S}(\*x) }
}$,
$b(\tilde{\cF}^*_S) = 
\log \rbr{
\frac{ \lambda }{ Z_U^{\tilde{\cF}^*_S}(\*x) }
}$,
and
$\xi(\tilde{\*f_{\*x}}) \in [0,1]$
is $\theta_{\mr{MAP}}(\tilde{\*f_{\*x}})$ when \eq{eq:LB-MAP}
and is 
$\II( \tilde{\*f_{\*x}} \in \cA_O^{\tilde{\cF}^*_S} )$
when
\eq{eq:LB-MC}.
% ただし，
% $a(\tilde{\cF}^*_S) = 
% \log\rbr{ 
% \frac{ \lambda }{ Z_U^{\tilde{\cF}^*_S}(\*x) } + \frac{ 1 - \lambda }{ Z_O^{\tilde{\cF}^*_S}(\*x) }
% } - 
% \log \rbr{
% \frac{ \lambda }{ Z_U^{\tilde{\cF}^*_S}(\*x) }
% }$
% 及び
% $b(\tilde{\cF}^*_S) = 
% \log \rbr{
% \frac{ \lambda }{ Z_U^{\tilde{\cF}^*_S}(\*x) }
% }$
% であり，
% $\xi(\tilde{\*f_{\*x}}) \in [0,1]$
% は\eq{eq:LB-MAP}なら
% $\theta_{\mr{MAP}}(\tilde{\*f_{\*x}})$，
% \eq{eq:LB-MC}なら
% $\II( \tilde{\*f_{\*x}} \in \cA_O^{\tilde{\cF}^*_S} )$
% とする．
%
% この推定量の分散を考えると，モンテカルロサンプルの独立性及びlaw of total varianceより以下のように分解できる． 
By using independence of the MC samples and law of total variance, the variance of this estimator is decomposed as follows:
{\small
\begin{align}
 & \VV_{\tilde{\cF}^*, \tilde{\*f}}
 \sbr{
 \frac{1}{K} \sum_{(\tilde{\cF}^*_S, \tilde{\*f}) \in F}
 a(\tilde{\cF}^*_S)
 \xi(\tilde{\*f_{\*x}})
 +
 b(\tilde{\cF}^*_S)
 }
 \notag \\ % ---
 & = 
 \frac{1}{K} 
 % \sum_{(\tilde{\cF}^*_S, \tilde{\*f}) \in F}
 \EE_{\tilde{\cF}^*}
 \VV_{\tilde{\*f} \mid \tilde{\cF}^*}
 \sbr{
 a(\tilde{\cF}^*_S)
 \xi(\tilde{\*f_{\*x}})
 +
 b(\tilde{\cF}^*_S)
 }
 \notag \\
 & \qquad 
 + 
 \frac{1}{K} 
 % \sum_{(\tilde{\cF}^*_S, \tilde{\*f}) \in F}
 \VV_{\tilde{\cF}^*}
 \EE_{\tilde{\*f} \mid \tilde{\cF}^*}
 \sbr{
 a(\tilde{\cF}^*_S)
 \xi(\tilde{\*f_{\*x}})
 +
 b(\tilde{\cF}^*_S)
 }
 \notag \\ % ---
 & = 
 \frac{1}{K} \biggl\{
 \EE_{\tilde{\cF}^*} 
 \sbr{
 a(\tilde{\cF}^*_S)^2
 \VV_{\tilde{\*f} \mid \tilde{\cF}^*} \sbr{
 \xi(\tilde{\*f_{\*x}})
 }}
 +
 \EE_{\tilde{\cF}^*} 
 \sbr{
 b(\tilde{\cF}^*_S)
 }
 \notag \\
 & \qquad 
 + 
 \VV_{\tilde{\cF}^*} 
 \sbr{
 a(\tilde{\cF}^*_S)
 \EE_{\tilde{\*f} \mid \tilde{\cF}^*} \sbr{
 \xi(\tilde{\*f_{\*x}})
 }
 +
 b(\tilde{\cF}^*_S)
 }
 \biggr\}
 \label{eq:decomposed_variance}
\end{align}}%
%
% 式\eq{eq:decomposed_variance}について一項目の中で$\xi$によって変化するのは
% $\VV_{\tilde{\*f} \mid \tilde{\cF}^*} \sbr{ \xi(\tilde{\*f_{\*x}}) }$
% である．
In the first term of \eq{eq:decomposed_variance}, only
$\VV_{\tilde{\*f} \mid \tilde{\cF}^*} \sbr{ \xi(\tilde{\*f_{\*x}}) }$
changes depending on $\xi$.
%
From
\begin{align*}
 \VV_{\tilde{\*f} \mid \tilde{\cF}^*} \sbr{ 
 \theta_{\mr{MAP}}(\tilde{\*f_{\*x}})
 }
 =
 \VV_{\tilde{\*f} \mid \tilde{\cF}^*} \sbr{ 
 \II( \tilde{\*f_{\*x}} \in \cA_O^{\tilde{\cF}^*_S} )
 } / 4,
\end{align*}
% であるため，MAPを使うことで分散が$1/4$になることがわかる．
we see that MAP makes the variance of the first term $1/4$.
%
% 第二項はMAPを使うかどうかに依存せず同じ項である．
The second term in \eq{eq:decomposed_variance} does not change depending on $\xi$.
%
% MAPの場合，式\eq{eq:decomposed_variance}の第三項は
In the case of the MAP estimate, the third term in \eq{eq:decomposed_variance} is
\begin{align*}
 & 
 \VV_{\tilde{\cF}^*} 
 \sbr{
 a(\tilde{\cF}^*_S)
 \EE_{\tilde{\*f} \mid \tilde{\cF}^*} \sbr{
 \xi(\tilde{\*f_{\*x}})
 }
 +
 b(\tilde{\cF}^*_S)
 } 
 \\ % ---
 & =
 \VV_{\tilde{\cF}^*} 
 \sbr{
 a(\tilde{\cF}^*_S)
 \EE_{\tilde{\*f} \mid \tilde{\cF}^*} \sbr{
 \frac{\hat{p} + \II( \tilde{\*f_{\*x}} \in \cA_O^{\tilde{\cF}^*_S} ) }{2}
 }
 +
 b(\tilde{\cF}^*_S)
 } 
 \\ % ---
 & =
 \VV_{\tilde{\cF}^*} 
 \sbr{
 a(\tilde{\cF}^*_S)
 \frac{\hat{p} + p( \tilde{\*f_{\*x}} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{\cF}^* ) }{2}
 +
 b(\tilde{\cF}^*_S)
 }.
 % \\ % ---
 % & =
 % \VV_{\tilde{\cF}^*} 
 % \sbr{
 % a(\tilde{\cF}^*_S)
 % p( \tilde{\*f_{\*x}} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{\cF}^* )
 % +
 % b(\tilde{\cF}^*_S)
 % +
 % a(\tilde{\cF}^*_S) \frac{\hat{p} - p( \tilde{\*f_{\*x}} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{\cF}^* ) }{2}
 % }  
\end{align*}
% であるが，
% $\hat{p} \approx p( \tilde{\*f_{\*x}} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{\cF}^* )$
% であればこの項は近似的にモンテカルロ設定
% $\xi(\tilde{\*f_{\*x}}) = \II( \tilde{\*f_{\*x}} \in \cA_O^{\tilde{\cF}^*_S} ) $の場合の値
% $\VV_{\tilde{\cF}^*} 
%  \sbr{
%  a(\tilde{\cF}^*_S)
%  p( \tilde{\*f_{\*x}} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{\cF}^* ) 
%  +
%  b(\tilde{\cF}^*_S)
%  }$
% と近しいとみなせる．
If 
$\hat{p} \approx p( \tilde{\*f_{\*x}} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{\cF}^* )$,
this should be similar to
$\VV_{\tilde{\cF}^*} 
 \sbr{
 a(\tilde{\cF}^*_S)
 p( \tilde{\*f_{\*x}} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{\cF}^* ) 
 +
 b(\tilde{\cF}^*_S)
 }$,
which is the variance in the case of
$\xi(\tilde{\*f_{\*x}}) = \II( \tilde{\*f_{\*x}} \in \cA_O^{\tilde{\cF}^*_S} ) $.
%
% よって，この仮定が成立するならば第一項の減少により全体の分散低減が期待される．
Therefore, under the assumption of 
$\hat{p} \approx p( \tilde{\*f_{\*x}} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{\cF}^* )$
the variance reduction is expected because of the variance reduction in the first term of \eq{eq:decomposed_variance}.

% --- {以降は多分誤り} ---

% 次に第二項をlaw of total varianceにより，
% $\tilde{\cF}^*_S$
% とそれ以外の
% $\tilde{\cF}^*_{-S} = \tilde{\cF}^* \setminus \tilde{\cF}^*_S$
% に分けると
% \begin{align*}
%  &
%  \VV_{\tilde{\cF}^*} 
%  \sbr{
%  a(\tilde{\cF}^*_S)
%  \EE_{\tilde{\*f} \mid \tilde{\cF}^*} \sbr{
%  \xi(\tilde{\*f_{\*x}})
%  }
%  +
%  b(\tilde{\cF}^*_S)
%  } 
%  \\ % ---
%  & =
%  \EE_{\tilde{\cF}^*_S} 
%  \VV_{\tilde{\cF}^*_{-S}} 
%  \sbr{
%  a(\tilde{\cF}^*_S)
%  \EE_{\tilde{\*f} \mid \tilde{\cF}^*} \sbr{
%  \xi(\tilde{\*f_{\*x}})
%  }
%  +
%  b(\tilde{\cF}^*_S)
%  } 
%  \\
%  & \qquad +
%  \VV_{\tilde{\cF}^*_S} 
%  \EE_{\tilde{\cF}^*_{-S}} 
%  \sbr{
%  a(\tilde{\cF}^*_S)
%  \EE_{\tilde{\*f} \mid \tilde{\cF}^*} \sbr{
%  \xi(\tilde{\*f_{\*x}})
%  }
%  +
%  b(\tilde{\cF}^*_S)
%  } 
% \end{align*}
% MAP推定量
% $\theta_{\mr{MAP}}(\tilde{\*f_{\*x}})$
% は
% $\tilde{\cF}^*_{-S}$
% に依存しないため，第一項はMAPの場合$0$になる．
% %
% 一方，
% $\II( \tilde{\*f_{\*x}} \in \cA_O^{\tilde{\cF}^*_S} )$
% は（暗黙のうちに）
% $\tilde{\cF}^*_{-S}$
% にも依存しているため{(これはおかしい気がする)}，第一項は一般に$0$にならない．
% %
% 一方，第二項はMAPの場合は
% \begin{align*}
%  &
%  \VV_{\tilde{\cF}^*_S} 
%  \EE_{\tilde{\cF}^*_{-S}} 
%  \sbr{
%  a(\tilde{\cF}^*_S)
%  \EE_{\tilde{\*f} \mid \tilde{\cF}^*} \sbr{
%  \xi(\tilde{\*f_{\*x}})
%  }
%  +
%  b(\tilde{\cF}^*_S)
%  }  
%  &
%  = 
%  \VV_{\tilde{\cF}^*_S} 
%  \EE_{\tilde{\cF}^*_{-S}} 
%  \sbr{
%  a(\tilde{\cF}^*_S)
%  \EE_{\tilde{\*f} \mid \tilde{\cF}^*} \sbr{
%  \xi(\tilde{\*f_{\*x}})
%  }
%  +
%  b(\tilde{\cF}^*_S)
%  }  
% \end{align*}


% --------------------------------------------------
% \subsection{ベイズ推定の実験的評価}
\subsection{Empirical Verification of MC Estimator of Lower Bound}
\label{app:empirical-study-BayesMAP}

% GPから生成した $d = 1$ の$2$目的最適化を使い，下限の計算精度を検証する．
Using a two objective problem generated by GPs ($d = 1$), we examine the accuracy of the MC estimator compared with the true lower bound. 
%
% 以降，Na{\"i}ve MCを式\eq{eq:LB-MC}をそのまま計算する方法，MC with Bayes MAPをベイズ指定を使う方法とする．
Hereafter, Na{\"i}ve MC indicates the calculation by \eq{eq:LB-MC}, and MC with Bayes MAP indicates the calculation by \eq{eq:LB-MAP}. 
%
% $x \in [0,1]$ に100点の一様グリッドな候補点を用意し，訓練点5点をランダムに選び，その事後分布で下限を計算する．
We calculate the lower bound at $100$ grid points in $x \in [0,1]$ with random $5$ training points.
%
% サンプル数$K = 10^5$のNa{\"i}ve MCを疑似的な正解とみなして，そこからの誤差を評価する．
Regarding the result by Na{\"i}ve MC with $K = 10^5$ samples as a pseudo ground-truth, compared with which we evaluate the estimation error.
%
% MC with Bayes MAPでは近似値 $\hat{p}$ へのバイアスが存在する．
% %
% これは，各 $\cF^*_S$ に対して，対応する $\*f_{\*x}$ は1サンプルしかないことに起因している．
% %
% そのため，それぞれの $\theta_{\mr{MAP}}$ はサンプリング数を増やしても事前分布の影響力が弱まらず，$\hat{p}$ へのバイアスが残る．
% %
% そこで $r$ をサンプル数 $K$ が増えると $r \rightarrow 0$ に減衰するように設定することで，通常のモンテカルロと同様の結果に収束させることができる．
In addition to the fixed $r$ setting, we here examine the setting $r = \sqrt{10/K}$, by which $r$ reduces with $O(1/\sqrt{K})$ (same as the general convergence rate of the MC estimator) and $r = 1$ when $K = 10$ in this setting.
%
% ここでは，$r = \sqrt{K_0/K}$ とする（一般に，モンテカルロ推定量の収束が$O(1/\sqrt{K})$であることからこのようにする）．
%
% $K_0$ はスケーリング係数となるが，今回は $K_0 = 10$ とする．

% GPから生成した $d = 1$ の$2$目的最適化を使い，以下の$3$つの方法の下限の計算精度を検証する：
% - Na{\"i}ve MC: 式\eq{eq:LB-MC}をそのまま計算
% - MC with Bayes MAP ($r = 1$): \eq{eq:LB-MAP}を $r = 1$ で計算
% - MC with Bayes MAP ($r = \sqrt{10/S}$): \eq{eq:LB-MAP}を $r = \sqrt{10/S}$ で計算

%$x \in [0,1]$ に100点の一様グリッドな候補点を用意し，訓練点5点をランダムに選び，その事後分布で下限を計算する．$S = 10^5$ のNa{\"i}ve MCを疑似的な正解とみなして，そこからの誤差を評価したものが

% 図\ref{fig:LB-MSE}に結果を示す．
Figure~\ref{fig:LB-MSE} shows the results by mean squared error (MSE).
%
% MC with Bayes MAPは$r = 1$と$r = \sqrt{10/S}$の場合を両方示している（$K = 10$の場合は二つの結果は一致する）．
MC with Bayes MAP shows $r = 1$ and $r = \sqrt{10/K}$, for which they have the same result when $K = 10$.
%
% サンプル数$K$が少ない場合，Na{\"i}ve MCよりもMC with Bayes MAPの誤差がどちらの$r$でも小さいことがわかる．
When the sample size $K$ is small, MC with Bayes MAP has smaller errors for both the $r$ settings compared with Na{\"i}ve MC.
%
% サンプル数$K$の増加とともいずれの方法も誤差が減少していくが，対数スケールの右図を見ると，MC with Bayes MAP ($r = 1$)が$K = 10^2$あたりから停滞していることがわかる．
With the increase of $K$, all methods decrease MSE, but in the right log scale plot, the decrease of MC with Bayes MAP ($r = 1$) stagnates at around $K = 10^2$--$10^3$. 
%
% 一方で，MC with Bayes MAP ($r = \sqrt{10/K}$)は事前分布の影響が減衰するためMSEが減少を続けている．
On the other hand, MC with Bayes MAP ($r = \sqrt{10/K}$) continues to decrease MSE because it can diminish the effect of the approximation in the prior.
%
% 結果より，$K = 10$などの小サンプル下ではMC with Bayes MAPが有効であることが示唆され，サンプル数を大きな値に設定できる際は$r$の影響を弱めるべきであることがわかる．

% --------------------------------------------------
% Fig: Comparison of Montecarlo MSE
% --------------------------------------------------
\begin{figure}[t]
  \begin{minipage}[b]{0.45\hsize} 
      \centering
      \includegraphics[width=\linewidth]{./figs/MSE.pdf}
      % \subcaption{\scriptsize{過剰な切断}}
      \vspace{-5pt}
  \end{minipage}
  \begin{minipage}[b]{0.45\hsize}
      \centering
      \includegraphics[width=\linewidth]{./figs/MSE-log-ver2.pdf}
      % \subcaption{\scriptsize{\textcolor{red}{混合分布}}}
      \vspace{-5pt}
  \end{minipage}
 \caption{
 % $K = 10^5$のNa{\"i}ve MCを正解とした場合のMSE．
 MSE compared with the pseudo ground truth, created by Na{\"i}ve MC with $K = 10^5$.
 % %
 % 左は元のスケール，右はMSEの$\log_{10}$をとったものである．
 The plot is the original scale, and the right plot is the $\log_{10}$ scale.
 } 
 \label{fig:LB-MSE}
\end{figure}

% \note{ここの実験はNeurIPSの時のままなのでやり直した方が良いと思われる}



% --------------------------------------------------
\section{Parallel Querying}
\label{app:parallel-querying}



We here consider parallel querying in which $Q$ queries should be selected every iteration.
%
Let 
$\cX_q \coloneqq \{\*x^{(1)}, \ldots, \*x^{(q)} \}$
and
$\cH_q = \{ \*f_{\*x^{(1)}}, \ldots, \*f_{\*x^{(q)}} \}$
for $q \leq Q$.
%
Then, 
$\mr{MI}(\cH_Q ; \cF^*)$
can be a selection criterion for determining $Q$ points simultaneously. 
%
However, this leads to $(Q \times d)$-dimensional optimization.
%
Instead, we employ a greedy strategy shown by \citep{Takeno2022-Sequential}, in which the MI approximation can be reduced to a similar computation to the case of single querying.


Assume that we have already select $q < Q$ points $\cX_q$, for which observations are not obtained yet, and consider determining the $(q+1)$-th point $\*x$.
%
In this case, 
$\mr{MI}(\cH_q \cup \*f_{\*x} ; \cF^*)$
should be maximized with respect to the additional $\*x$.
%
We see
\begin{align*}
 \mr{MI}(\cH_q \cup \*f_{\*x} ; \cF^*)
 =
 \mr{MI}(\cH_q ; \cF^*)
 +
 \mr{CMI}(\*f_{\*x} ; \cF^* \mid \cH_q),
\end{align*}
where
$\mr{CMI}(\*f_{\*x} ; \cF^* \mid \cH_q)
=
\EE_{\cH_q}\sbr{ \mr{MI}(\*f_{\*x} ; \cF^* \mid \cH_q) }$
is the MI conditioned on $\cH_q$.
%
Since the first term does not depend on $\*x$, we only need to consider the second term
$\mr{CMI}(\*f_{\*x} ; \cF^* \mid \cH_q)$.


The lower bound of 
$\mr{MI}(\*f_{\*x} ; \cF^* \mid \cH_q)$
is derived in the same way as the lower bound of
$\mr{MI}(\*f_{\*x} ; \cF^*)$, i.e., \eq{eq:VLB-lambda}.
%
The only difference is that the GPs have additional training data consisting of $\cX_q$ and $\cH_q$.
%
Let
$\zeta_{\lambda,q}^{\cF^*_S}(\*x)$
and 
$\eta_{\lambda,q}^{\cF^*_S}(\*x)$
be
$\zeta_{\lambda}^{\cF^*_S}(\*x)$
and 
$\eta_{\lambda}^{\cF^*_S}(\*x)$
in which the GPs with additional $q$ observations are used to calculate $Z_U^{\cF_S^*}(\*x)$ and $Z_O^{\cF_S^*}(\*x)$ as follows:
\begin{align*}
 \zeta_{\lambda,q}^{\cF^*_S}(\*x)
 & = \frac{ \lambda }{ Z_U^{\cF^*_S}(\*x \mid \cH_q) } 
 + \frac{ 1 - \lambda }{ Z_O^{\cF^*_S}(\*x \mid \cH_q) },
 \\
 \eta_{\lambda,q}^{\cF^*_S}(\*x)
 &= \frac{ \lambda }{ Z_U^{\cF^*_S}(\*x \mid \cH_q) },
\end{align*}
where
$Z_U^{\cF^*_S}(\*x \mid \cH_q) \coloneqq p(\*f_{\*x} \in \cA_U^{\cF^*_S} \mid \cH_q)$
and
$Z_O^{\cF^*_S}(\*x \mid \cH_q) \coloneqq p(\*f_{\*x} \in \cA_O^{\cF^*_S} \mid \cH_q)$.
%
%
% Let 
% $\wh{L}(\*x, \lambda \mid \cH_q)$
% be the MC approximation of the lower bound of 
% $\mr{MI}(\*f_{\*x} ; \cF^* \mid \cH_q)$,
%
% Therefore, 
Then, we can write
\begin{align}
 &
 \EE_{\cH_q}\sbr{ \mr{MI}(\*f_{\*x} ; \cF^* \mid \cH_q) }
 \notag \\
 &
 \geq 
 \EE_{\cH_q}
 \EE_{\cF^*, \*f_{\*x} \mid \cH_q} 
 \biggl[
 \log
 \bigl\{
 \zeta_{\lambda,q}^{\cF^*_S}(\*x)
 \II( \*f_{\*x} \in \cA_O^{\cF^*_S} ) 
 \notag \\
 & \qquad \qquad \qquad
 + \eta_{\lambda,q}^{\cF^*_S}(\*x)
 \II( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} )
 \bigr\}
 \biggr]
 \notag \\ % --
 & = \EE_{\cF^*, \*f_{\*x}, \cH_q} 
 \biggl[
 \log
 \bigl\{
 \zeta_{\lambda,q}^{\cF^*_S}(\*x)
 \II( \*f_{\*x} \in \cA_O^{\cF^*_S} ) 
 \notag \\
 & \qquad \qquad \qquad
 + \eta_{\lambda,q}^{\cF^*_S}(\*x)
 \II( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} )
 \bigr\}
 \biggr] 
 \label{eq:qVLB}
\end{align}
% where 
% $\zeta_{\lambda,q}^{\cF^*_S}(\*x)$
% and 
% $\eta_{\lambda,q}^{\cF^*_S}(\*x)$
% are 
% $\zeta_{\lambda}^{\cF^*_S}(\*x)$
% and 
% $\eta_{\lambda}^{\cF^*_S}(\*x)$
% in which the GPs with additional $q$ observations are used to calculate $Z_U^{\cF_S^*}(\*x)$ and $Z_O^{\cF_S^*}(\*x)$.
%
Since the expectation 
$\EE_{\cH_q} \EE_{\cF^*, \*f_{\*x} \mid \cH_q}$
% in \eq{eq:qVLB} 
can be seen as the joint expectation
$\EE_{\cF^*, \*f_{\*x}, \cH_q}$,
the MC approximation can be performed by using samples from the joint distribution of $\cF^*, \*f_{\*x}$ and $\cH_q$.
%
Let $F_q$ be a set of samples
$(\tilde{\cF}^*_S, \tilde{\*f}_{\*x}, \tilde{\cH}_q)$
from the joint distribution.
%
Then, the MC approximation of the lower bound \eq{eq:qVLB} is
\begin{align*}
 & \frac{1}{K}
 \sum_{(\tilde{\cF}^*_S, \tilde{\*f}_{\*x}, \tilde{\cH}_q) \in F_q}
 \log
 \bigl\{
 \zeta_{\lambda,q}^{\tilde{\cF}^*_S}(\*x)
 \II( \tilde{\*f}_{\*x} \in \cA_O^{\tilde{\cF}^*_S} ) 
 \\
 & \qquad \qquad \qquad
 + \eta_{\lambda,q}^{\tilde{\cF}^*_S}(\*x)
 \II( \tilde{\*f_{\*x}} \in \cA_{U \setminus O}^{\tilde{\cF}^*_S} ) 
 \bigr\}
\end{align*}
The sampling of $F_q$ can be performed by almost the same procedure as the single querying.
%
First, we generate the ``entire function $\tilde{\*f}$'' by using RFM.
%
$\tilde{\cF}^*_S$ is obtained by applying NSGA-II to $\tilde{\*f}$.
%
$\tilde{\*f}_{\*x}$ and $\tilde{\cH}_q$ can be immediately obtained from RFM.
%
Note that even when we perform the next $(q + 2)$-th point selection, we can reuse $\tilde{\cF}^*_S$ and $\tilde{\*f}$, from which $\tilde{\cH}_{q+1}$ can also be immediately obtained.

The MAP-based approximation can also be applied to the parallel setting. 
%
The lower bound \eq{eq:qVLB} can be re-written as
\begin{align*}
 &
 \EE_{\cF^*, \cH_q} 
 \EE_{ \*f_{\*x} \mid \cF^*, \cH_q} 
 \biggl[
 \II( \*f_{\*x} \in \cA_O^{\cF^*_S} ) 
 \log
 \zeta_{\lambda,q}^{\cF^*_S}(\*x) 
 \notag \\
 & \qquad \qquad \qquad
 + 
 \II( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} )
 \log \eta_{\lambda,q}^{\cF^*_S}(\*x)
 \biggr]
 \\
 &
 = \EE_{\cF^*, \cH_q} 
 \biggl[
 p( \*f_{\*x} \in \cA_O^{\cF^*_S} \mid \cF^*, \cH_q) 
 \log
 \zeta_{\lambda,q}^{\cF^*_S}(\*x)
 \notag \\
 & \qquad \qquad \qquad
 + 
 p( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} \mid \cF^*, \cH_q)
 \log
 \eta_{\lambda,q}^{\cF^*_S}(\*x)
 \bigr\}
 \biggr].
 % \label{eq:qVLB}
\end{align*}
%
The prior approximation for 
$p( \*f_{\*x} \in \cA_O^{\cF^*_S} \mid \cF^*, \cH_q)$
becomes
$p( \*f_{\*x} \in \cA_O^{\cF^*_S} \mid \cF^*, \cH_q) \approx Z_O^{\cF^*_S}(\*x \mid \cH_q) / Z_U^{\cF^*_S}(\*x \mid \cH_q)$.
%
Then, $\theta_{\rm MAP}$ can be obtained by the same procedure shown in Section~\ref{ssec:computations}. 
%
As a result, we have an approximation of the lower bound \eq{eq:qVLB} 
\begin{align*}
 & \frac{1}{K}
 \sum_{(\tilde{\cF}^*_S, \tilde{\*f}_{\*x}, \tilde{\cH}_q) \in F_q}
 \theta_{\rm MAP}
 \log
 \zeta_{\lambda,q}^{\tilde{\cF}^*_S}(\*x)
 \\
 & \qquad \qquad \qquad
 + (1 - \theta_{\rm MAP})
 \log 
 \eta_{\lambda,q}^{\tilde{\cF}^*_S}(\*x).
\end{align*}

Figure~\ref{fig:results-parallel} shows the empirical evaluation for which the setting is same as in Section~\ref{ssec:GPDerivedArtificialFunctions}. 
%
Here, we set $Q = 2$ and $3$, and we used the $(d, L) = (3,3)$ GP derived functions. 
%
For comparison, ParEGO, EHVI, MOBO-RS and JES were used.
%
ParEGO and EHVI consider the expected improvement when $Q$ points are simultaneously selected, which is a well known general strategy \citep{Shahriari2016-Taking}.
%
Unlike the single querying, the expectation is approximated by the MC estimation for which the number of samples was $100$ and $10$ for ParEGO and EHVI, respectively.
%
For MOBO-RS, $Q$ points are selected by repeating Thompson sampling with different sample paths $Q$ times \citep{Kandasamy2018-Parallelised}, in which the weights in the Tchebycheff (also known as Chebyshev) scalarization were also re-sampled.
%
JES approximates the simultaneous information gain by $Q$ points as indicated by \citep{Tu2022-joint}.
%
From the results, we can see that the proposed method shows sufficiently high performance in the parallel querying.


% --------------------------------------------------
% Fig: Results on Parallel
% --------------------------------------------------
\begin{figure}
 \centering
 \subfigure[$Q = 2$]{
 \ig{.22}{./figs/Ext-Parallel/Q2/RHV_input_dim_3output_dim_3_length_scale_0.1.pdf}}
 \subfigure[$Q = 3$]{
 \ig{.22}{./figs/Ext-Parallel/Q3/RHV_input_dim_3output_dim_3_length_scale_0.1.pdf}}
 \caption{
 Results on parallel querying.
 }
 \label{fig:results-parallel}
\end{figure}


% --------------------------------------------------
\section{Decoupled Setting}
\label{app:decoupled-setting}

For the decoupled setting, MI and its lower bound are 
{\small
\begin{align*}
 &\mr{MI}(f^l_{\*x} ; \cF^*) \\
 &=
 \EE_{\cF^*, f^l_{\*x}}\sbr{
 \log \frac{q(f^l_{\*x} \mid \cF^{*})}{p(f^l_{\*x})} 
 }
 + D_{\mr{KL}}\rbr{ 
 p(f^l_{\*x} \mid \cF^*) \parallel q(f^l_{\*x} \mid \cF^*) 
 }
 \\
 &\geq
 \EE_{\cF^*, f^l_{\*x}}\sbr{
 \log \frac{q(f^l_{\*x} \mid \cF^{*})}{p(f^l_{\*x})} 
 } \eqqcolon L_{\rm Dec}(\*x, l, \lambda).
\end{align*}}%
%
We define 
$q(f^l_{\*x} \mid \cF^{*})$ 
as the marginal distribution of 
$q_\lambda(\*f_{\*x} \mid \cF^{*})$:
\begin{align}
 & q(f^l_{\*x} \mid \cF^{*})
 \notag \\ % --
 & =
 \int 
 q_\lambda(\*f_{\*x} \mid \cF^{*})
 \mr{d}\*f^{-l}_{\*x}
 \notag \\ % --
 & =
 \int 
 \lambda q_U(\*f_{\*x} \mid \cF^*_S) + (1 - \lambda) q_O(\*f_{\*x} \mid \cF^*_S) 
 \mr{d}\*f^{-l}_{\*x}
 \notag \\ % --
 & =
 \int 
 p(\*f_{\*x})
 \zeta_\lambda^{\cF^*_S}(\*x)
 \II( \*f_{\*x} \in \cA_O^{\cF^*_S} ) \mr{d}\*f^{-l}_{\*x} 
 \notag \\
 & \qquad \qquad
 + 
 \int 
 p(\*f_{\*x})
 \eta_\lambda^{\cF^*_S}(\*x)
 \II( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} )
 \mr{d}\*f^{-l}_{\*x}
 \notag \\ % --
 & =
 p(f^l_{\*x}) 
 \bigl\{
 \zeta_\lambda^{\cF^*_S}(\*x)
 \int 
 p(\*f^{-l}_{\*x} \mid f^l_{\*x})
 \II( \*f_{\*x} \in \cA_O^{\cF^*_S} ) \mr{d}\*f^{-l}_{\*x} 
 \notag \\
 & \qquad \qquad  
 + 
 \eta_\lambda^{\cF^*_S}(\*x)
 \int 
 p(\*f^{-l}_{\*x} \mid f^l_{\*x})
 \II( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} )
 \mr{d}\*f^{-l}_{\*x}
 \bigr\}
 \notag \\ % --
 & =
 p(f^l_{\*x}) 
 \bigl\{
 \zeta_\lambda^{\cF^*_S}(\*x) % f^l_{\*x}の確率的揺らぎは関係ないはず
 p(\*f_{\*x} \in \cA_O^{\cF^*_S} \mid f^l_{\*x})
 % \int 
 % p(\*f^{-l}_{\*x})
 % \II( \*f_{\*x} \in \cA_O^{\cF^*_S} ) \mr{d}\*f^{-l}_{\*x} 
 \notag \\
 & \qquad \qquad \qquad
 + 
 % p(f^l_{\*x}) 
 \eta_\lambda^{\cF^*_S}(\*x)
 p( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} \mid f^l_{\*x})
 % \int 
 % p(\*f^{-l}_{\*x})
 % \II( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} )
 % \mr{d}\*f^{-l}_{\*x}
 \bigr\},
 \label{eq:decoupled-vd}
\end{align}
where $\*f_{\*x}^{-l}$ is the $(L-1)$-dimensional subvector of $\*f_{\*x}$ in which $f^l_{\*x}$ is removed.
%
Then, the lower bound and its MC approximation is obtained as
\begin{align*}
 & L_{\rm Dec}(\*x, l, \lambda) 
 \\
 & = 
 \EE_{\cF^*, f^l_{\*x}} \biggl[
 \log 
 \bigl\{
 \zeta_\lambda^{\cF^*_S}(\*x)
 p(\*f_{\*x} \in \cA_O^{\cF^*_S} \mid f^l_{\*x})
 \\
 & \qquad \qquad \qquad
 +
 \eta_\lambda^{\cF^*_S}(\*x)
 p( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} \mid f^l_{\*x})
 \bigr\}
 \biggr]
 \\ % ---
 & \approx
 \frac{1}{K} \sum_{(\tilde{\cF}^*_S, \tilde{\*f}) \in F}
 \log 
 \bigl\{
 \zeta_\lambda^{\tilde{\cF}^*_S}(\*x)
 p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{f}^l_{\*x})
 \\
 & \qquad \qquad \qquad
 +
 \eta_\lambda^{\tilde{\cF}^*_S}(\*x)
 p( \*f_{\*x} \in \cA_{U \setminus O}^{\tilde{\cF}^*_S} \mid \tilde{f}^l_{\*x})
 \bigr\}.
\end{align*}
%
% $\bar{f}^l \coloneqq \max \{ f^l \mid \*f \in \cF_S^* \}$
% \begin{align*} % 間違い
%  \EE_{\cF^*, f^l_{\*x}}\sbr{
%  \log \left(
%  \zeta_\lambda^{\cF^*_S}(\*x)
%  p(\*f_{\*x} \in \cA_O^{\cF^*_S} \mid f^l_{\*x})
%  \right) 
%  \II(f^l_{\*x} \leq \bar{f}^l)
%  +
%  \log \left(
%  \eta_\lambda^{\cF^*_S}(\*x)
%  p( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} \mid f^l_{\*x})
%  \right)
%  } 
% \end{align*}
%
The probabilities 
$p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{f}^l_{\*x})$
and
$p( \*f_{\*x} \in \cA_{U \setminus O}^{\tilde{\cF}^*_S} \mid \tilde{f}^l_{\*x})$
can be analytically calculated. 
%
Let
$\cC_i = (\ell_i^1, u_i^1] \times (\ell_i^2, u_i^2] \times \cdots \times (\ell_i^L, u_i^L]$
be the cell partitions of the over-truncated region $\cA_O^{\cF_S^*}$. 
%
% Further, suppose that
% $f_1^l < f_2^l < \cdots < f^l_{S_l}$ for $S_l \leq S$
% be a sequence ascendingly sorted by the $l$-th dimension of all 
% $\*f_{\*x} \in \cF^*_S$ 
% (duplicated values are eliminated), where 
% $S = |\cF^*_S|$. 
%
% For all cells $\cC_1, \ldots, \cC_C$, % $c \in [C]$
% we assume that there exists
% $s \in \{ 0, \ldots, S_l \}$
% such that
% $\ell^l_c= f^l_s$ 
% and
% $u^l_c = f^l_{s+1}$ 
% % $(\ell^l_c, u^l_c] = (f^l_s, f^l_{s+1}]$ 
% (This assumption is only for notational brevity. It is always easy to create cells satisfying this condition).
% %
% $\cI(l,s) = \{ c \mid (\ell^l_c, u^l_c] = (f^l_s, f^l_{s+1}] \}$
% The set of indices of $\cC_c$ having the interval $(f^l_s, f^l_{s+1}]$ is denoted as
% $\cI(l,s) = \{ c \mid \ell^l_c= f^l_s, u^l_c = f^l_{s+1} \}$. 
%
Then, from the independence of $\*f_{\*x}$, we see
\begin{align}
 & p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{f}^l_{\*x})
 \notag \\ % --
 & = \int 
 p(\*f^{-l}_{\*x})
 \II( \*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} ) \mr{d}\*f^{-l}_{\*x}  
 \notag \\ % --
 & =
 \sum_{c = 1}^C
 \II(f_{\*x}^l \in (\ell^l_c, u^l_c])
 \int_{\cC_c^{-l}}
 p(\*f^{-l}_{\*x})
 \mr{d}\*f^{-l}_{\*x}  
 \notag \\ % --
 & =
 \sum_{c = 1}^C
 \II(f_{\*x}^l \in (\ell^l_c, u^l_c])
 \prod_{l^\prime \neq l} 
 \rbr{ 
 \Phi(\bar{\alpha}_{c,l^\prime}) - \Phi(\underline{\alpha}_{c,l^\prime}) 
 }
 \notag \\ % --
 & =
 \sum_{c = 1}^C
 \II(f_{\*x}^l \in (\ell^l_c, u^l_c])
 \prod_{l^\prime \neq l} Z_{cl^\prime}, 
 \label{eq:prob-A_O-given-f_l}
\end{align}
% \begin{align} % 上と同じ趣旨の数式．上の方が簡潔．
%  & p(\*f_{\*x} \in \cA_O^{\cF^*_S} \mid f^l_{\*x})
%  \notag \\
%  & = \int 
%  p(\*f^{-l}_{\*x})
%  \II( \*f_{\*x} \in \cA_O^{\cF^*_S} ) \mr{d}\*f^{-l}_{\*x}  
%  \notag \\
%  & =
%  % \sum_{c^\prime \in \cI(l,s^l_{f^l_{\*x}})}
%  \sum_{c \in \cI(l,s^l(f^l_{\*x}))}
%  \int_{\cC_c^{-l}}
%  p(\*f^{-l}_{\*x})
%  \mr{d}\*f^{-l}_{\*x}  
%  \notag \\
%  & =
%  \sum_{c \in \cI(l,s^l(f^l_{\*x}))}
%  \prod_{l^\prime \neq l} 
%  \rbr{ 
%  \Phi(\bar{\alpha}_{c,l^\prime}) - \Phi(\underline{\alpha}_{c,l^\prime}) 
%  },
%  \notag \\
%  & =
%  \sum_{c \in \cI(l,s^l(f^l_{\*x}))}
%  \prod_{l^\prime \neq l} Z_{cl^\prime}
%  \label{eq:prob-A_O-given-f_l}
% \end{align}
where 
$Z_{cl^\prime} = \Phi(\bar{\alpha}_{c,l^\prime}) - \Phi(\underline{\alpha}_{c,l^\prime})$ 
and
$\cC_c^{-l}$ is the $(L-1)$-dimensional hyper-rectangle created by removing the $l$-th dimension of $\cC_c$.
% ,
% and
% $s^l(f) \in [S_l]$
% is the index such that 
% $f \in (f^l_s, f^l_{s+1}]$.
%
For 
$p( \*f_{\*x} \in \cA_{U \setminus O}^{\tilde{\cF}^*_S} \mid \tilde{f}^l_{\*x})$,
we use the following relation: 
\begin{align*}
 & p( \*f_{\*x} \in \cA_{U \setminus O}^{\tilde{\cF}^*_S} \mid \tilde{f}^l_{\*x})
 \\
 &= 
 1 - p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{f}^l_{\*x})
 - p(\*f_{\*x} \notin \cA_U^{\tilde{\cF}^*_S} \mid \tilde{f}^l_{\*x}).
\end{align*}
Since 
$\*f_{\*x} \notin \cA_U^{\tilde{\cF}^*_S}$ in the last term
can be written as ``dominated region'', shown in the end of Appendix~\ref{app:CalcZ}.
%
We can calculate 
$p(\*f_{\*x} \notin \cA_U^{\tilde{\cF}^*_S} \mid \tilde{f}^l_{\*x})$
by the same dominated region decomposition as \eq{eq:prob-A_O-given-f_l}.


% \begin{align*}
%  & L_{\rm Dec}(\*x, l, \lambda) 
%  \\
%  & = 
%  \EE_{\cF^*, f^l_{\*x}} \biggl[
%  \log 
%  \bigl\{
%  \II(f^l_{\*x} \leq \max \{ f^l_{\*x} \mid \*f_{\*x} \in \cF^* \})
%  \zeta_\lambda^{\cF^*_S}(\*x)
%  p(\*f_{\*x} \in \cA_O^{\cF^*_S} \mid f^l_{\*x})
%  \\
%  & \qquad \qquad \qquad
%  +
%  \eta_\lambda^{\cF^*_S}(\*x)
%  p( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} \mid f^l_{\*x})
%  \bigr\}
%  \biggr]
%  \\ % --
%  & = 
%  \EE_{\cF^*, f^l_{\*x}} \biggl[
%  \II(f^l_{\*x} \leq \max \{ f^l_{\*x} \mid \*f_{\*x} \in \cF^* \})
%  \log  
%  \bigl\{
%  \zeta_\lambda^{\cF^*_S}(\*x)
%  p(\*f_{\*x} \in \cA_O^{\cF^*_S} \mid f^l_{\*x})
%  \\
%  & \qquad \qquad 
%  +
%  \eta_\lambda^{\cF^*_S}(\*x)
%  p( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} \mid f^l_{\*x})
%  \bigr\}
%  \\
%  & \qquad \qquad 
%  + 
%  \II(f^l_{\*x} > \max \{ f^l_{\*x} \mid \*f_{\*x} \in \cF^* \})
%  \log  
%  \eta_\lambda^{\cF^*_S}(\*x)
%  p( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} \mid f^l_{\*x})
%  \biggr]
% \end{align*}

% --------------------------------------------------
% Fig: Results on Decoupled
% --------------------------------------------------
\begin{figure*}
 \centering
 \subfigure[$\ell_{\rm RBL} = 0.05$]{
 % \ig{.25}{./figs/Ext-Decoupled/maxIRHV_input_dim_3output_dim_3_length_scale_0.05.pdf}}
%  \ig{.25}{./figs/Ext-Decoupled/RHV_input_dim_3output_dim_3_length_scale_0.05.pdf}}
 \ig{.25}{./figs/Decoupled/Dec_RHV_input_dim_3output_dim_3_length_scale_0.05.pdf}}
 \subfigure[$\ell_{\rm RBL} = 0.1$]{
 % \ig{.25}{./figs/Ext-Decoupled/maxIRHV_input_dim_3output_dim_3_length_scale_0.1.pdf}}
%  \ig{.25}{./figs/Ext-Decoupled/RHV_input_dim_3output_dim_3_length_scale_0.1.pdf}}
 \ig{.25}{./figs/Decoupled/Dec_RHV_input_dim_3output_dim_3_length_scale_0.1.pdf}}
 \subfigure[$\ell_{\rm RBL} = 0.25$]{
 % \ig{.25}{./figs/Ext-Decoupled/maxIRHV_input_dim_3output_dim_3_length_scale_0.25.pdf}}
%  \ig{.25}{./figs/Ext-Decoupled/RHV_input_dim_3output_dim_3_length_scale_0.25.pdf}}
\ig{.25}{./figs/Decoupled/Dec_RHV_input_dim_3output_dim_3_length_scale_0.25.pdf}}
 \caption{
 Results on decoupled setting.
 }
 \label{fig:results-decoupled}
\end{figure*}

% \red{Figure~\ref{fig:results-decoupled}の実験に関して，KG手法がBOTorchを用いたものであることを述べる．（Appendixで述べるのかあるいは本文で言及するのか要検討）}

Figure~\ref{fig:results-decoupled} shows the empirical evaluation for which the setting is same as in Section~\ref{ssec:GPDerivedArtificialFunctions}. 
%
Here, we used the $(d, L) = (3, 3)$ GP derived functions for three length scales. 
%
As a baseline, the hypervolume-based KG is used.
%
Since KG is defined as the hyper-volume defined by the `one-step ahead' posterior mean, it is easy to extend to the decoupled setting as shown by \citep{daulton23-hypervolume}.
%
% \remove{To simplify the implementation, we evaluate the posterior mean hyper-volume after adding sampled $\tilde{f}^{l}(\*x)$ into the GPs only by using the pre-defined grid points in $\cX$ (uniformly taken $5$ points in each dimension is used).}
% \red{
We used BoTorch's qHypervolumeKnowledgeGradient implementation for the HVKG baseline, which is based on the `one shot' optimization of KG in the decoupled setting. Due to the long computational time, we set the number of Pareto-optimal points in the one-step ahead posterior mean as 10 in HVKG.
%
For fair comparison, our proposed method also set the size of the Pareto-optimal points in the sampled function (i.e., the NSGA-II population size) as 10.
%
The number of samples (so called fantasy points) in HVKG is also set as 10. 
%
% \remove{Although there is an implementation difference (our proposed method is GPy-based while HVKG uses BoTorch), the results show that our method achieves sufficient performance compared to this existing package.}%
%
For the final evaluation of the performance, since the decoupled setting observes only one objective function $f^l(\*x_t)$ in each iteration, the hyper-volume consisting of observed points is difficult to define.
%
Instead, we employ an approach similar to so-called inference regret.
%
At each iteration $t$, we apply NSGA-II to the posterior mean $\*\mu(\*x)$, and obtain a set of the Pareto-optimal points $\cX^*$ for $\*\mu(\*x)$.
%
We evaluate the hyper-volume defined by the ground-truth objective function values on $\cX^*$, and the plots are the maximum values of the volumes identified until each iteration.
%
From results, we see that the decoupled extension of PFEV has reasonable performance (Note that we only have about $1/3$ observations compared with the same number of iterations of the coupled setting because only one of the objective functions is observed).
%
Due to the package differences (PFEV is based on GPy, while HVKG is BoTorch), this comparison is not a completely fair comparison. 
%
However, it demonstrates that the proposed method can achieve comparable or superior performance to a standard package. 
%
A more fair and thorough comparison is our future work.




% --------------------------------------------------
\section{Joint Entropy Extension}
\label{app:JES}

Let
$\cX^* = \{ \*x \mid \*f_{\*x} \in \cF^* \}$.
% and $\cH = \{ (\*x, \*f_{\*x}) \}_{\*x \in \cX^*}$.
%
The lower bound is
\begin{align*}
 % & \mr{MI}(\*f_{\*x} ; \cF^*, \cX^* ) 
 % \\ % --
 % & 
 % \geq 
 % \EE_{\cF^*, \cX^*, \*f_{\*x}}\sbr{
 % \log \frac{q(\*f_{\*x} \mid \cF^{*}, \cX^*)}{p(\*f_{\*x})} 
 % }
 % \\ % --
 % &=
 % \EE_{\cF^*, \cX^*, \*f_{\*x}}\sbr{
 % \log
 % \left\{
 % \zeta_{\lambda}^{\cF^*_S}(\*x)
 % \II( \*f_{\*x} \in \cA_O^{\cF^*_S} ) 
 % + \eta_{\lambda,}^{\cF^*_S}(\*x)
 % \II( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} )
 % \right\}
 % }. 
 \mr{MI}(\*f_{\*x} ; \cX^*, \cF^* ) 
 & 
 \geq 
 \EE_{\cX^*, \cF^*, \*f_{\*x}}\sbr{
 \log \frac{q(\*f_{\*x} \mid \cX^*, \cF^*)}{p(\*f_{\*x})} 
 }.
\end{align*}
%
In practice, we only obtain a subset $\cX_S^* \subseteq \cX^*$, by which 
$\cF_S^* = \{ \*f_{\*x} \}_{\*x \in \cX_S^*}$
and
$\cH_S = \{ (\*x, \*f_{\*x}) \}_{\*x \in \cX_S^*}$
are defined.
%
In the variational distribution 
$q(\*f_{\*x} \mid \cX^*, \cF^*)$,
$\cH_S$ can be seen as an additional training data of the GPs $\*f_{\*x}$.
%
Then, a natural extension of the variational distribution \eq{eq:q} is 
{\small
\begin{align*}
& q_{\lambda}(\*f_{\*x} \mid \cX^*_S, \cF^*_S) 
% = \lambda q_U(\*f_{\*x} \mid \cF^*_S) + (1 - \lambda) q_O(\*f_{\*x} \mid \cF^*_S), 
\notag \\ 
& =
\begin{cases}
\rbr{ 
\frac{ \lambda }{ Z_U^{\cF^*_S}(\*x \mid \cH_S) } + 
\frac{ 1 - \lambda }{ Z_O^{\cF^*_S}(\*x \mid \cH_S) } } 
p(\*f_{\*x} \mid \cH_S)
& 
\text{ if } \*f_{\*x} \in \cA_O^{\cF^*_S}, 
\\
\frac{\lambda}{ Z_U^{\cF^*_S}(\*x \mid \cH_S)  }
p(\*f_{\*x} \mid \cH_S)  
& \text{ if } \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S}, 
\\
0 & \text{ otherwise, }
\end{cases}
\end{align*}}%
where
$Z_U^{\cF^*_S}(\*x \mid \cH_S) \coloneqq p(\*f_{\*x} \in \cA_U^{\cF^*_S} \mid \cH_S)$
and
$Z_O^{\cF^*_S}(\*x \mid \cH_S) \coloneqq p(\*f_{\*x} \in \cA_O^{\cF^*_S} \mid \cH_S)$.
%
Note that here the conditioning on $\cH_S$ is interpreted as a simple addition of the training data, and does not impose the conditions that ``$\cH_S$ is the optimal solutions'', which is represented by the truncation (Because of this reason, we do not give `$*$' to $\cH_S$).
%
The resulting lower bound is 
\begin{align}
 & 
 \EE_{\cX^*, \cF^*, \*f_{\*x}}\biggl[
 \log
 \bigl\{
 \zeta_{\lambda}^{\cF^*_S}(\*x \mid \cH_S)
 \II( \*f_{\*x} \in \cA_O^{\cF^*_S} ) 
 \notag \\
 & \qquad \qquad \qquad
 + \eta_{\lambda}^{\cF^*_S}(\*x \mid \cH_S)
 \II( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} )
 \bigr\}
 \biggr],
 \label{eq:VLB-JES}
\end{align}
where
$\zeta_\lambda^{\cF^*_S}(\*x \mid \cH_S) = \frac{ \lambda }{ Z_U^{\cF^*_S}(\*x \mid \cH_S) } + \frac{ 1 - \lambda }{ Z_O^{\cF^*_S}(\*x \mid \cH_S) }$
and
$\eta_\lambda^{\cF^*_S}(\*x \mid \cH_S) = \frac{ \lambda }{ Z_U^{\cF^*_S}(\*x \mid \cH_S) }$.
%
The same MC approximation as \eq{eq:LB-MC} can be used to evaluate \eq{eq:VLB-JES}.

The MAP-based approximation is also possible based on transformation of \eq{eq:VLB-JES}: 
\begin{align*}
 & 
 \EE_{\cX^*, \cF^*}\biggl[
 p( \*f_{\*x} \in \cA_O^{\cF^*_S} \mid \cX^*, \cF^*) 
 \log
 % \bigl\{
 \zeta_{\lambda}^{\cF^*_S}(\*x \mid \cH_S)
 % \II( \*f_{\*x} \in \cA_O^{\cF^*_S} ) 
 \notag \\
 & \qquad \qquad \qquad
 + 
 p(\*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} \mid \cX^*, \cF^*)
 \log
 \eta_{\lambda}^{\cF^*_S}(\*x \mid \cH_S)
 % \II( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} )
 % \bigr\}
 \biggr]. 
\end{align*}
%
Based on the same idea shown in Section~\ref{ssec:computations}, we approximate
$p( \*f_{\*x} \in \cA_O^{\cF^*_S} \mid \cX^*, \cF^*) \approx Z_O^{\cF^*_S}(\*x \mid \cH_S) / Z_U^{\cF^*_S}(\*x \mid \cH_S)$, 
from which the MAP estimator can be defined.



Figure~\ref{fig:results-proposed-JES} shows the empirical evaluation for which the setting is same as in Section~\ref{ssec:GPDerivedArtificialFunctions}. 
%
Here, we used the $(d, L) = (3, 4)$ GP derived functions for three length scales. 
%
We see that the original proposed method shows slightly better performance than the JES extension, though their behaviors are similar.
%
% Since the JES extension builds the GPs with additional training data $\cH_S$ for each sample, additional computations are required.


% --------------------------------------------------
% Fig: Results on JES 
% --------------------------------------------------
\begin{figure*}
 \centering
 \subfigure[$\ell_{\rm RBL} = 0.05$]{
 \ig{.25}{./figs/Ext-JES/RHV_input_dim_3output_dim_4_length_scale_0.05.pdf}}
 \subfigure[$\ell_{\rm RBL} = 0.1$]{
 \ig{.25}{./figs/Ext-JES/RHV_input_dim_3output_dim_4_length_scale_0.1.pdf}}
 \subfigure[$\ell_{\rm RBL} = 0.25$]{
 \ig{.25}{./figs/Ext-JES/RHV_input_dim_3output_dim_4_length_scale_0.25.pdf}}
 \caption{
 Comparison with JES extension of proposed method.
 }
 \label{fig:results-proposed-JES}
\end{figure*}


% \begingroup
% \color{blue}

% --------------------------------------------------
\section{Noisy Observation}
\label{app:noisy-obs}

% --------------------------------------------------
% \subsection{PFEV with Noisy Observation}

Let 
$y^l_{\*x} = f^l_{\*x} + \veps$ 
and 
$\*y_{\*x} = (y^1_{\*x}, \ldots, y^L_{\*x})^\top$, 
where 
$\veps \sim \cN(0, \sigma_{\rm noise}^2)$. 
%
The mutual information for noisy observation is 
$\mr{MI}(\*y_{\*x} ; \cF^*)$,
for which the lower bound can be derived as
\begin{align*}
 &\mr{MI}(\*y_{\*x} ; \cF^*) \\
 &=
 \EE_{\cF^*, \*y_{\*x}}\sbr{
 \log \frac{q(\*y_{\*x} \mid \cF^{*})}{p(\*y_{\*x})} 
 }
 \\
 & \qquad + D_{\mr{KL}}\rbr{ 
 p(\*y_{\*x} \mid \cF^*) \parallel q(\*y_{\*x} \mid \cF^*) 
 }
 \\
 &\geq
 \EE_{\cF^*, \*y_{\*x}}\sbr{
 \log \frac{q(\*y_{\*x} \mid \cF^{*})}{p(\*y_{\*x})} 
 }.
\end{align*}
%
Since $\cF^*$ and $\*y_{\*x}$ are independent if $\*f_{\*x}$ is given, we define
$q(\*y_{\*x} \mid \cF^{*})$
by using 
$q_\lambda(\*f_{\*x} \mid \cF^{*})$
as follows.
\begin{align*}
 & q(\*y_{\*x} \mid \cF^{*})
 \\ % --
 & =
 \int 
 p(\*y_{\*x} \mid \*f_{\*x})
 q_\lambda(\*f_{\*x} \mid \cF^{*})
 \mr{d}\*f_{\*x}
 \\ % --
 & =
 \int 
 p(\*y_{\*x} \mid \*f_{\*x})
 (
 \lambda q_U(\*f_{\*x} \mid \cF^*_S) 
 \\
 & \qquad \qquad 
 + (1 - \lambda) q_O(\*f_{\*x} \mid \cF^*_S) )
 \mr{d}\*f_{\*x}
 \\ % --
 & =
 \int 
 p(\*y_{\*x} \mid \*f_{\*x})
 p(\*f_{\*x})
 \bigl\{
 \zeta_\lambda^{\cF^*_S}(\*x)
 \II( \*f_{\*x} \in \cA_O^{\cF^*_S} ) \\
 & \qquad \qquad
 + \eta_\lambda^{\cF^*_S}(\*x)
 \II( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} )
 \bigr\}
 \mr{d}\*f_{\*x}
 \\
 % --
 & =
 \int_{\*f_{\*x} \in \cA_O^{\cF^*_S} }
 p(\*y_{\*x}, \*f_{\*x})
 \zeta_\lambda^{\cF^*_S}(\*x)
 \mr{d}\*f_{\*x}
 \\
 & \qquad \qquad
 + \int_{\*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} }
 p(\*y_{\*x}, \*f_{\*x})
 \eta_\lambda^{\cF^*_S}(\*x) 
 \mr{d}\*f_{\*x}
 \\
 % --
 & =
 p(\*y_{\*x}) \biggl\{ 
 \zeta_\lambda^{\cF^*_S}(\*x)
 \int_{\*f_{\*x} \in \cA_O^{\cF^*_S} }
 p(\*f_{\*x} \mid \*y_{\*x}) 
 \mr{d}\*f_{\*x}
 \\
 & \qquad \qquad
 + 
 \eta_\lambda^{\cF^*_S}(\*x) 
 \int_{\*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} }
 p(\*f_{\*x} \mid \*y_{\*x}) 
 \mr{d}\*f_{\*x}
 \biggr\}
 \\
 % --
 & =
 p(\*y_{\*x}) \left\{
 \zeta_\lambda^{\cF^*_S}(\*x)
 p(\*f_{\*x} \in \cA_O^{\cF^*_S} \mid \*y_{\*x})
 \right.
 \\
 & \qquad \qquad \left. + 
 \eta_\lambda^{\cF^*_S}(\*x)  
 p(\*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} \mid \*y_{\*x})
 \right\}.
\end{align*}
Then, the MC approximation becomes
\begin{align*}
 & \EE_{\cF^*, \*y_{\*x}} \left[
 \log
 \left\{
 \zeta_\lambda^{\cF^*_S}(\*x)
 p(\*f_{\*x} \in \cA_O^{\cF^*_S} \mid \*y_{\*x})
 \right.
 \right.
 \\
 & \qquad
 \left.
 \left.
 + 
 \eta_\lambda^{\cF^*_S}(\*x)  
 p(\*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} \mid \*y_{\*x}) 
 \right\}
 \right]
 \\ % --
 & \approx
 \frac{1}{K K_{\veps}} 
 \sum_{(\tilde{\cF}^*_S, \tilde{\*f}) \in F}
 \sum_{\tilde{\veps} \in E}
 \log
 \left\{
 \zeta_\lambda^{\tilde{\cF}^*_S}(\*x)
 p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{\*y}_{\*x})
 \right.
 \\ 
 & \qquad
 \left.
 + 
 \eta_\lambda^{\tilde{\cF}^*_S}(\*x)  
 p(\*f_{\*x} \in \cA_{U \setminus O}^{\tilde{\cF}^*_S} \mid \tilde{\*y}_{\*x}) 
 \right\}.
 %  \\ % --
 % & \approx
 % \frac{1}{K} \sum_{(\tilde{\cF}^*_S, \tilde{\*f}) \in F}
 % \log
 % \left\{
 % \zeta_\lambda^{\tilde{\cF}^*_S}(\*x)
 % \frac{1}{K_\veps} \sum_{\tilde{\veps} \in E}
 % p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \*y_{\*x})
 % \right.
 % \\ 
 % & \qquad
 % \left.
 % + 
 % \eta_\lambda^{\tilde{\cF}^*_S}(\*x)  
 % \frac{1}{K_\veps} \sum_{\tilde{\veps} \in E}
 % p(\*f_{\*x} \in \cA_{U \setminus O}^{\tilde{\cF}^*_S} \mid \*y_{\*x}) 
 % \right\},
\end{align*}
where $E$ is a set of $L$-dimension noise samples $\tilde{\veps}$ from $\cN(0,\sigma^2_{\rm noise} I)$, 
$\tilde{\*y}_{\*x} = \tilde{\*f}_{\*x} + \tilde{\veps}$
is a sample of $\*y_{\*x}$, and $K_{\veps} = |E|$. 
%
Note that, in this approximation, we transform 
$\EE_{\cF^*, \*y_{\*x}}$
to
$\EE_{\cF^*, \*f_{\*x}} \EE_{\*\veps}$, which is possible because of the independence of the noise term. 
%
To evaluate this MC approximation, we need the conditional distribution
$p(\*f_{\*x} \mid \tilde{\*y}_{\*x})$, written as
\begin{align*}
 \*f_{\*x} \mid \tilde{\*y}_{\*x}
 \sim \cN(\*\nu(\*x), \mr{diag} (\*s(\*x))),
\end{align*}
where 
\begin{align*}
 \nu_l(\*x) &= \mu_l(\*x) + \frac{\sigma_l^2(\*x)}{\sigma_l^2(\*x) + \sigma_{\rm noise}^2} (\tilde{y}^l_{\*x} - \mu_l(\*x)), 
 \\
 s_l(\*x) &= \sigma_l^2(\*x) - \frac{\sigma_l^4(\*x)}{\sigma_l^2(\*x) + \sigma_{\rm noise}^2}.
\end{align*}
% Therefore, 
% $p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{\*y}_{\*x})$
% and 
% $p(\*f_{\*x} \in \cA_{U \setminus O}^{\tilde{\cF}^*_S} \mid \tilde{\*y}_{\*x})
% =
% p(\*f_{\*x} \in \cA_{U}^{\tilde{\cF}^*_S} \mid \tilde{\*y}_{\*x})
% -
% p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{\*y}_{\*x})
% $
% can be calculated by using the same procedure as 
% $Z_O^{\tilde{\cF}^*_S} = p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S})$
% and 
% $Z_U^{\tilde{\cF}^*_S} = p(\*f_{\*x} \in \cA_U^{\tilde{\cF}^*_S})$, described in Appendix~\ref{app:CalcZ}.
% %
% First, 
% $p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{\*y}_{\*x})$ 
% is
Therefore, 
$p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{\*y}_{\*x})$
can be calculated by using the same procedure as 
$Z_O^{\tilde{\cF}^*_S} = p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S})$ shown in \eq{eq:decompose_Z_O}: 
\begin{align*}
 p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{\*y}_{\*x})
 & = \sum_{i = 1}^C \int_{C_i} 
 p(\*f_{\*x} \mid \tilde{\*y}_{\*x}) \mr{d} \*f_{\*x}
 \\
 & = \sum_{i = 1}^C
 \prod_{l = 1}^L
 \int_{\ell_i^l}^{u_i^l}
 p(f^l_{\*x} \mid \tilde{y}^l_{\*x}) \mr{d} f^l_{\*x}
 \\
 & = \sum_{i = 1}^C 
 \prod_{l = 1}^L
 \rbr{
 \Phi( \bar{\beta}_{i,l} ) 
 - \Phi( \underline{\beta}_{i,l} )
 }
\end{align*}
where
$\underline{\beta}_{i,l} = (\ell_i^l - \nu_l(\*x))/s_l(\*x)$
and
$\bar{\beta}_{i,l} = (u_i^l - \nu_l(\*x))/s_l(\*x)$. 
%
For
$p(\*f_{\*x} \in \cA_{U \setminus O}^{\tilde{\cF}^*_S} \mid \tilde{\*y}_{\*x})$,
we can use a relation
$p(\*f_{\*x} \in \cA_{U \setminus O}^{\tilde{\cF}^*_S} \mid \tilde{\*y}_{\*x})
=
p(\*f_{\*x} \in \cA_{U}^{\tilde{\cF}^*_S} \mid \tilde{\*y}_{\*x})
-
p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{\*y}_{\*x})$.
%
The last term
$p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \tilde{\*y}_{\*x})$
can be calculated by the same approach as 
$Z_U^{\tilde{\cF}^*_S} = p(\*f_{\*x} \in \cA_U^{\tilde{\cF}^*_S})$, described in the end of Appendix~\ref{app:CalcZ}.
%
% Because of the independence of $\*\veps$, 
% \begin{align*}
%  \EE_{\*\veps}\sbr{
%  p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \*y_{\*x})
%  }
% & = \sum_{i = 1}^C 
%  \prod_{l = 1}^L
%  \rbr{
%  \EE_{\veps}\sbr{ \Phi( \bar{\beta}_{i,l} ) }
%  - \EE_{\veps}\sbr{ \Phi( \underline{\beta}_{i,l} ) }
%  }
% \end{align*}



Figure~\ref{fig:results-noisy} shows the empirical evaluation for which the setting is same as in Section~\ref{ssec:GPDerivedArtificialFunctions}. 
%
Here, we used the $(d, L) = (3, 3)$ GP derived functions for three length scales. 
%
We added the independent noise $\cN(0, \sigma_{\rm noise}^2)$ with $\sigma_{\rm noise} = 0.1$ to all the observations.
%
The GPs have the same value of the noise parameter $\sigma_{\rm noise} = 0.1$.
%
We compared with EHVI, MOBO-RS, and JES.
%
EHVI and MOBO-RS can handle the noise just by incorporating it into the surrogate GPs.
%
JES \citep{Tu2022-joint} considers the information gain from noisy observations.
%
PFEV shows similar results to its noisy observation counterpart.
%
We empirically see that $\mr{MI}(\*f(\*x) ; \cF^*)$ sufficiently works even when the observation contains a moderate level of noise.
%
The investigation under stronger noise is our future work.

% --------------------------------------------------
% Fig: Results on noisy setting  
% --------------------------------------------------
\begin{figure*}
 \centering
 \subfigure[$\ell_{\rm RBL} = 0.05$]{
 \ig{.25}{./figs/Ext-Noisy/RHV_input_dim_3output_dim_3_length_scale_0.05.pdf}}
 \subfigure[$\ell_{\rm RBL} = 0.1$]{
 \ig{.25}{./figs/Ext-Noisy/RHV_input_dim_3output_dim_3_length_scale_0.1.pdf}}
 \subfigure[$\ell_{\rm RBL} = 0.25$]{
 \ig{.25}{./figs/Ext-Noisy/RHV_input_dim_3output_dim_3_length_scale_0.25.pdf}}
 \caption{Results with noisy observations in GP-derived synthetic functions (average and standard error of $10$ runs)}
 \label{fig:results-noisy}
\end{figure*}

% \begin{align*}
%  \underline{\beta}_{i,l}
%  &= 
%  \rbr{\ell_i^l - 
%  \mu_l(\*x) - \frac{\sigma_l^2(\*x)}{\sigma_l^2(\*x) + \sigma_{\rm noise}^2} (y^l_{\*x} - \mu_l(\*x))
%  }
%  /s_l(\*x)
%  \\ % --
%  &= 
%  \underbrace{
%  \rbr{\ell_i^l - 
%  \mu_l(\*x) - \frac{\sigma_l^2(\*x)}{\sigma_l^2(\*x) + \sigma_{\rm noise}^2} (f^l_{\*x} - \mu_l(\*x))
%  }
%  /s_l(\*x)}_{\eqqcolon w_0}
%  \\
%  & \qquad 
%  + 
%  \underbrace{
%  \frac{- \sigma_l^2(\*x)}{\sigma_l^2(\*x) + \sigma_{\rm noise}^2} /s_l(\*x)}_{\eqqcolon w_1} \ \veps
%  \\ % --
%  & =
%  w_0 + w_1 \veps.
% \end{align*}

% By using a general relation 
% $\int_{-\infty}^{\infty} \Phi(a + bx) \phi(x) \mr{d}x = \Phi(\frac{a}{\sqrt{1 + b^2}})$, we obtain
% \begin{align*}
%  \EE_{\veps}\sbr{ \Phi( \underline{\beta}_{i,l} ) }
%  = 
%  \Phi\rbr{
%  \frac{w_0}{\sqrt{1 + w^2_1}}
%  }. 
% \end{align*}
% %
% $\EE_{\veps}[ \Phi( \bar{\beta}_{i,l} ) ]$ 
% can also be obtained by the same transformation.
% %
% Therefore, 
% $\EE_{\*\veps}[ p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid \*y_{\*x}) ]$
% can be calculated analytically. 



% % --------------------------------------------------
% \subsection{Parallel Querying}

% % --------------------------------------------------
% \subsection{Decoupled Setting}

% For the decoupled setting, MI and its lower bound is 
% \begin{align*}
%  &\mr{MI}(y^l_{\*x} ; \cF^*) \\
%  &=
%  \EE_{\cF^*, y^l_{\*x}}\sbr{
%  \log \frac{q(y^l_{\*x} \mid \cF^{*})}{p(y^l_{\*x})} 
%  }
%  + D_{\mr{KL}}\rbr{ 
%  p(y^l_{\*x} \mid \cF^*) \parallel q(y^l_{\*x} \mid \cF^*) 
%  }
%  \\
%  &\geq
%  \EE_{\cF^*, y^l_{\*x}}\sbr{
%  \log \frac{q(y^l_{\*x} \mid \cF^{*})}{p(y^l_{\*x})} 
%  } \eqqcolon L_{\rm Dec}(\*x, \lambda).
% \end{align*}
% %
% Based on the same idea for the coupled case 
% $q(\*y_{\*x} \mid \cF^*)$, 
% we first decompose 
% \begin{align*}
%  q(y^l_{\*x} \mid \cF^{*})
%  = \int 
%  p(y^l_{\*x} \mid f^l_{\*x})
%  q(f^l_{\*x} \mid \cF^{*})
%  \mr{d} f^l_{\*x}. 
% \end{align*}
% %
% Substituting \eq{eq:decoupled-vd} into the right-hand-side, we obtain 
% \begin{align*}
%  q(y^l_{\*x} \mid \cF^{*})
%  & = 
%  \int 
%  p(y^l_{\*x} \mid f^l_{\*x})
%  p(f^l_{\*x}) 
%  \bigl\{
%  \zeta_\lambda^{\cF^*_S}(\*x) % f^l_{\*x}の確率的揺らぎは関係ないはず
%  p(\*f_{\*x} \in \cA_O^{\cF^*_S} \mid f^l_{\*x})
%  \notag \\
%  & \qquad \qquad \qquad
%  + 
%  \eta_\lambda^{\cF^*_S}(\*x)
%  p( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} \mid f^l_{\*x})
%  \bigr\}
%  \mr{d} f^l_{\*x}
%  \\ % --
%  & = 
%  p(y^l_{\*x})
%  \int 
%  p(f^l_{\*x} \mid y^l_{\*x} )
%  \bigl\{
%  \zeta_\lambda^{\cF^*_S}(\*x)
%  p(\*f_{\*x} \in \cA_O^{\cF^*_S} \mid f^l_{\*x})
%  \notag \\
%  & \qquad \qquad \qquad
%  + 
%  \eta_\lambda^{\cF^*_S}(\*x)
%  p( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} \mid f^l_{\*x})
%  \bigr\}
%  \mr{d} f^l_{\*x}
%  \\ % --
%  & = 
%  p(y^l_{\*x})
%  \bigl\{
%  \zeta_\lambda^{\cF^*_S}(\*x)
%  p(\*f_{\*x} \in \cA_O^{\cF^*_S} \mid y^l_{\*x})
%  \notag \\
%  & \qquad \qquad \qquad
%  + 
%  \eta_\lambda^{\cF^*_S}(\*x)
%  p( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} \mid y^l_{\*x})
%  \bigr\}
% \end{align*}
% %
% Then, the lower bound and its MC approximation is obtained as
% \begin{align*}
%  & L_{\rm Dec}(\*x, \lambda) 
%  \\ % --
%  & = 
%  \EE_{\cF^*, y^l_{\*x}} \biggl[
%  \log
%  \bigl\{
%  \zeta_\lambda^{\cF^*_S}(\*x)
%  p(\*f_{\*x} \in \cA_O^{\cF^*_S} \mid y^l_{\*x})
%  \notag \\
%  & \qquad \qquad \qquad
%  + 
%  \eta_\lambda^{\cF^*_S}(\*x)
%  p( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} \mid y^l_{\*x})
%  \bigr\}
%  \biggr]
%  \\ % --
%  & = 
%  \EE_{\cF^*, f^l_{\*x}} \biggl[
%  \log
%  \bigl\{
%  \zeta_\lambda^{\cF^*_S}(\*x)
%  \EE_{\veps}[
%  p(\*f_{\*x} \in \cA_O^{\cF^*_S} \mid y^l_{\*x})
%  ]
%  \notag \\
%  & \qquad \qquad \qquad
%  + 
%  \eta_\lambda^{\cF^*_S}(\*x)
%  \EE_{\veps}[
%  p( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} \mid y^l_{\*x})
%  ]
%  \bigr\}
%  \biggr]
%  \\ % --
%  & \approx
%  \frac{1}{K} \sum_{(\tilde{F}_S^*, \tilde{\*f}) \in F}
%  \log
%  \bigl\{
%  \zeta_\lambda^{\tilde{\cF}^*_S}(\*x)
%  \EE_{\veps}[
%  p(\*f_{\*x} \in \cA_O^{\tilde{\cF}^*_S} \mid y^l_{\*x})
%  ]
%  \notag \\
%  & \qquad \qquad \qquad
%  + 
%  \eta_\lambda^{\tilde{\cF}^*_S}(\*x)
%  \EE_{\veps}[
%  p( \*f_{\*x} \in \cA_{U \setminus O}^{\tilde{\cF}^*_S} \mid y^l_{\*x})
%  ]
%  \bigr\}
% \end{align*}
% %
% $p(\*f_{\*x} \in \cA_O^{\cF^*_S} \mid y^l_{\*x})$
% \begin{align*}
%  & p(\*f_{\*x} \in \cA_O^{\cF^*_S} \mid y^l_{\*x})
%  \\ % --
%  & = \sum_{i = 1}^C \int_{C_i} 
%  p(\*f_{\*x} \mid y^l_{\*x}) \mr{d} \*f_{\*x}
%  \\  % --
%  & = \sum_{i = 1}^C
%  \int_{\ell_i^l}^{u_i^l}
%  p(f^l_{\*x} \mid y^l_{\*x}) \mr{d} f^l_{\*x}
%  \prod_{l^\prm \neq l}
%  \int_{\ell_i^{l^\prm}}^{u_i^l}
%  p(f^{l^\prm}_{\*x}) \mr{d} f^{l^\prm}_{\*x}
%  \\  % --
%  & = \sum_{i = 1}^C 
%  \rbr{
%  \Phi( \bar{\beta}_{i,l^\prm} ) 
%  - \Phi( \underline{\beta}_{i,l^\prm} )
%  }
%  \prod_{l^{\prm} \neq l}
%  \rbr{
%  \Phi( \bar{\alpha}_{i,l^\prm} ) 
%  - \Phi( \underline{\alpha}_{i,l^\prm} )
%  }
% \end{align*}

% \begin{align*}
%  &
%  \EE_{\veps}[p(\*f_{\*x} \in \cA_O^{\cF^*_S} \mid y^l_{\*x})]
%  = 
%  \\  % --
%  & = \sum_{i = 1}^C 
%  \rbr{
%  \EE_{\veps}[ \Phi( \bar{\beta}_{i,l^\prm} ) ]
%  - \EE_{\veps}[ \Phi(  \underline{\beta}_{i,l^\prm} ) ]
%  }
%  \prod_{l^{\prm} \neq l}
%  \rbr{
%  \Phi( \bar{\alpha}_{i,l^\prm} ) 
%  - \Phi( \underline{\alpha}_{i,l^\prm} )
%  }
% \end{align*}



% $\EE_{\veps}[p( \*f_{\*x} \in \cA_{U \setminus O}^{\cF^*_S} \mid y^l_{\*x})]$

% --------------------------------------------------
% \subsection{Joint Entropy}


% \endgroup

% \remove{

% \section{GP with Additional Observations}

% For a set $\cX_q = \{\*x_1, \ldots, \*x_q\}$, define 
% $\*f^l_{\cX_q} = (f^l_{\*x_1}, \ldots, f^l_{\*x_q})^\top$.
% %
% The predictive distribution for $\cX_q$ of the $l$-th objective function is denoted as
% \begin{align*}
%  \*f^l_{\cX_q} \sim \cN(\*\mu^l_{\cX_q}, \Sigma^l_{\cX_q})
% \end{align*}
% where
% $\*\mu^l_{\cX_q} = (\mu^l_{\*x_1}, \ldots, \mu^l_{\*x_q})^\top$
% and 
% $\Sigma^l_{\cX_q} \in \RR^{q \times q}$ is the predictive covariance matrix.
% %

% $p(\*f_{\*x} \mid \*f^l_{\cX_q})$

% \begin{align*}
%  \*f_{\*x} \mid \*f^l_{\cX_q}
%  \sim 
%  \cN(\*\nu_{\*x \mid q}, \mr{diag}(\*s_{\*x \mid q}))
% \end{align*}
% \begin{align*}
%  \nu^l_{\*x \mid q}
%  = \mu^l_{\*x} + 
%  \Sigma^l_{\cX_q}
%  (\Sigma^l_{\cX_q})^{-1}
%  \*f^l_{\cX_q}
% \end{align*}
% }

% --------------------------------------------------
\section{Additional Discussion on Related Work}
\label{app:related-work}


Although our main focus is on information-theoretic approaches, here, other criteria are also reviewed.
% ParEGO（\citep{Knowles2006-parego}）はスカラー化に基づく初期の多目的ベイズ最適化手法としてよく知られているが，スカラー化によって目的関数が圧縮され情報の損失が起きると思われる．
A classical approach is the scalarization that transforms multiple objective functions into a scalar value, among which ParEGO \citep{Knowles2006-parego} is a well-known method based on a random scalarization. 
%
However, the information of the Pareto-frontier may be lost by the scalarization.
% ParEGO \citep{Knowles2006-parego} is widely known as a classical scalarization based MOBO, but the random scalarization may lose the information of Pareto-frontier.
%
% 標準的な期待改善（EI）の拡張として，パレート超体積の増加を考慮する手法（\citep{Emmerich2005-single}）があり，これを期待超体積改善（EHVI）と呼ぶ．さらに，\citep{Shah2016-pareto}はEHVIを相関のある目的関数に拡張した．EIは広く受け入れられている基準であるが計算量が大きいことが知られている．
The standard expected improvement (EI) has been extended based on measuring the improvement of the hyper-volume called EHVI (expected hyper-volume improvement) \citep{Emmerich2005-single,Shah2016-pareto}.
%
% Upper confidence bound（UCB）はBOのもう一つの有名な獲得関数である（\citep{Srinivas2010-Gaussian}）．SMSego（\citep{Ponweiser2008-multiobjective}）は超体積を楽観的に評価するUCBベースのアプローチの一つである．
The GP upper confidence bound (UCB) is another well-known general approach to BO \citep{Srinivas2010-Gaussian}. 
%
UCB based MOBO methods have been studied \citep{Ponweiser2008-multiobjective,Zuluaga2013-active,Zuluaga2016-pal}, but the setting of the confidence interval sometimes becomes practically difficult.
% PALと$\epsilon$-PAL（\citep{Zuluaga2013-active}, \citep{Zuluaga2016-pal}）は，パレートフロンティアの信頼区間に基づく評価を提案する別のUCBアプローチである．\citep{Shilton2018-multi}はUCB基準を定義するために，クエリされた点とパレートフロンティアの間の距離を評価する．
% UCBアプローチの課題は，不確実性項の影響をバランスさせるハイパーパラメータにある．
%
% SUR \citep{Picheny2015-multiobjective}）は不確実性低減の指標として改善確率（PI）の期待減少量を考慮する．しかしながら，SURは計算コストが極めて高い．
SUR \citep{Picheny2015-multiobjective} is based on the reduction of PI after the querying, which is computationally quite expensive. 
% これは，問い合わせ点を訓練集合に追加した後のPIを入力空間 $\mathcal{X}$ 全体で積分する必要があり，入力空間の次元に対するスケーラビリティが著しく制限されるためである．
% KG\citep{}の多目的拡張としてHypervolume KG \citep{daulton23-hypervolume}が提案されている．Hypervolume KGの直接計算は非常に重いため近似を導入する．入れ子上の最適化を同時最適化に変換するone shotアプローチが採用されているが，次元が上がる．
A hypervolume-based multi-objective extension of knowledge gradient (KG) is considered by \citep{daulton23-hypervolume}. 
%
Na\"ive computations of the hypervolume KG are computationally intractable, and several approximation and acceleration strategies have been studied. 
%
For example, so-called one-shot strategy transforms the nested optimization into simultaneous optimization which makes computation much faster, but the dimension of the acquisition function optimization becomes high.
% Hypervolume KGの直接計算は非常に重いため，離散的に一手先のHypervolumeを有限の点だけに限って評価している．
% 理論上のrateはboundされているが実践上rateの定数がどの程度の誤差かは不明である．
% また，入れ子上の最適化を同時最適化に変換するone shotアプローチが採用されているが，次元が上がる．

% 本論文では，特に情報論的アプローチに焦点を当てる．このアプローチは単一目的のBOにおいて成功を収めている（\citep{Henning2012-Entropy}, \citep{Hernandez2014-Predictive}, \citep{Wang2017-Max}）．
We focus on the information-theoretic approach, which was first proposed for single-objective BO \citep{Henning2012-Entropy,Hernandez2014-Predictive,Wang2017-Max}.
%
% \citep{cheng2024-variational}は単一の目的関数で変分下限最大化によるBOを提案しているが，単目的であり本研究とは趣旨が大きく異なる．
Recently, \citep{cheng2024-variational} proposed a different variational lower bound approach to single-objective BO, which is only for single-objective problems.
%
A seminal work in the information-theoretic approach to MOBO is the Predictive Entropy Search for Multi-Objective Optimization (PESMO) \citep{Hernandez-lobatoa2016-Predictive}.
%
PESMO defines an acquisition function through the entropy of the set of Pareto-optimal solutions $\*x$, which is based on complicated approximation by expectation propagation (EP) \citep{Minka2001-Minka}.
% 多目的最適化におけるこの方向性の先駆的な研究として，パレート最適な $\boldsymbol{x}$ の集合のエントロピーを通じて獲得関数を定義する predictive entropy search for multiobjective optimization（PESMO）がある（\citep{Hernandez-lobatoa2016-Predictive}）．
%
% 彼らは，エントロピーに基づく獲得関数が他の種類の基準と比較して優れた性能を達成できることを示した．
%
% しかしながら，PESMOは期待値伝播（EP）（\citep{Minka2001-Minka}）に基づく近似を採用しているが結果として得られる獲得関数の計算は極めて複雑である．
%%
% これは，エントロピーの直接的な評価が計算上扱いづらいためである．
%
%彼らのEPでは，非ガウス密度がガウス密度で置き換えられ，この置換の精度と信頼性を示すことは難しい．
%
% さらに，結果として得られる獲得関数の計算は極めて複雑である．
%
% 一方，\citep{Belakaria2019-max}は各次元 $l=1, \ldots, L$ の最大値のエントロピーを用いることを提案し，これを max-value entropy search for multi-objective optimization（MESMO）と呼んだ．
On the other hand, \citet{Belakaria2019-max} proposed using the individual max-value entropy of each objective function, called max-value entropy search for multi-objective optimization (MESMO).
%
% これにより計算は大幅に簡略化されるが明らかにPareto-frontierの情報を失っている．
This largely simplifies the computations, but obviously, information of the Pareto-frontier is lost.
%
% 最近JES baseの多目的がもう一つ提案された．
Another JES based approach has been recently proposed \citep{sanchez2024-joint}, which is in a more general formulation including multi-fidelity and constrained problems. 
%
Their computations are based on the Gaussian based entropy approximation, whose validity remains unclear.
% これはmulti-fidelityや制約などより汎用性のある形で提案されているが，Pareto-frontier givenの分布の近似にガウス分布を使うがこの妥当性は不明である．
% This has been proposed in a more general form, such as for multi-fidelity and constrained problems, but it uses a Gaussian distribution to approximate the distribution given the Pareto frontier, the validity of which remains unclear.
% これにより計算は大幅に簡略化されるが，明らかに，各軸の最大値付近に値を持たない $\boldsymbol{f}_{\boldsymbol{x}} \in \mathcal{F}^{*}$ はこの基準では好まれない．
%
% これは，多目的最適化問題において本質的に重要となることが多い目的関数間のトレードオフ関係を捉えることができないことを意味する．

% KG?

% BOtie 

% lower bound系？


% 多目的最適化問題に対して，スカラー化と進化計算を組み合わせる手法が広く用いられてきた（例えば，\citep{Knowles2006-parego}, \citep{Zhang2009-expensive}）．特に，ParEGO（\citep{Knowles2006-parego}）はその優れた性能で広く知られている．スカラー化アプローチは，多目的最適化を単一目的問題に変換し，一定の正則性条件の下でパレート最適解を得ることができる．しかしながら，変換された単一目的に対する獲得関数は最適性を欠く可能性がある．近年，パレートフロンティアの特定の部分集合を識別するためのスカラー化の拡張が研究されているが（\citep{Paria2020-flexible}, \citep{Astudillo2017-multi}），本論文ではパレートフロンティア全体の識別に焦点を当てる．

% 通常のベイズ最適化（BO）の獲得関数を拡張することは，多目的最適化研究において一般的なアプローチとなっている．標準的な期待改善（EI）の拡張として，パレート超体積の増加を考慮する手法（\citep{Emmerich2005-single}）があり，これを期待超体積改善（EHVI）と呼ぶ．さらに，\citep{Shah2016-pareto}はEHVIを相関のある目的関数に拡張した．EIは広く受け入れられている基準であるが，局所的な有用性のみを測る．
% Upper confidence bound（UCB）はBOのもう一つの有名な獲得関数である（\citep{Srinivas2010-Gaussian}）．SMSego（\citep{Ponweiser2008-multiobjective}）は超体積を楽観的に評価するUCBベースのアプローチの一つである．
% % PALと$\epsilon$-PAL（\citep{Zuluaga2013-active}, \citep{Zuluaga2016-pal}）は，パレートフロンティアの信頼区間に基づく評価を提案する別のUCBアプローチである．\citep{Shilton2018-multi}はUCB基準を定義するために，問い合わせ点とパレートフロンティアの間の距離を評価する．
% UCBアプローチの課題は，不確実性項の影響をバランスさせるハイパーパラメータにある．

% \citep{Campigotto2013-active}は，パレートフロンティアを関数として直接モデル化するための不確実性サンプリングを考案した．最も単純な不確実性サンプリングは問い合わせ点における局所的な不確実性のみを測るが，大域的な不確実性測度も研究されている．
% SUR（\citep{Picheny2015-multiobjective}）は不確実性低減の指標として改善確率（PI）の期待減少量を考慮する．しかしながら，SURは計算コストが極めて高い．これは，問い合わせ点を訓練集合に追加した後のPIを入力空間 $\mathcal{X}$ 全体で積分する必要があり，入力空間の次元に対するスケーラビリティが著しく制限されるためである．

% 本論文では，特に情報論的アプローチに焦点を当てる．このアプローチは単一目的のBOにおいて成功を収めている（\citep{Henning2012-Entropy}, \citep{Hernandez2014-Predictive}, \citep{Wang2017-Max}）．
% 多目的最適化におけるこの方向性の先駆的な研究として，パレート最適な $\boldsymbol{x}$ の集合のエントロピーを通じて獲得関数を定義する predictive entropy search for multiobjective optimization（PESMO）がある（\citep{Hernandez-lobatoa2016-Predictive}）．
% 彼らは，エントロピーに基づく獲得関数が他の種類の基準と比較して優れた性能を達成できることを示した．
% しかしながら，PESMOは期待値伝播（EP）（\citep{Minka2001-Minka}）に基づく近似を採用している．
% これは，エントロピーの直接的な評価が計算上扱いづらいためである．
% 彼らのEPでは，非ガウス密度がガウス密度で置き換えられ，この置換の精度と信頼性を示すことは難しい．
% さらに，結果として得られる獲得関数の計算は極めて複雑である．
% 一方，\citep{Belakaria2019-max}は各次元 $l=1, \ldots, L$ の最大値のエントロピーを用いることを提案し，こ
% れを max-value entropy search for multi-objective optimization（MESMO）と呼んだ．
% これにより計算は大幅に簡略化されるが，明らかに，各軸の最大値付近に値を持たない $\boldsymbol{f}_{\boldsymbol{x}} \in \mathcal{F}^{*}$ はこの基準では好まれない．
% これは，多目的最適化問題において本質的に重要となることが多い目的関数間のトレードオフ関係を捉えることができないことを意味する．
% % （既存の情報論的手法との関係については，第5節でさらに議論する\red{(少なくともIBISMLではこの議論は（長くなるので）不要？)}．）
% % --------------------------------------------------
% 最近の情報論的手法として，まずJoint Entropy Search（JES）が挙げられる．\citep{Tu2022-joint}は最適な入出力集合に対するjoint entropyを用いることを提案し，
% これをJoint Entropy Search（JES）と呼んだ．JESは多目的ベイズ最適化において初めてjoint entropyを導入したという点で重要な貢献がある．
% しかしながら，JESは過剰な切断に基づく近似を採用している．これは，分布$p\left(\boldsymbol{y} \mid \boldsymbol{x}, \mathcal{D}_{n},\left(\mathcal{X}^{*}, \mathcal{Y}^{*}\right)\right)$の直接的な評価が計算上扱いづらいためである．
% 彼らの過剰な切断に基づく近似では，その置換により情報量の非負性を示すことは難しい．
% さらに，結果として得られる獲得関数の近似は極めて複雑である．
% 次に，Pareto-frontier entropy search（PFES）がある．
% \citep{Suzuki2020-multi}はパレート最適な$\boldsymbol{x}$との情報量を用いることを提案し，
% これをPareto-frontier entropy search（PFES）と呼んだ．
% しかしながら，PFESも過剰な切断に基づく近似を採用しており，
% 彼らの過剰な切断に基づく近似でも，情報量の非負性を示すことは難しい．
% 最後に，Parallel Feasible Pareto Frontier Entropy Search（$\{\text{PF}\}^{2}\text{ES}$）について述べる．
% \citep{Qing2022-text}はパレート最適な$\boldsymbol{x}$との情報量に対する変分下限を用いることを提案し，
% これを$\{\text{PF}\}^{2}\text{ES}$と呼んだ．
% この手法では，over-truncationからなる，切断領域の過大評価を避けるために，離散パレートフロンティア$\cF^*_S$をシフトするための小さなペナルティベクトル$\boldsymbol{\varepsilon}=\left[\varepsilon_{1}, \ldots, \varepsilon_{L}\right]$を導入し，離散的なパレートフロンティアの近似をシフトする．
% 彼らは，目的関数が2つの場合に，真のパレートフロンティアの極値となるすべての点が，サンプリングされたパレートフロンティアの集合$\mathrm{PF}$に含まれており，かつ，$|\mathrm{PF}| \to \infty$を満たすという，極端な仮定の下で，獲得関数$\alpha_{\{\mathrm{PF}\}^{2} \mathrm{ES}}$が変分下限であるための$\boldsymbol{\varepsilon}$を構築可能であると主張している．
% しかしながら，\citep{Qing2022-text}ではVDCを考慮できていないため，この主張の審議について検証が必要と思われるが現時点では明らかにできていない．

% \begin{itemize}
%   \item JES
%   \begin{itemize}
%     \item \citep{Tu2022-joint}は最適な入出力集合に対するjoint entropyを用いることを提案し，これをJoint Entropy Search:JESと呼んだ．
%     \item JESの貢献　joint entropyを初めてMOBOに導入
%     \item しかしながらJESは過剰な切断に基づく近似を採用している．これは，分布$p\left(\mathcal{y} \mid \mathcal{x}, \mathcal{D_{n}},\left(\mathcal{X}^{*}, \mathcal{Y}^{*}\right)\right)$の直接的な評価が計算上扱いづらいためである．
%     \item 彼らの過剰な切断に基づく近似では，彼らの置換により情報量の非負性を示すことは難しい．
%     \item さらに，結果として得られる獲得関数の近似は極めて複雑である．
%   \end{itemize}
%   \item PFES
%   \begin{itemize}
%     \item \citep{Suzuki2020-multi}はパレート最適な$\boldsymbol{x}$との情報量を用いることを提案し，これをPareto-frontier entropy search:PFESと読んだ．
%     \item PFESの貢献
%     \item しかしながら，PFESは過剰な切断に基づく近似を採用している．これは，
%     \item 彼らの過剰な切断にも続く近似では，彼らの置換により情報量の非負性を示すことは難しい．
%     \item さらに，
%   \end{itemize}
 %   \item $\{\text{PF}\}^{2}\text{ES}$
%   \begin{itemize}
%     \item \citep{Qing2022-text}はパレート最適な$\boldsymbol{x}$との情報量に対する変分下限を用いることを提案し，これをParallel Feasible Pareto Frontier Entropy Search:$\{\text{PF}\}^{2}\text{ES}$と呼んだ．
%     \item $\{\text{PF}\}^{2}\text{ES}$の貢献
%     \item この，超直方体への分解から生じる$\mathcal{A}_{\mathcal{F}^{*}}$の過大評価を避けるために，
%     \citep{Qing2022-text}では，
%     $\mathcal{F}^{*}_{\boldsymbol{F}}:=\mathcal{F}^{*}+\boldsymbol{\varepsilon}$として，
%     離散パレートフロンティア$\cF^*_S$の近似をシフトするための小さなペナルティベクトル$\boldsymbol{\varepsilon}=\left[\varepsilon_{1}, \ldots, \varepsilon_{L}\right]$を導入し，離散的なパレートフロンティアの近似をシフトすることを提案した．
%     \item 彼らは，目的関数が2つの場合に，真のパレートフロンティアの極値となるすべての点が，サンプリングされたパレートフロンティアの集合$\mathrm{PF}$に含まれており，かつ，$|\mathrm{PF}| \to \infty$を満たすという，
%     極端な仮定の下で，獲得関数$\alpha_{\{\mathrm{PF}\}^{2} \mathrm{ES}}$が変分下限であるための$\boldsymbol{\varepsilon}$を構築可能であると主張している．
%     しかしながら，\citep{Qing2022-text}ではVDCを考慮できていないため，この主張の審議について検証が必要と思われるが現時点では明らかにできていない．
%   \end{itemize}
% \end{itemize}



% --------------------------------------------------
% \section{ベイズ最適化の設定}
\section{Detail of Experimental Settings}
\label{app:bo-settings}

% 本節では，計算機実験におけるベイズ最適化の設定について述べる．
%
% 本稿の計算機実験においてベイズ最適化はPythonパッケージのGPy\citep{GPy2014}を用いて実装されている．
Bayesian optimization was implemented by a Python package called GPy \citep{GPy2014}.
%
% 目的関数値は標準化し，訓練データは正規化する．
%
% 目的関数$f_{l}(\boldsymbol{x})$のGPモデルは以下のように定義されるRBFカーネルを用いて構築される．
% \begin{align*}
%  % k\left(\*x, \*x^{\prime}\right)=\theta_1 \exp \left(-\frac{\left\|\*x-\*x^{\prime}\right\|^2}{\theta_2}\right).
% \end{align*}
% ただし，$\theta_1, \theta_{2} \in \mathbb{R}$はハイパーパラメータである．
% すべての実験において，$\theta_1$は1.0に固定し，$\theta_2$のみを反復ごとに周辺尤度最大化により最適化する．
% パレートサンプリングのサンプルサイズは全手法で10とし，獲得関数の最大化にはDIRECTアルゴリズム\citep{Jones1993-lipschitzian}を用いる．
% 目的関数値は標準化し，訓練データは正規化する．初期観測点は5点をランダムに選択する．
%
% PFEVとPFESおよび$\{\text{PF}\}^{2}\text{ES}$で必要となる領域$\mathcal{C}_{m}$のセル分割には，quick hypervolume（QHV）\citep{Russo2014-quick}を用いる．
PFEV, PFES, and $\{\text{PF}\}^{2}\text{ES}$ require $\cC_i$ that are hyper-rectangles decomposing the dominated region. 
%
To obtain $\cC_i$, we used quick hypervolume (QHV) \citep{Russo2014-quick}, which is an efficient recursive algorithm originally proposed for the Pareto hyper-volume calculation.
%
% QHVは分割統治法に基づき，領域を再帰的に分割しながら超体積計算を行う手法である．
%
% 領域の定義の詳細は詳細はAppendix~\ref{app:CalcZ}に記述する．
In PFEV, we maximize $\lambda$ for each given $\*x$ by calculating 
$\wh{\mr{LB}}(\*x, \lambda)$ 
for $11$ grid points of $\lambda$ ($10^{-3}, 0.1, 0.2, \ldots, 1.0$).
%
In RFM used for sampling $\cF^*$ (required in PFEV, PFES, MESMO, $\{\text{PF}\}^{2}\text{ES}$, and JES), the number of bases $D$ was $500$.
%
The GP hyper-parameter $\sigma^2_{\rm noise}$ is fixed as $10^{-4}$.
%
In ParEGO, the coefficient parameter in the augmented Tchebycheff function was set $0.05$ as shown in \citep{Knowles2006-parego}.
% , and the coefficient $\beta$ of the confidence bound in SMSego was set $\beta = \Phi^{-1}(0.5+1/2^{L})$, where $\Phi$ is the cumulative distribution function of the standard normal distribution.
%
In EHVI, the two reference points are required, shown as 
$\*v_{\rm ref}$
and 
$\*w_{\rm ref}$ 
in \citep{Shah2016-pareto}.
%
The worst point vector
$\*v_{\rm ref}$
is defined by subtracting $10^{-4}$ from the vector consisting of the minimum value of each dimension of 
$\*y_i$
in the training data. 
%
On the other hand, the ideal point vector
$\*w_{\rm ref}$ 
is defined by adding $1$ to the vector consisting of the maximum value of each dimension of $\*y_i$.


The definition of each benchmark function is as follows.
\begin{itemize}
 \item Fonseca-Fleming \citep{Fonseca1995-multiobjective}
\begin{align*}
f_1(\boldsymbol{x}) &= 1 - \exp \left[-\sum_{i=1}^{d} \left(x_i - \frac{1}{\sqrt{d}}\right)^2\right] \\
f_2(\boldsymbol{x}) &= 1 - \exp \left[-\sum_{i=1}^{d} \left(x_i + \frac{1}{\sqrt{d}}\right)^2\right] \\
\text{subject to} &\quad -4 \leq x_i \leq 4, \quad i \in [d]. % i = 1,2,\dots,d.
\end{align*}
 \item Kursawe \citep{Kursawe1990-variant}
\begin{align*}
f_1(\boldsymbol{x}) &= \sum_{i=1}^{2} \left[ -10 \exp \left( -0.2 \sqrt{x_i^2 + x_{i+1}^2} \right) \right] \\
f_2(\boldsymbol{x}) &= \sum_{i=1}^{3} \left[ |x_i|^{0.8} + 5 \sin(x_i^3) \right] \\
\text{subject to} &\quad -5 \leq x_i \leq 5, \quad 1 \leq i \leq 3.
\end{align*}
% \begin{align*}
% f_1(\boldsymbol{x}) &= \sum_{i=1}^{d-1} \left[ -10 \exp \left( -0.2 \sqrt{x_i^2 + x_{i+1}^2} \right) \right] \\
% f_2(\boldsymbol{x}) &= \sum_{i=1}^{d} \left[ |x_i|^{0.8} + 5 \sin(x_i^3) \right] \\
% \text{subject to} &\quad -5 \leq x_i \leq 5, \quad i \in [d]. % i = 1,2,\dots,d.
% \end{align*}
 \item Viennet \citep{Vlennet1996-multicriteria}
\begin{align*}
f_1(x, y) &= 0.5 \left( x^2 + y^2 \right) + \sin \left( x^2 + y^2 \right) \\
f_2(x, y) &= \frac{(3x - 2y + 4)^2}{8} + \frac{(x - y + 1)^2}{27} + 15 \\
f_3(x, y) &= \frac{1}{x^2 + y^2 + 1} - 1.1 \exp \left( - (x^2 + y^2) \right) \\
\text{subject to} &\quad -3 \leq x, y \leq 3.
\end{align*}
% \begin{align*}
% f_1(\boldsymbol{x}) &= 0.5 \sum_{i=1}^{d} x_i^2 + \sin \left( \sum_{i=1}^{d} x_i^2 \right) \\
% f_2(\boldsymbol{x}) &= \sum_{i=1}^{d} \left( \frac{(3x_i - 2x_{i+1} + 4)^2}{8} + \frac{(x_i - x_{i+1} + 1)^2}{27} \right) + 15 \\
% f_3(\boldsymbol{x}) &= \frac{1}{\sum_{i=1}^{d} x_i^2 + 1} - \exp \left( -\sum_{i=1}^{d} x_i^2 \right) \\
% \text{subject to} &\quad -3 \leq x_i \leq 3, \quad i \in [d]. % i = 1,2,\dots,d.
% \end{align*}
 \item FES1 \citep{Fieldsend2003-using}
\begin{align*}
f_1(\boldsymbol{x}) &= \sum_{i=1}^{d} \left| x_i - \exp \left( \frac{(i/d)^2}{3} \right) \right|^{0.5} \\
f_2(\boldsymbol{x}) &= \sum_{i=1}^{d} \left( x_i - 0.5 \cos \left( \frac{10\pi i}{d} \right) - 0.5 \right)^2 \\
\text{subject to} &\quad 0 \leq x_i \leq 1, \quad i \in [d]. % i = 1,2,\dots,d.
\end{align*}
 \item FES2 \citep{Fieldsend2003-using}
       {\small
\begin{align*}
f_1(\boldsymbol{x}) &= \sum_{i=1}^{d} \left( x_i - 0.5 \cos \left( \frac{10\pi i}{d} \right) - 0.5 \right)^2 \\
f_2(\boldsymbol{x}) &= \sum_{i=1}^{d} \left| x_i - \sin^2(i-1) \cos^2(i-1) \right|^{0.5} \\
f_3(\boldsymbol{x}) &= \sum_{i=1}^{d} \left| x_i - 0.25 \cos(i-1) \cos(2i-2) - 0.5 \right|^{0.5} \\
\text{subject to} &\quad 0 \leq x_i \leq 1, \quad i \in [d]. % i = 1,2,\dots,d.
\end{align*}}%
 \item FES3 \citep{Fieldsend2003-using}
{\small
\begin{align*}
f_1(\*{x}) &= -\sum_{i=1}^d \left|x_i - \frac{\exp\left(\left(\frac{i}{d}\right)^2\right)}{3}\right|^{0.5}, \\
f_2(\*{x}) &= -\sum_{i=1}^d \left|x_i - \sin(i-1)^2 \cos(i-1)^2\right|^{0.5}, \\
f_3(\*{x}) &= -\sum_{i=1}^d | x_i - (0.25 \cos(i-1) \cos(2i-1) \\
& \qquad - 0.5 ) |^{0.5}, \\
f_4(\*{x}) &= -\sum_{i=1}^d \left(x_i - \frac{1}{2}\sin\left(1000\pi\frac{i}{d}\right) - \frac{1}{2}\right)^2 \\
\text{subject to} &\quad 0 \leq x_i \leq 1, \quad i \in [d]. % i=1, 2, \ldots, d.
\end{align*}}%
\end{itemize}

% --------------------------------------------------
\section{Additional Results of Empirical Evaluation}
\label{app:additional_experiments}

% --------------------------------------------------
\subsection{Additional Results on GP-derived Synthetic Functions}
\label{app:additional_experiments_GP}


Additional results on GP-derived synthetic functions are shown in Fig.~\ref{fig:results-GP-App-d2}-\ref{fig:results-GP-App-d4}.
%
The results are all combinations of 
$\ell_{\rm RBF} \in \{ 0.05, 0.1, 0.25 \}$,
$L \in \{2, 3, 4, 5, 6\}$,
and
$d \in \{2, 3, 4\}$ (Note that the results in the main text Fig.~\ref{fig:results-GP} are also included).
%
We here also show results of ParEGO, MOBO-RS, and MESMO, which are omitted in the main text.
%\remove{(Note that $\ell_{\rm RBF} = 0.1$ in $d \in \{2, 3\}$ is the same results as the main text).}
% \red{(Note that the main text only includes our method's results for $\ell_{\rm RBF} = 0.1$ in $d \in \{2, 3\}$, while PerEGO, MOBO-RS, and MESMO results for this setting appear exclusively in Fig.~\ref{fig:results-GP-App-d2}-\ref{fig:results-GP-App-d4}).}
%
The same format of boxplots as Fig~\ref{fig:GP-boxplot} created from all the results are shown in Fig.~\ref{fig:GP-boxplot-all}.
%
We also examined an input dimension wise boxplot in Fig.~\ref{fig:GP-boxplot-input-dim} in which differences of all the methods gradually decrease with the increase of the input dimension.
%
We further plot separately for each length scale setting of the true objective function in Fig~\ref{fig:GP-boxplot-input-dim-len-scale}.  
%
We see that, particularly for small length scale problems (which tends to be multi-modal functions), differences become small. 
%
We speculate that the differences were less apparent for challenging problems with high-dimensional and highly multi-modal functions.


Further, Fig.~\ref{fig:BayesMAP-boxplot-app} is performance difference between Bayes MAP \eq{eq:LB-MAP} and na{\"i}ve MC \eq{eq:LB-MC}. 



% --------------------------------------------------
% Fig: GP data regret
% --------------------------------------------------
\begin{figure*}
\centering
\subfigure[{\small $(L, \ell_{\rm RBF}) = (2, 0.05)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_2output_dim_2_length_scale_0.05.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (3, 0.05)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_2output_dim_3_length_scale_0.05.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (4, 0.05)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_2output_dim_4_length_scale_0.05.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (5, 0.05)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_2output_dim_5_length_scale_0.05.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (6, 0.05)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_2output_dim_6_length_scale_0.05.pdf}
} \hspace{-.5em}

\subfigure[{\small $(L, \ell_{\rm RBF}) = (2, 0.1)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_2output_dim_2_length_scale_0.1.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (3, 0.1)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_2output_dim_3_length_scale_0.1.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (4, 0.1)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_2output_dim_4_length_scale_0.1.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (5, 0.1)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_2output_dim_5_length_scale_0.1.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (6, 0.1)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_2output_dim_6_length_scale_0.1.pdf}
} \hspace{-.5em}

\subfigure[{\small $(L, \ell_{\rm RBF}) = (2, 0.25)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_2output_dim_2_length_scale_0.25.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (3, 0.25)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_2output_dim_3_length_scale_0.25.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) \! = \! (4, 0.25)$}]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_2output_dim_4_length_scale_0.25.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (5, 0.25)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_2output_dim_5_length_scale_0.25.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (6, 0.25)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_2output_dim_6_length_scale_0.25.pdf}
} \hspace{-.5em}

\caption{Results on GP-derived synthetic function ($d = 2$)}
\label{fig:results-GP-App-d2}
\end{figure*}


\begin{figure*}
\centering
\subfigure[{\small $(L, \ell_{\rm RBF}) = (2, 0.05)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_3output_dim_2_length_scale_0.05.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (3, 0.05)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_3output_dim_3_length_scale_0.05.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (4, 0.05)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_3output_dim_4_length_scale_0.05.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (5, 0.05)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_3output_dim_5_length_scale_0.05.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (6, 0.05)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_3output_dim_6_length_scale_0.05.pdf}
} \hspace{-.5em}

\subfigure[{\small $(L, \ell_{\rm RBF}) = (2, 0.1)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_3output_dim_2_length_scale_0.1.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (3, 0.1)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_3output_dim_3_length_scale_0.1.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (4, 0.1)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_3output_dim_4_length_scale_0.1.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (5, 0.1)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_3output_dim_5_length_scale_0.1.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (6, 0.1)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_3output_dim_6_length_scale_0.1.pdf}
} \hspace{-.5em}

\subfigure[{\small $(L, \ell_{\rm RBF}) = (2, 0.25)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_3output_dim_2_length_scale_0.25.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (3, 0.25)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_3output_dim_3_length_scale_0.25.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) \! = \! (4, 0.25)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_3output_dim_4_length_scale_0.25.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (5, 0.25)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_3output_dim_5_length_scale_0.25.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (6, 0.25)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_3output_dim_6_length_scale_0.25.pdf}
} \hspace{-.5em}

\caption{Results on GP-derived synthetic function ($d = 3$)}
\label{fig:results-GP-App-d3}
\end{figure*}


\begin{figure*}
\centering
\subfigure[{\small $(L, \ell_{\rm RBF}) = (2, 0.05)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_4output_dim_2_length_scale_0.05.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (3, 0.05)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_4output_dim_3_length_scale_0.05.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (4, 0.05)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_4output_dim_4_length_scale_0.05.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (5, 0.05)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_4output_dim_5_length_scale_0.05.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (6, 0.05)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_4output_dim_6_length_scale_0.05.pdf}
} \hspace{-.5em}

\subfigure[{\small $(L, \ell_{\rm RBF}) = (2, 0.1)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_4output_dim_2_length_scale_0.1.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (3, 0.1)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_4output_dim_3_length_scale_0.1.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (4, 0.1)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_4output_dim_4_length_scale_0.1.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (5, 0.1)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_4output_dim_5_length_scale_0.1.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (6, 0.1)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_4output_dim_6_length_scale_0.1.pdf}
} \hspace{-.5em}

\subfigure[{\small $(L, \ell_{\rm RBF}) = (2, 0.25)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_4output_dim_2_length_scale_0.25.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (3, 0.25)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_4output_dim_3_length_scale_0.25.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) \! = \! (4, 0.25)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_4output_dim_4_length_scale_0.25.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (5, 0.25)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_4output_dim_5_length_scale_0.25.pdf}
} \hspace{-.5em}
\subfigure[{\small $(L, \ell_{\rm RBF}) = (6, 0.25)$ }]{
 \ig{.19}{./figs/GP-appendix/RHV_input_dim_4output_dim_6_length_scale_0.25.pdf}
} \hspace{-.5em}

\caption{Results on GP-derived synthetic function ($d = 4$)}
\label{fig:results-GP-App-d4}
\end{figure*}





% --------------------------------------------------
% Fig: GP data boxplot: 出力次元の変化
% --------------------------------------------------
\begin{figure}
 \centering

 \ig{.4}{./figs/GP-boxplot-all/GP-boxplot-legend.pdf}

 \vspace{-.5em}

\subfigure[$L = 2$]{
 \ig{.09}{./figs/GP-boxplot-all/boxplot_L2.pdf}
} \hspace{-.7em}
\subfigure[$L = 3$]{
 \ig{.09}{./figs/GP-boxplot-all/boxplot_L3.pdf}
} \hspace{-.7em}
\subfigure[$L = 4$]{
 \ig{.09}{./figs/GP-boxplot-all/boxplot_L4.pdf}
} \hspace{-.7em}
\subfigure[$L = 5$]{
 \ig{.09}{./figs/GP-boxplot-all/boxplot_L5.pdf}
} \hspace{-.7em}
\subfigure[$L = 6$]{
 \ig{.09}{./figs/GP-boxplot-all/boxplot_L6.pdf}
}

 \caption{
 Boxplots of RHV at $100$-th iteration.
 }
 \label{fig:GP-boxplot-all}
\end{figure}


% --------------------------------------------------
% Fig: GP data boxplot: 入力次元の変化
% --------------------------------------------------
\begin{figure}
	\centering
   
	\ig{.4}{./figs/GP-boxplot/GP-boxplot-legend.pdf}
   
	\vspace{-.5em}
   
   \subfigure[$d = 2$]{
	\ig{.14}{./figs/GP-boxplot/boxplot_D2.pdf}
   } \hspace{-.7em}
   \subfigure[$d = 3$]{
	\ig{.14}{./figs/GP-boxplot/boxplot_D3.pdf}
   } \hspace{-.7em}
   \subfigure[$d = 4$]{
	\ig{.14}{./figs/GP-boxplot/boxplot_D4.pdf}
   } \hspace{-.7em}
   
 \caption{
 Boxplot of RHV at $100$-th iteration for each input dimension.
 }
 \label{fig:GP-boxplot-input-dim}
\end{figure}

% --------------------------------------------------
% Fig: GP data boxplot: 入力次元およびlength scale
% --------------------------------------------------
\begin{figure}[t!]
	\centering
   
	\ig{.4}{./figs/GP-boxplot/GP-boxplot-legend.pdf}
   
	\vspace{-.5em}
   
   \subfigure[{\tiny $d = 2, \ell_{\rm RBF} = 0.05$ }]{
	\ig{.15}{./figs/GP-boxplot/boxplot_D2_LS0.05.pdf}
   } \hspace{-.7em}
   \subfigure[{\tiny $d = 2, \ell_{\rm RBF} = 0.1$ }]{
	\ig{.15}{./figs/GP-boxplot/boxplot_D2_LS0.1.pdf}
   } \hspace{-.7em}
   \subfigure[{\tiny $d = 2, \ell_{\rm RBF} = 0.25$ }]{
	\ig{.15}{./figs/GP-boxplot/boxplot_D2_LS0.25.pdf}
   } \hspace{-.7em}
   
   \subfigure[{\tiny $d = 3, \ell_{\rm RBF} = 0.05$ }]{
	\ig{.15}{./figs/GP-boxplot/boxplot_D3_LS0.05.pdf}
   } \hspace{-.7em}
   \subfigure[{\tiny $d = 3, \ell_{\rm RBF} = 0.1$ }]{
	\ig{.15}{./figs/GP-boxplot/boxplot_D3_LS0.1.pdf}
   } \hspace{-.7em}
   \subfigure[{\tiny $d = 3, \ell_{\rm RBF} = 0.25$ }]{
	\ig{.15}{./figs/GP-boxplot/boxplot_D3_LS0.25.pdf}
   } \hspace{-.7em}
   
   \subfigure[{\tiny $d = 4, \ell_{\rm RBF} = 0.05$ }]{
	\ig{.15}{./figs/GP-boxplot/boxplot_D4_LS0.05.pdf}
   } \hspace{-.7em}
   \subfigure[{\tiny $d = 4, \ell_{\rm RBF} = 0.1$ }]{
	\ig{.15}{./figs/GP-boxplot/boxplot_D4_LS0.1.pdf}
   } \hspace{-.7em}
   \subfigure[{\tiny $d = 4, \ell_{\rm RBF} = 0.25$ }]{
	\ig{.15}{./figs/GP-boxplot/boxplot_D4_LS0.25.pdf}
   } \hspace{-.7em}
   
 \caption{
 Boxplot of RHV at $100$-th iteration for each input dimension and length scale.
 % Input-dimension and length scale wise boxplots of RHV at $100$-th iteration.
 }
	\label{fig:GP-boxplot-input-dim-len-scale}
   \end{figure}

% --------------------------------------------------
% Fig: Boxplot for BayesMAP vs NaiveMC
% --------------------------------------------------
\begin{figure}
 \centering
 \ig{.25}{./figs/MCvsBayes/boxplot_all.pdf}
 \caption{
 Boxplot of difference of average RHV between Bayes MAP and na{\"i}ve MC (Bayes MAP minus na{\"i}ve MC).  
 %
 The differences of the $10$ runs average RHV are shown for BO iterations $50$, $75$, and $100$. 
 %
 The GP-derived functions of $d \in \{ 2, 3, 4\}$, $L \in \{ 2, 3, 4 \}$, and $\ell_{\rm RBF} \in \{0.05, 0.1, 0.25\}$ were used (i.e., $27 = 3 \times 3 \times 3$ points for each iteration). 
 %
 Since positive values indicate Bayes MAP is better than na{\"i}ve MC, we see that Bayes MAP shows slightly better performance across iterations.
 }
 \label{fig:BayesMAP-boxplot-app}
\end{figure}


\clearpage

% --------------------------------------------------
\subsection{Additional Results on Benchmark Functions}
\label{app:additional_experiments_bench}



Figure~\ref{fig:results_benchmark-extended} presents an extended version of Fig.~\ref{fig:results_benchmark} from the main text, including additional baseline methods (ParEGO, MOBO-RS, and MESMO).
%
Figure~\ref{fig:results_benchmark-App} shows additional results on benchmark functions.
%
FES1 and FES2 are $(d, L) = (3, 2)$ and $(d, L) = (3, 3)$, respectively.
%
Therefore, FES1$+$Kursawe and FES2$+$Kursawe are $(d, L) = (3, 4)$ and $(d, L) = (3, 5)$, respectively.
%
%\remove{Further, Figure~\ref{fig:results_benchmark_high_indim-App} shows the results on higher dimensional input setting ($d = 10$) of FES1, FES2, and FES3.}
%
The experimental setup is identical to that in Section~\ref{ssec:GPDerivedArtificialFunctions}. 
%
These additional results further demonstrate our method's superior performance across various problem configurations.
% %
% \red{
% Figure~\ref{fig:results_benchmark-extended} presents an extended version of Figure~\ref{fig:results_benchmark} from the main text, including additional baseline methods (ParEGO, MOBO-RS, and MESMO) that were omitted from the main text due to space limitations. 
% %
% The experimental setup is identical to that in Section~\ref{ssec:GPDerivedArtificialFunctions}. These additional results further demonstrate our method's superior performance across various problem configurations.
% }


% --------------------------------------------------
% 
% --------------------------------------------------
\begin{figure}[t!]
	\centering
	\subfigure[Fonseca-Fleming]{ % $(d, L) = (2, 2)$
	  \ig{.2}{./figs/benchmark-appendix/RHV_Fonseca_Fleming_max_input_dim_2_output_dim_2.pdf}
	}
	\subfigure[Kursawe]{ % $(d, L) = (3, 2)$
	  \ig{.2}{./figs/benchmark-appendix/RHV_Kursawe_max_input_dim_3_output_dim_2.pdf}
	}
	\subfigure[Viennet]{ % $(d, L) = (2, 3)$
	  \ig{.2}{./figs/benchmark-appendix/RHV_Viennet_max_input_dim_2_output_dim_3.pdf}
	}
	\subfigure[FES3]{ % $(d, L) = (3, 4)$
	  \ig{.2}{./figs/benchmark-appendix/RHV_FES3_max_input_dim_3_output_dim_4.pdf}
	}
	\subfigure[Fonseca$+$Viennet]{ % $(d, L) = (2, 5)$
	  \ig{.2}{./figs/benchmark-appendix/RHV_Fonseca_Viennet_scaled_max_input_dim_2_output_dim_5.pdf}
	}
	\subfigure[FES3$+$Kursawe]{ % $(d, L) = (3, 6)$
	  \ig{.2}{./figs/benchmark-appendix/RHV_FES3_Kursawe_scaled_max_input_dim_3_output_dim_6.pdf}
	} 
	
	 \caption{
	 % ベンチマーク関数における性能比較（10回の実行における平均値と標準誤差）
	 Performance comparison in benchmark functions (average and standard deviation of $10$ runs).
	 }
	 \label{fig:results_benchmark-extended}
	\end{figure}

To assess the scalability of the proposed method, we extend our experiments to higher input dimensions.
%
Figures~\ref{fig:results_FES1_high_indim-App},~\ref{fig:results_FES2_high_indim-App}, and~\ref{fig:results_FES3_high_indim-App} display the results for FES1, FES2, and FES3 benchmark functions with input dimensions ranging from $d = 5$ to $d = 10$.
%
All experimental settings except for the input dimension are identical to those in the main text.
%
The results show that our method demonstrates stable optimization performance as the input dimension increases, similar to the cases presented in the main text.
%
% Investigating the method's performance in even higher dimensions for real-world applications remains an important direction for future research.
Additionally, we evaluated our method on the DTLZ benchmark suite with $(d, L) = (3, 3)$, as shown in Figure~\ref{fig:results_DTLZ-App}.
%
On DTLZ2, DTLZ5, DTLZ6, and DTLZ7, our proposed method achieves higher RHV compared to other methods.
%
For DTLZ1 and DTLZ3, all methods show similarly high RHV values (close to 1) with small differences between them.
%
In the case of DTLZ4, EHVI and MESMO demonstrate better performance, while our method performs comparably to the remaining baselines.


% --------------------------------------------------
% Fig: Additional Bench 1
% --------------------------------------------------
\begin{figure}[t!]
\subfigure[FES1]{ 
  \ig{.22}{./figs/Bench1/RHV_FES1_max_input_dim_3_output_dim_2.pdf}
}
\subfigure[FES2]{ 
  \ig{.22}{./figs/Bench1/RHV_FES2_max_input_dim_3_output_dim_3.pdf}
}

\subfigure[FES1$+$Kursawe]{ 
  \ig{.22}{./figs/Bench1/RHV_FES1_Kursawe_scaled_max_input_dim_3_output_dim_4.pdf}
}
\subfigure[FES2$+$Kursawe]{ 
  \ig{.22}{./figs/Bench1/RHV_FES2_Kursawe_scaled_max_input_dim_3_output_dim_5.pdf}
} 

 \caption{
 Performance comparison in additional benchmark functions (average and standard deviation of $10$ runs).
 }
 \label{fig:results_benchmark-App}
\end{figure}


% --------------------------------------------------
% Fig: FES1
% --------------------------------------------------
\begin{figure}[t!]
	\centering
   
	\subfigure[$d = 5$]{
	\ig{.22}{./figs/FES/RHV_FES1_max_input_dim_5_output_dim_2.pdf}}
	\subfigure[$d = 6$]{
	\ig{.22}{./figs/FES/RHV_FES1_max_input_dim_6_output_dim_2.pdf}}
	
	\subfigure[$d = 7$]{
	\ig{.22}{./figs/FES/RHV_FES1_max_input_dim_7_output_dim_2.pdf}}
	\subfigure[$d = 8$]{
	\ig{.22}{./figs/FES/RHV_FES1_max_input_dim_8_output_dim_2.pdf}}
	
	\subfigure[$d = 9$]{
	\ig{.22}{./figs/FES/RHV_FES1_max_input_dim_9_output_dim_2.pdf}}
	\subfigure[$d = 10$]{
	\ig{.22}{./figs/FES/RHV_FES1_max_input_dim_10_output_dim_2.pdf}}
 \caption{
 Results on FES1.
 }
	\label{fig:results_FES1_high_indim-App}
   \end{figure}

% --------------------------------------------------
% Fig: FES2
% --------------------------------------------------
\begin{figure}[t!]
	\centering
   
	\subfigure[$d = 5$]{
	\ig{.22}{./figs/FES/RHV_FES2_max_input_dim_5_output_dim_3.pdf}}
	\subfigure[$d = 6$]{
	\ig{.22}{./figs/FES/RHV_FES2_max_input_dim_6_output_dim_3.pdf}}
	\subfigure[$d = 7$]{
	
	\ig{.22}{./figs/FES/RHV_FES2_max_input_dim_7_output_dim_3.pdf}}
	\subfigure[$d = 8$]{
	\ig{.22}{./figs/FES/RHV_FES2_max_input_dim_8_output_dim_3.pdf}}
	\subfigure[$d = 9$]{
	
	\ig{.22}{./figs/FES/RHV_FES2_max_input_dim_9_output_dim_3.pdf}}
	\subfigure[$d = 10$]{
	\ig{.22}{./figs/FES/RHV_FES2_max_input_dim_10_output_dim_3.pdf}}
	\caption{
Results on FES2.
	}
	\label{fig:results_FES2_high_indim-App}
   \end{figure}

% --------------------------------------------------
% Fig: FES3
% --------------------------------------------------
\begin{figure}[t!]
	\centering
   
	\subfigure[$d = 5$]{
	\ig{.22}{./figs/FES/RHV_FES3_max_input_dim_5_output_dim_4.pdf}}
	\subfigure[$d = 6$]{
	\ig{.22}{./figs/FES/RHV_FES3_max_input_dim_6_output_dim_4.pdf}}
	\subfigure[$d = 7$]{
	
	\ig{.22}{./figs/FES/RHV_FES3_max_input_dim_7_output_dim_4.pdf}}  
	\subfigure[$d = 8$]{
	\ig{.22}{./figs/FES/RHV_FES3_max_input_dim_8_output_dim_4.pdf}}
	\subfigure[$d = 9$]{
	
	\ig{.22}{./figs/FES/RHV_FES3_max_input_dim_9_output_dim_4.pdf}}
	\subfigure[$d = 10$]{
	\ig{.22}{./figs/FES/RHV_FES3_max_input_dim_10_output_dim_4.pdf}}
	\caption{
 Results on FES3.
	}
	\label{fig:results_FES3_high_indim-App}
   \end{figure}
\clearpage

% % --------------------------------------------------
% % Fig: Additional Bench 2
% % --------------------------------------------------
% \begin{figure}[t!]
% \centering
% \subfigure[FES1-10]{ 
%  \ig{.22}{./figs/Bench2/RHV_FES1_max_input_dim_10_output_dim_2.pdf}
% }
% \subfigure[FES2-10]{ 
%  \ig{.22}{./figs/Bench2/RHV_FES2_max_input_dim_10_output_dim_3.pdf}
% }
% \subfigure[FES3-10]{ 
%  \ig{.22}{./figs/Bench2/RHV_FES3_max_input_dim_10_output_dim_4.pdf}
% }

%  \caption{
%  \remove{Performance comparison in benchmark functions (average and standard deviation of $10$ runs).}
%  }
%  \label{fig:results_benchmark_high_indim-App}
% \end{figure}


% --------------------------------------------------
% Fig: dim = 3
% --------------------------------------------------
\begin{figure}[t!]
	\centering
   
   \subfigure[DTLZ1]{
	% \ig{.3}{./benchmark/RHV_pymoo_DTLZ1_3_3_max_input_dim_3_output_dim_3.pdf}
	\ig{.22}{./figs/benchmark-ver2/RHV_pymoo_DTLZ1_3_3_max_input_dim_3_output_dim_3.pdf}
   }
   \subfigure[DTLZ2]{
	% \ig{.3}{./benchmark/RHV_pymoo_DTLZ2_3_3_max_input_dim_3_output_dim_3.pdf}
	\ig{.22}{./figs/benchmark-ver2/RHV_pymoo_DTLZ2_3_3_max_input_dim_3_output_dim_3.pdf}
   }

   \subfigure[DTLZ3]{
	% \ig{.3}{./benchmark/RHV_pymoo_DTLZ3_3_3_max_input_dim_3_output_dim_3.pdf}
	\ig{.22}{./figs/benchmark-ver2/RHV_pymoo_DTLZ3_3_3_max_input_dim_3_output_dim_3.pdf}
   }
   \subfigure[DTLZ4]{
	% \ig{.3}{./benchmark/RHV_pymoo_DTLZ4_3_3_max_input_dim_3_output_dim_3.pdf}
	\ig{.22}{./figs/benchmark-ver2/RHV_pymoo_DTLZ4_3_3_max_input_dim_3_output_dim_3.pdf}
   }

   \subfigure[DTLZ5]{
	% \ig{.3}{./benchmark/RHV_pymoo_DTLZ5_3_3_max_input_dim_3_output_dim_3.pdf}
	\ig{.22}{./figs/benchmark-ver2/RHV_pymoo_DTLZ5_3_3_max_input_dim_3_output_dim_3.pdf}
   }
   \subfigure[DTLZ6]{
	% \ig{.3}{./benchmark/RHV_pymoo_DTLZ6_3_3_max_input_dim_3_output_dim_3.pdf}
	\ig{.22}{./figs/benchmark-ver2/RHV_pymoo_DTLZ6_3_3_max_input_dim_3_output_dim_3.pdf}
   }
   
   \subfigure[DTLZ7]{
	% \ig{.3}{./benchmark/RHV_pymoo_DTLZ7_3_3_max_input_dim_3_output_dim_3.pdf}
	\ig{.22}{./figs/benchmark-ver2/RHV_pymoo_DTLZ7_3_3_max_input_dim_3_output_dim_3.pdf}
   }
   
	\caption{
	{Results on DTLZ ($d = 3, L = 3$). 
	%
	% The settings are same as the main text.
	}}
	% \label{fig:}
	\label{fig:results_DTLZ-App}
   \end{figure}


   




% --------------------------------------------------
\subsection{Computational Time}
\label{app:time}

We here examine the computational time of PFEV.
%
We used the GP-derived synthetic function ($d = 3$) from Section~\ref{ssec:GPDerivedArtificialFunctions}. 
%
The training dataset was randomly selected $50$ points, and we evaluated the computational time (CPU time) required to calculate the acquisition function values for $100$ points generated by the Latin hyper cube sampling.
%
In PFEV, we evaluate time of calculating $11$ grid points of $\lambda$ ($10^{-3}, 0.1, 0.2, \ldots, 1.0$) for a given $\*x$.
%
% The results are shown in Table~\ref{tab:time}, in which we evaluate ParEGO, JES, PFES, EHVI, and PFEV (Proposed). 
The results are shown in Table~\ref{tab:time}, in which we evaluate ParEGO, PFES, EHVI, and PFEV (Proposed). 


Obviously, ParEGO was quite fast because it applies the usual single-objective BO to the scalarized value.
%
For $L = 3$ and $4$, EHVI was also fast, but it becomes slow at $L = 5$ and we stopped it at $L = 6$ because of the long computational time.
%
The slow computation of EHVI at large $L$ is widely known. 
%
PFEV and PFES were similar up to $L = 4$, but for $L = 5$ and $L = 6$, PFEV was slower than PFES.
%
This is because of the computation of QHV. 
%
% For $L = 3$ and $L = 4$, the computational time of NSGAII was dominant in PFEV (Note that the same procedure is also performed in PFES and JES).
For $L = 3$ and $L = 4$, the computational time of NSGAII was dominant in PFEV (Note that the same procedure is also performed in PFES).
%
However, for $L = 5$, QHV requires the similar cost as NSGAII, and for $L = 6$, the computational cost of QHV became much larger than NSGAII.
%
% Since PFEV requires QHV two times for each sampled Pareto-frontier (see Appendix~\ref{app:CalcZ}) while PFES (and JES) requires QHV only once for each sampled Pareto-frontier.
PFEV requires QHV two times for each sampled Pareto-frontier (see Appendix~\ref{app:CalcZ}) while PFES requires QHV only once for each sampled Pareto-frontier.
%
This was major reason of the difference of PFEV and PFES in $L = 6$.
%
% On the other hand, JES requires longer time for $L = 5$ and $6$.
%
% JES requires computations of the GP predictive distributions given $\cX^*$ and $\cF^*$ for each MC sample (i.e., the $K \times L$ additional predictive distribution calculation is required for each candidate $\*x$). 

% --------------------------------------------------
% Table: Time 
% --------------------------------------------------
\begin{table*}
 \centering
 \caption{
 CPU time evaluation (sec).
 }
 \label{tab:time}
\begin{tabular}{ll|rrrr}
 &  & $L = 3$
 & $L = 4$
 & $L = 5$
 & $L = 6$
\\ \hline
ParEGO &
 & 0.95 $\pm$ 0.08 & 1.15 $\pm$ 0.06 & 1.38 $\pm$ 0.07 & 1.62 $\pm$ 0.11\\ \hline
% JES &
%  & 22.61 $\pm$ 0.15 & 31.41 $\pm$ 0.34 & 92.43 $\pm$ 10.43 & 1364.70 $\pm$ 469.52\\ \hline
PFES &
 & 21.43 $\pm$ 0.20 & 29.18 $\pm$ 0.39 & 45.23 $\pm$ 1.41 & 127.64 $\pm$ 24.44\\ \hline
EHVI &
 & 0.86 $\pm$ 0.06 & 3.51 $\pm$ 2.24 & 500.09 $\pm$ 336.18 & - \\ \hline
Proposed & Total
 & 21.93 $\pm$ 0.42 & 31.74 $\pm$ 0.64 & 61.04 $\pm$ 3.26 & 274.49 $\pm$ 28.99\\
 & \textsc{CalcPFEV}
 & 0.59 $\pm$ 0.05 & 1.56 $\pm$ 0.13 & 5.04 $\pm$ 0.49 & 24.76 $\pm$ 3.71\\
 & NSGAII
 & 19.59 $\pm$ 0.37 & 25.66 $\pm$ 0.37 & 31.36 $\pm$ 0.27 & 37.26 $\pm$ 0.22\\
 & RFM
 & 0.59 $\pm$ 0.00 & 0.80 $\pm$ 0.01 & 1.00 $\pm$ 0.00 & 1.19 $\pm$ 0.00\\
 & QHV
 & 0.42 $\pm$ 0.03 & 2.72 $\pm$ 0.26 & 22.41 $\pm$ 2.65 & 209.81 $\pm$ 25.68\\
%  &
%  & $L = 3$
%  & $L = 4$
%  & $L = 5$
%  & $L = 6$
% \\ \hline
% ParEGO &
%  & 0.95 $\pm$ 0.08 & 1.15 $\pm$ 0.06 & 1.38 $\pm$ 0.07 & 1.62 $\pm$ 0.11\\ \hline
% JES &
%  & 22.61 $\pm$ 0.15 & 31.41 $\pm$ 0.34 & 92.43 $\pm$ 10.43 & 1364.70 $\pm$ 469.52\\ \hline
% PFES &
%  & 21.43 $\pm$ 0.20 & 29.18 $\pm$ 0.39 & 45.23 $\pm$ 1.41 & 127.64 $\pm$ 24.44\\ \hline
% EHVI &
%  & 0.86 $\pm$ 0.06 & 3.51 $\pm$ 2.24 & 500.09 $\pm$ 336.18 & nan $\pm$ nan\\ \hline
% Proposed & Total
%  & 21.93 $\pm$ 0.42 & 31.74 $\pm$ 0.64 & 61.04 $\pm$ 3.26 & 274.49 $\pm$ 28.99\\
%  & \textsc{CalcPFEV}
%  & 0.59 $\pm$ 0.42 & 1.56 $\pm$ 0.64 & 5.04 $\pm$ 3.26 & 24.76 $\pm$ 28.99\\
%  & NSGAII
%  & 19.59 $\pm$ 0.42 & 25.66 $\pm$ 0.64 & 31.36 $\pm$ 3.26 & 37.26 $\pm$ 28.99\\
%  & RFM
%  & 0.59 $\pm$ 0.42 & 0.80 $\pm$ 0.64 & 1.00 $\pm$ 3.26 & 1.19 $\pm$ 28.99\\
%  & QHV
%  & 0.42 $\pm$ 0.42 & 2.72 $\pm$ 0.64 & 22.41 $\pm$ 3.26 & 209.81 $\pm$ 28.99\\
\end{tabular}
\end{table*}

% --------------------------------------------------
% % \section{ベンチマーク関数の詳細}
% \section{Benchmark Functions}
% \label{app:benchmarks}

% % 以下にベンチマーク関数の定義を示す．
% %
% % ただし，$\*x_M$は，$\*x$の末尾$(d - L + 1)$成分からなる部分ベクトルである．
% %
% % また以下の関数は最小化用に作られたものであるため，実験では符号を反転したものを使用している．
% All the following benchmark functions were originally proposed for the minimization problem.
% %
% In our experiments, we flipped the sign and used as maximization problems.
% %
% Note that $\*x_M$ indicates the last $(d - L + 1)$ dimensions of $\*x$.


% \subsection{FES3}
% % FES3関数は以下のように定義される．
% FES3 is defined as
% {\small
% \begin{align*}
% f_1(\*{x}) &= -\sum_{i=1}^d \left|x_i - \frac{\exp\left(\left(\frac{i}{d}\right)^2\right)}{3}\right|^{0.5}, \\
% f_2(\*{x}) &= -\sum_{i=1}^d \left|x_i - \sin(i-1)^2 \cos(i-1)^2\right|^{0.5}, \\
% f_3(\*{x}) &= -\sum_{i=1}^d \left|x_i - \left(0.25 \cos(i-1) \cos(2i-1) - 0.5\right)\right|^{0.5}, \\
% f_4(\*{x}) &= -\sum_{i=1}^d \left(x_i - \frac{1}{2}\sin\left(1000\pi\frac{i}{d}\right) - \frac{1}{2}\right)^2 \\
% \text{subject to} &\quad 0 \leq x_i \leq 1, \quad i=1, 2, \ldots, d.
% \end{align*}}

% \subsection{Sphere}
% % 入力次元$d=2$のSphere関数は以下のように定義される．
% Sphere is defined as
% \begin{align*}
%   f(\*{x}) &= \sum_{i=1}^{d} x_i^2 \\
% \text { subject to }  &\quad -5.12 \leq x_i \leq 5.12,  \quad\text { for } i=1,2, \ldots, d.
% \end{align*}

% \subsection{DTLZ2}
% % 入力次元$d$のDTLZ2関数は以下のように定義される．
% DTLZ2 is defined as
% \begin{align*}
% f(\*{x}) &= -\left(1 + g(\*x_M)\right) \prod_{i=1}^{M-1} \cos\left(\frac{\pi}{2} x_i\right), \\
% \quad g(\*x_M) &= \sum_{x_i \in \*x_M} \left(x_i - 0.5\right)^2 \\
% \text{subject to} &\quad 0 \leq x_i \leq 1, \quad i=1, 2, \ldots, d.
% \end{align*}

% \subsection{DTLZ4}
% % 入力次元$d$のDTLZ4関数は以下のように定義される．
% DTLZ4 is defined as
% \begin{align*}
% f(\*{x}) &= -\left(1 + g(\*x_M)\right) \prod_{i=1}^{M-1} \cos\left(\frac{\pi}{2} x_i^\alpha\right), \\
% \quad g(\*x_M) &= \sum_{x_i \in \*x_M} \left(x_i - 0.5\right)^2 \\
% \text{subject to} &\quad 0 \leq x_i \leq 1, \quad i=1, 2, \ldots, d,
% \end{align*}
% where the scaling coefficient $\alpha$ is set as $100$ that are typically used in the past works.
% % スケーリング係数$\alpha$は典型的な設定である100を採用した．

% \subsection{Rosenbrock}
% % 入力次元$d$のRosenbrock関数は以下のように定義される．
% Rosenbrock is defined as
% \begin{align*}
% f(\*{x}) &= -\sum_{i=1}^{d-1} \left[100 \left(x_{i+1} - x_i^2\right)^2 + \left(1 - x_i\right)^2 \right] \\
% \text{subject to} &\quad -2.048 \leq x_i \leq 2.048, \quad i=1, 2, \ldots, d.
% \end{align*}

% --------------------------------------------------
% \section{\red{Hyper-volume and Truncation Error Analysis}}
\section{Difference of Over- and Under-Truncation}
\label{app:hyper-volume}


Here, we discuss approximation error caused by replacing the dominated region by the entire Pareto-frontier $\cA^{\cF^*}$ with its counter-part created by $\cF_S^*$, i.e., $\cA_O^{\cF_S^*}$ or $\cA_U^{\cF_S^*}$.
%
The difference actually can be small if $S$ is sufficiently large, but practically intractable size of $S$ is required even for reasonable size of $L$.
%
To demonstrate this claim, we evaluate differences of hyper-volumes of $\cA_O^{\cF_S^*}$ and $\cA_U^{\cF_S^*}$.
%
If the difference of $\cA_O^{\cF_S^*}$ and $\cA_U^{\cF_S^*}$ are small, it suggests that the true Pareto-frontier $\cF^*$ can be accurately approximated by $\cF_S^*$. 


% \red{
% As shown in Figure~\ref{fig:hyper-volume-analysis} (c)-(d), if the population size of NSGA-II increases, the differences between over-truncation and the true truncation decreases. 
% %
% However, the continuous Pareto-frontier is the $(L-1)$-dimensional space, for which the required number of points to keep the sufficient density of approximation points increases exponentially when $L$ increases. 
% }

{
In Fig.~\ref{fig:hyper-volume-analysis}, we empirically investigate the ratio of the volume of under- and over- truncations compared with the true volume. 
%
We assume that the Pareto-frontier is the simplex ($\sum_{i \in [L]} f^i = 1$ and $f^i \geq 0$), and approximation points $\cF^*_S$ are sampled uniformly in the simplex as shown in Fig.~\ref{fig:hyper-volume-analysis} (a). 
%
The examples of the volume ratio is shown in Fig.~\ref{fig:hyper-volume-analysis} (b).
%
In Fig.~\ref{fig:hyper-volume-analysis}~(c), we see that, when $L = 2$, the difference between the truncations rapidly decreases, but for $L \geq 3$ shown in Fig.~\ref{fig:hyper-volume-analysis}~(d) and (e), large differences remain even when the population size is 1,000 (Note that in this example, over-truncation is closer to the true value than under-truncation, but in general, it depends on the shape of the true Pareto frontier which is unknown).
%
The continuous Pareto-frontier is the $(L-1)$-dimensional space, and we conjecture that the required number of points to keep the sufficient density of approximation points $\cF_S^*$ increases exponentially when $L$ increases. 
}


About the difference between $\cF^*$ and $\cF^*_S$, increasing the number of MC samples cannot mitigate the essential problem in principle.
%
In our formulation, the over-truncation corresponds to $\lambda = 0$. Therefore, the over-truncation based lower bound is biased toward a smaller value, because the bound is defined as the maximizer with respect to $\lambda$. 
%
This discussion holds even in the population 
$\mr{LB}(\boldsymbol x, \lambda)$ 
(i.e., before introducing the sample approximation), and therefore, increasing the number of samples from the GPs does not solve this intrinsic bias.

% --------------------------------------------------
% Fig: Volume ratio
% --------------------------------------------------
\begin{figure*}
 \centering
 
 \subfigure[{
 Illustration of $L = 3$. 
 %
 The true Pareto-frontier is assumed to be the simplex. 
 %
 The discretized points (red points) are sampled from the uniform distribution on the simplex (Dirichlet distribution).}]{
 \ig{.2}{./figs/volume/PF.pdf}
 } ~~~
 \subfigure[
 {
 The difference between two truncations is evaluated by the volume of the colored region defined in the $L$-dimensional unit cube $[0,1]^L$.
 %
 When $L = 2$, the true volume is $1/2$. 
 %
 % In the plot (c), the area of the orange region divided by $1/2$ and the blue region divided by $1/2$ are evaluated, respectively. 
 In the plot (c), the areas of the orange and the blue regions are compared (each of which are divided by $1/2$ in (c), respectively). 
 }]{ 
 \ig{.4}{./figs/volume/volume-diff.pdf}
 }
 

 \subfigure[$L = 2$]{
 \ig{.4}{./figs/volume/vol_ratio_outdim2.pdf}
 }
 \subfigure[$L = 3$]{
 \ig{.4}{./figs/volume/vol_ratio_outdim3.pdf}
 } 
 \subfigure[$L = 4$]{
 \ig{.4}{./figs/volume/vol_ratio_outdim4.pdf}
 }
 
 \caption{
 {
 Hyper-volume relative differences between over- and under- truncations.
 %
 The volume is defined in the unit cube $[0,1]^L$.
 %
 The vertical axis is the ratio compared with the true volume.
 }}
 % \label{fig:}
 \label{fig:hyper-volume-analysis}
\end{figure*}


% --------------------------------------------------
\section{Consideration on Gradient-based Optimizer}
\label{app:gradient}

Figure~\ref{fig:qlogNEHVI} shows results with qLogNEHVI \citep{daulton20differentiable,daulton21parallel,ament2023unexpected} for GP-derived functions ($d = 3, L = 3, 4, 5$) and four benchmark functions. 
%
For qLogNEHVI, we used qLogNoisyExpectedHypervolumeImprovement of BoTorch. 
%
The reference point is defined by $y_{\min} - 0.1 (y_{\max} - y_{\min})$, where $y_{\min}$ and $y_{\max}$ are vectors consisting of the minimum and the maximum of each dimension in training $\*y_i$, respectively. 
%
For qLogNEHVI, we used both the gradient descent ({\tt optimize\_acqf} function of BoTorch) and DIRECT for the GP-derived functions. 
%
We see that the gradient optimizer slightly improves the results, but DIRECT also has the similar performance. 
%
Overall, qLogNEHVI shows good performance, while PFEV also shows comparable performance. 
%
Although implementations are not exactly consistent (PFEV is GPy base and qLogNEHVI is BoTorch), we can see that performance in our results is not largely different from the well-known package. 

% --------------------------------------------------
% qLogNEHVI
% --------------------------------------------------
\begin{figure}
 \centering
   
 \subfigure[$L = 3$]{
 \ig{.35}{./figs/qLogNEHVI/GP/RHV_input_dim_3output_dim_3_length_scale_0.1.pdf}
 }
 \subfigure[$L = 4$]{
 \ig{.35}{./figs/qLogNEHVI/GP/RHV_input_dim_3output_dim_4_length_scale_0.1.pdf}
 }
 \subfigure[$L = 5$]{
 \ig{.35}{./figs/qLogNEHVI/GP/RHV_input_dim_3output_dim_5_length_scale_0.1.pdf}
 }
   
 \caption{
 Comparison with qLogNEHVI.
 }
 \label{fig:qlogNEHVI}
\end{figure}
